Deconvolution with Unknown Error Distribution Interpreted as Blind Isotonic Regression

Deconvolution is a statistical inverse problem to estimate the distribution of a random variable based on its noisy observations. Despite the extensive studies on the topic, deconvolution with unknown noise distribution remains as a notoriously hard problem. We propose a matrix-based viewpoint for collective deconvolution that subsumes the setup with repeated measurements as a special case. As the main result, we describe a simple algorithm that partially utilizes matrix structure to solve deconvolution problem and provide non-asymptotic error analysis for the algorithm. We show that the proposed algorithm achieves the minimax optimal rate for deconvolution in a restricted sense. We also remark the connection between the collective deconvolution and the so-called statistical seriation as a byproduct or our matrix viewpoint. We conjecture that the link suggests that collective deconvolution, as well as deconvolution with repeated measurements, is intrinsically much easier than usual deconvolution of a single distribution.

==> contents/03_algorithm_copy.tex <==
\section{Algorithm}\label{sec:algorithm}

In this section, we describe our algorithm for estimating the matrix $A$. The generic algorithm consists of three steps: 
(1) column feature (= quantile) estimation; (2) CDF (which turns out to be the inverse of the latent function) estimation; and 
(3) the estimation of the matrix entries by combining them together. The details in the first two steps vary depending on 
the noise assumptions.

First, we describe a ``generic recipe'' of our matrix estimation algorithm in Section \ref{sec:alg_generic}. Next, we introduce 
some notations in Section \ref{sec:notation_algorithm} that are needed to describe the detailed algorithms.
Then we discuss the details of the algorithm adapted to each of the three noise scenarios considered in this work: 
the noiseless setup in Section \ref{sec:alg_noiseless}; the noisy setup with known noise distribution in Section 
\ref{sec:alg_noisy_known}; and the noisy setup with unknown noise distribution in Section \ref{sec:alg_noisy_unknown}.


\subsection{Generic Recipe of Our Algorithm}\label{sec:alg_generic}
We shall use a ``generic recipe'' for estimation in all three noise scenarios considered in this work: noiseless, noisy with known 
noise distribution, and noisy with unknown noise distribution. The generic algorithm described in Algorithm \ref{alg:generic} 
is adapted for each setup to deal with the effect of the noise: see Sections \ref{sec:alg_noiseless}, \ref{sec:alg_noisy_known}, 
\ref{sec:alg_noisy_unknown}.

\begin{algorithm}
\caption{Generic recipe of the algorithm}
\label{alg:generic}
{
	\begin{enumerate}
		\item Estimate the latent feature (=quantile) $\fcol{j}$ of column $j $. Let it be denoted by $\hat{q}(j)$ ~$j \in [n]$.
		\item Estimate $F^{(i)} =  g^{-1}_{x=\frow{i}}$ on row $i$, which is the inverse of the latent function $g \big( \frow{i}, \cdot \big)$ restricted on the first coordinate. Let it be denoted by $\hat{F}^{(i)}$, ~$i \in [m]$.
		\item Plug in the estimates: $\hat{A}(i,j) = \hat{g}^{(i)}(\hat{q}(j))$, ~$i \in [m], ~j \in [n]$, 
			where $\hat{g}^{(i)} = \big(\hat{F}^{(i)}\big)^{-1}$.		
	\end{enumerate}
}
\end{algorithm}


In step 1, we estimate the latent column feature by the average of the corresponding column's order statistic. 
In step 2, we estimate the latent function for each row of the matrix by estimating the corresponding CDF. 
Specifically, we take empirical CDF in the noiseless setup, and use a kernel deconvolution estimator in the noisy setups.

We note that for any given $x \in [0,1]$, the latent function $g(x, \cdot): [0,1] \to \mathbb{R}$ is continuous and monotone 
increasing with respect to the second argument, and hence invertible due to our model assumptions. For each fixed $x$, 
$g^{-1}(x, \cdot): \mathbb{R} \to [0,1]$, can be viewed as a cumulative distribution function (CDF) for a certain distribution on 
$\mathbb{R}$. That is, for each row $i \in [m]$, we can consider the latent function $g(x, \cdot)$ restricted to $x = \frow{i}$ as 
the inverse of the CDF\footnote{See Definitions \ref{defn:CDF} and \ref{defn:Quantile} in Appendix \ref{appx:distribution} for details.} 
of signal along row $i$. The method for estimating $F^{(i)}$ varies depending upon whether it is noiseless or noisy with 
known/unknown noise distribution. 

In the last step, matrix entries are estimated to be the evaluation of the latent function estimated in step 2 at the column feature 
estimated in step 1.


\subsection{Notation Used in Detailed Algorithm Description}\label{sec:notation_algorithm}
For $i \in [m]$, and for $j \in [n]$, we define
\begin{align}
	\cB_i &= \{ j' \in [n]: M(i,j') = 1 \},		\label{eqn:set_support_row}\\
	\cB^j &= \{ i' \in [m]: M(i',j) = 1 \}.	\label{eqn:set_support_column}
\end{align}
We let $\bbI$ denote the indicator function, i.e., given a boolean formula, namely, `condition', $\bbI\{\text{condition} \} = 1$ if and only 
if condition is true (and $0$ otherwise). Lastly, we define $\bbI_H: \Reals \to \left\{0, \frac{1}{2}, 1 \right\}$ as
\begin{equation}\label{eqn:Heaviside}
	\heavi{x} = \frac{1}{2} \big( \Ind{x > 0} + \Ind{ x\geq 0 } \big).
\end{equation}


For completeness, we describe how our algorithm handles exceptions such as $\cB_i = \emptyset$ or $\cB^j = \emptyset$. 
For $j \in [n]$ with $\cB^j = \emptyset$, we let our algorithm output a trivial estimate $\hfcol{j} = \frac{1}{2} $. Likewise, for $i \in [m]$ with 
$\cB_i = \emptyset$, we let our algorithm return a trivial estimate $\hat{g}^{(i)} (z) = (\fmax - \fmin) z + \fmin $ for $z \in [0,1]$.
In case, $\fmin, \fmax$ are not known a priori, we instead use any given constants $\tfmin, \tfmax$ such that $ \tfmin \leq \fmin$ 
and $ \tfmax \geq \fmax$.



\subsection{Details for the Noiseless Setup}\label{sec:alg_noiseless}

%\subsubsection{Column Feature Estimation}
\begin{itemize}
\item Column Feature Estimation: 
Given $j \in [n]$, we define 
\begin{equation}\label{eqn:quantile_rowwise}
	\hat{q}_i(j) = \frac{\sum_{j' \in \cB_i}  \heavi{ Z(i, j) - Z(i, j') } }{| \cB_i |}. 	
\end{equation}
for all $i \in \cB^j$. Then we define our estimate for $\fcol{j}$ to be
\begin{equation}\label{eqn:quantile_est}
	\hat{q}(j) = \hat{q}_{i^*(j)}(j)
\end{equation}
where $i^*(j)$ is chosen uniformly at random from $\cB^j$.

%\subsubsection{CDF Estimation}
\item CDF Estimation: 
For $i \in [m]$, we define $\breve{F}^{(i)}: \Reals \to [0,1]$ as
\begin{equation}\label{eqn:ECDF_noiseless}
	\breve{F}^{(i)} (z) = \frac{\sum_{j' \in \cB_i } \Ind{Z(i,j') \leq z }}{| \cB_i |}.
\end{equation}

%\subsubsection{Final Estimator $\breve{\varphi}$}
\item Final Estimator $\breve{\varphi}$: 
For each $i \in [m]$, let $\breve{g}^{(i)} = \big(\breve{F}^{(i)}\big)^{-1}$ denote the quantile function (right pseudo-inverse) 
associated with $\breve{F}^{(i)}$. For $(i,j) \in [m] \times [n]$, we let
\begin{equation}\label{eqn:estimate_noiseless}
	\breve{A}(i,j) = \breve{\varphi}(Z)(i,j) = \breve{g}^{(i)}\left( \hat{q}(j) \right).
\end{equation}
\end{itemize}

\subsection{Details for the Noisy Setup with Known Noise Distribution}\label{sec:alg_noisy_known}
The generic algorithm remains the same as that described in Algorithm \ref{alg:generic}. However, the details of step 1 
(estimating $\fcol{j}$, ~$j \in [n]$) and step 2 (estimating $F^{(i)}$, ~$i \in [m]$) change due to presence of noise. 
We shall explicitly use the knowledge of noise distribution in step 2. 		

\begin{itemize}
%\subsubsection{Column Feature Estimation}
\item Column Feature Estimation: 
For $j \in [n]$, we define 
\begin{align}\label{eqn:Z_marg}
	Z_{\marg}(j) \frac{ \sum_{i' \in \cB^j } Z(i',j)}{ | \cB^j |}.
\end{align}
Then,  we estimate the column feature of $j \in [n]$ as
\begin{align}\label{eqn:estimate_marg}
	\hat{q}_{\marg}(j) & = \frac{1}{n}\sum_{j' = 1}^n ~\heavi{ Z_{\marg}(j) - Z_{\marg}(j') }.
\end{align}

%\subsubsection{CDF Estimation}\label{sec:CDFest_noisy_known}
\item CDF Estimation:
Let $\phi_N$ denote the Fourier transform of the noisy density. Let $K$ be a symmetric Kernel with $\phi_K$ being 
its Fourier transform such that $\supp \phi_K \subset [-1,1]$. Using $K$ and the knowledge on the noise distribution, 
we define function $L$ as $L \triangleq  \cF^{-1} \left\{ \frac{ \phi_K(\, \cdot \,) }{\phi_N(\, \cdot \, h^{-1})} \right\}$, i.e.,
\begin{align}\label{eqn:kernel_known_main}
	L(z) = \frac{1}{2\pi} \int \exp(- \img\, t z ) \frac{\phi_K(t)}{\phi_N\left(\frac{t}{h}\right)} dt, ~~z \in \Reals.
\end{align}

Next, we define $\tilde{F}^{(i)}$, estimate of $F^{(i)}$ as follows. Suppose two constants $\tfmin, \tfmax$ such that 
$\tfmin \leq \fmin$ and $\tfmax \geq \fmax$ are given. For $i \in [m]$, let
\begin{equation}\label{eqn:ECDF_known_noise}
	\tilde{F}^{(i)}(z) = \begin{cases}
		\int_{\tfmin}^{z } \tilde{f}^{(i)}(w) dw,	& \text{if } z < \tfmax,\\
		1,							& \text{if } z \geq \tfmax.
	\end{cases}
\end{equation}
where we define
\begin{align}
	\tilde{f}^{(i)}(z) &= \frac{1}{h |\cB_i|} \sum_{j\in \cB_i} L \left( \frac{z- Z(i,j)}{h} \right). \label{eqn:known_density}
\end{align}
Here, $h$ denotes the kernel bandwidth parameter. Specifically, we choose $h = \left(4\gamma \right)^{\frac{1}{\beta}}\left( \log |\cB_i| \right)^{-\frac{1}{\beta}}$, 
where $\beta$ and $\gamma$ are smoothness parameters for the noise $N$: cf. \eqref{eqn:model_supersmooth}.

%\subsubsection{Final Estimator $\tilde{\varphi}$}
\item Final Estimator $\tilde{\varphi}$: 
For each $i \in [m]$, let $\tilde{g}^{(i)} = \big(\tilde{F}^{(i)}\big)^{-1}$ denote the quantile function (right pseudo-inverse) 
associated with $\tilde{F}^{(i)}$. For $(i,j) \in [m] \times [n]$, we let
\begin{align}\label{eqn:estimate_noisy_known}
	\tilde{A}(i,j) & = \tilde{\varphi}(Z)(i,j) = \tilde{g}^{(i)}\left( \hat{q}_{\marg}(j) \right).	
\end{align}
\end{itemize}

Note that we cannot simply use $\hat{q}_i(j)$ -- the empirical quantile along a given row $i$ -- as a proxy of the latent column feature 
because the noise in data can corrupt the estimate, unlike noiseless setting. However, we can overcome the noise effect by ``averaging'' 
it out. To that end, we shall use empirical quantile estimation based on the ``averaged'' value, i.e., $Z_{\marg}(j)$. 

Also, when estimating $F^{(i)}$, we cannot simpy use the empirical CDF any longer because there is noise added in each entry.
Instead, we can view each entry $Z(i,j)$ in the row $i$ as a sum of two independent random variables: (i) $g(\frow{i}, \fcol{j})$ with 
the randomness induced by that in the column parameter $\fcol{j}$; and (ii) the additive noise $N(i,j)$. Therefore, the empirical CDF 
of the observations gives an estimated CDF for the sum of these two random variables. We are interested in recovering the distribution 
of the first random variable, hence, we shave off the second random variable by deconvolution.	




\subsection{Details for the Setup with Unknown Noise Distribution}\label{sec:alg_noisy_unknown}
When the noise distribution is not known a priori, the CDF estimate defined in \eqref{eqn:ECDF_known_noise} is no longer valid. 
It is because the deconvolution kernel $L$ is defined based on the knowledge of the noise characteristic function $\phi_N$; 
see \eqref{eqn:kernel_known_main}. To overcome the challenge of unknown noise distribution, we first estimate the noise 
characteristic function and then define a modified deconvolution kernel $\hat{L}$. Then we estimate the CDF using the modified 
deconvolution kernel in a similar manner, but with an additional ridge parameter $\rho$ to avoid division by zero. 
Note that the column feature estimation step in \ref{sec:alg_noisy_known} does not use any knowledge of the noise distribution, 
hence, $\hat{q}_{\marg}(j)$ defined in \eqref{eqn:estimate_marg} is a valid estimate even in the current setup.

\begin{itemize}
%\subsubsection{Column Feature Estimation}
\item Column Feature Estimation:
The same as described in Section \ref{sec:alg_noisy_known}.

%\subsubsection{CDF Estimation}
\item CDF Estimation:
%We estimate the distribution over each row by essentially same procedure as in Section \ref{sec:CDFest_noisy_known}. 
	\begin{enumerate}
%	\paragraph{Estimation of $\phi_N(t)$}
	\item Estimating $\phi_N(t)$:
	Recall that the characteristic function of the additive noise, $\phi_N$, is unknown and needs to be estimated from data.
	\begin{enumerate}
		\item 
		Construct set $\cT$ as described\footnote{Roughly speaking, $\cT$ is the set of index triples to mimic the setup 
		with repeated measurements, i.e., $\cT = \big\{ (i, j_1, j_2) \in [m] \times [n]^2: M(i, j_1) = M(i, j_2) = 1$ 
		$\text{ and }\hat{q}_{\marg}(j_1) \approx \hat{q}_{\marg}(j_2) \big\}$.} in Algorithm \ref{alg:setT_main}.
		\item 
		For each $i \in [n]$, define 
		\begin{equation}\label{eqn:set_Ti}
			\cT_i \triangleq \Big\{ (i',j_1, j_2) \in \cT: i' \neq i\Big\}.
		\end{equation}
		\item 
		For each $i \in [n]$, estimate the noise characteristic function $\phi_N$ as
		\begin{align}
			&\hat{\phi}_{N, i}(t) =			\label{eqn:chN_est}\\
			&\bigg| \frac{1}{\left| \cT_i \right|} \sum_{ \left(i, j_1, j_2 \right) \in \cT_i} 
				\cos \Big[ t \big( Z(i, j_1) - Z(i, j_2)  \big) \Big] \bigg|^{1/2}.	\nonumber
		\end{align}
	\end{enumerate} 
	For row $i$, we use $\cT_i$, which is a subset of $\cT$ tailored to exclude the data from row $i$. 
	This refinement of $\cT$ to $\cT_i$ for each row $i$ is done for the convenience in analysis.
				
	\begin{algorithm}%[H]
		\SetAlgoLined
		\KwResult{Return the set of triples $\cT$}
		$J \gets \left\{ j \in [n]: |\cB^j| \geq \frac{mp}{2}\right\}$\;
		$I \gets \left\{ i \in [m]: |\cB_i \cap J| \geq \frac{|J|p}{2}\right\}$\;
		
		$\cT \gets \emptyset$ \;
		Sort $j \in [n]$ in the increasing order of $\hat{q}_{\marg}(j)$, i.e., find a permutation $\pi$ such that $\hat{q}_{\marg}\left( j \right) \leq \hat{q}_{\marg}\left( j' \right)$ if $\pi(j) <\pi( j')$\;
		\For{$i \in I$}{
 			Renumber $j \in \cB_i \cap J$ with $j' \in \left[\left| \cB_i \cap J \right| \right]$ in the increasing order of $\hat{q}_{\marg}\left( j \right)$\;
			(let $\sigma_i: \cB_i \cap J \subseteq [n] \to \left[\left| \cB_i \cap J \right| \right]$; this map can be induced from $\pi$)\\
			$j' \gets 0$\;
			\While{$j' \leq \left| \cB_i \cap J \right| - 1 $}{
			\eIf{$\hat{q}_{\marg}\left( \sigma_i^{-1} (j' + 1)\right) - \hat{q}_{\marg}\left( \sigma_i^{-1} (j')\right) \leq \frac{1}{\sqrt{\left| \cB_i \cap J \right|}}$}{
				$\cT \gets \cT \cup \left\{ (i, \sigma_i^{-1}\left(j'\right), \sigma_i^{-1}(j'+1)) \right\}$\;
				$j' \gets j' + 2$\;
			}{
				$j' \gets j' + 1$\;
			}
			}
 		}
		\caption{Construction of the set $\cT$.}
		\label{alg:setT_main}
	\end{algorithm}
	
%	\paragraph{Estimating $F^{(i)}$}
	\item Estimating $F^{(i)}$:
	Let $K$ be a symmetric Kernel with $\phi_K$ being its Fourier transform such that $\supp \phi_K \subset [-1,1]$. 
	For $i \in [m]$, we define a modified deconvolution kernel
	\begin{equation}\label{eqn:kernel_estimated}
		\deconvker(z) = \frac{1}{2\pi} \int e^{-\img tz} \frac{\phi_K(t)}{\hat{\phi}_{N,i}\left(\frac{t}{h}\right) + \rho}dt.	
	\end{equation}
	Here, the ridge parameter $\rho > 0$ is introduced to avoid division-by-zero. In this paper, we specifically choose $\rho = |\cB_i|^{-7/24}$ for our analysis. 
	
	Suppose two constants $\tfmin, \tfmax$ such that $\tfmin \leq \fmin$ and $\tfmax \geq \fmax$ are given. Let
	\begin{equation}\label{eqn:ECDF_unknown_noise}
		\hat{F}^{(i)}(z) = \begin{cases}
			\int_{\tfmin}^{z } \hat{f}^{(i)}(w) dw,	& \text{if } z < \tfmax,\\
			1,							& \text{if } z \geq \tfmax,
		\end{cases}
	\end{equation}
	where
	\begin{equation}\label{eqn:unknown_density}
		\hat{f}^{(i)}(z) = \frac{1}{h |\cB_i|} \sum_{j\in \cB_i} \deconvker \left( \frac{z- Z(i,j)}{h} \right).
	\end{equation}
	Here $h$ denotes the kernel bandwidth parameter. Specifically, we choose 
	$h = \left(4\gamma\right)^{\frac{1}{\beta}} \left( \log \left| \cB_i \right| \right)^{-\frac{1}{\beta}}$ where $\beta$ and $\gamma$ are 
	smoothness parameters for the noise $N$: cf. see \eqref{eqn:model_supersmooth}.  	
	\end{enumerate}

%\subsubsection{Final Estimator $\hat{\varphi}$} 
\item Final Estimator $\hat{\varphi}$:
For each $i \in [m]$, let $\hat{g}^{(i)} = \big(\hat{F}^{(i)}\big)^{-1}$ denote the quantile function (right pseudo-inverse) associated with $\hat{F}^{(i)}$. 
For $(i,j) \in [m] \times [n]$, we let 		
\begin{equation}\label{eqn:estimate_noisy_unknown}
	\hat{A}(i,j) = \hat{\varphi}(Z)(i,j) = \hat{g}^{(i)}\left( \hat{q}_{\marg}(j) \right).	
\end{equation}
\end{itemize}

\begin{remark}
We wish to recover distribution of random variable $X$, but we observe samples of $Z = X + N$ instead of $X$. And we do not know 
the distribution of $N$. Due to independence, we know that $\phi_Z(t) = \phi_X(t) \phi_N(t)$ for all $t \in \Reals$, where $\phi_Z, \phi_X, \phi_N$ 
denote the characteristic function of random variable $Z, X$ and $N$ respectively. To overcome the challenge of unknown noise distribution, 
we estimate the noise characteristic function first and then estimate the CDF using kernel deconvolution, but with an additional ridge parameter 
to avoid division by zero.
\end{remark}


\begin{remark}
We produce estimated characteristic function $\hat{\phi}_{N, i}(t)$ for noise distribution using pairs of `similar' 
observations from rows $i' \in [m] \setminus i$. To begin with, suppose that we can repeatedly observe the same instance 
$X_i$ of target random variable up to independent additive noise, i.e., $Z_{ij} = X_i + N_{ij}$ with $N_{ij}$ independent. 
Although we don't know the value of $X_i$, we can see that the difference in the observed data entries is equal to the difference 
between two independent noise instances: $Z_{i1} - Z_{i2} = \left( X_i + N_{i 1} \right) - \left( X_i + N_{i2}\right) = N_{i1} - N_{i2}$. 
Assuming symmetry in the noise distribution, $N_{i1} - N_{i2} \equiv N_{i1} + N_{i2}$. Therefore, $\phi_{N_{i1} - N_{i2}}(t) = \phi_N(t)^2$.
From symmetry of $N$, we know that $\phi_N(t)$ is real-valued. Moreover, it is positive because $N$ is supersmooth. Therefore, 
we can estimate $\phi_N(t)$ by taking square root of the (absolute value of the) estimate $\hat{\phi}_{N_1 - N_2}(t)$ as
\[
	\hat{\phi}_N(t) = \hat{\phi}_{N_1 - N_2}(t)^{\frac{1}{2}} 
	= \bigg| \frac{1}{n} \sum_{i=1}^n \cos \big[ t (N_{i1} - N_{i2} ) \big] \bigg|^{\frac{1}{2}}.
\]
However, the repeated measurement assumption is not feasible because we have {\em at most} one measurement for a given index 
$(i, j)$. Despite this challenge, we can still hope to obtain {\em nearly} repeated samples from observations in a given row, 
if we choose columns $j_1, j_2 \in [n]$ that have {\em very} similar features $\fcol{j_1} \approx \fcol{j_2}$ so that
\begin{align*}
	&Z(i,j_1) - Z(i,j_2)\\
		&\qquad= \underbrace{ \left[ A(i, j_1) - A(i,j_2) \right] }_{\approx 0,~ \because \fcol{j_1} \approx \fcol{j_2} } + \left[ N(i,j_1) - N(i,j_2) \right]\\
		&\qquad \approx N(i,j_1) - N(i,j_2). 	
\end{align*}
Intuitively, $\cT$ is the set of index triples to imitate the repeated measurements. 
\end{remark}



==> contents/04_upper_bounds.tex <==
\section{Upper Bounds: Details for Theorems \ref{thm:simple_noiseless}, \ref{thm:simple_known}, \ref{thm:simple_unknown}}	\label{sec:upper_bounds}

\subsection{Notation Used in Our Analysis}\label{sec:notation_constants}
Recall that $\fmax, \fmin, \lipmax, \lipmin$ are model parameters associated with $A$ (and hence, with $g$). 
We let $\frange \triangleq \fmax - \fmin$ denote the range of the latent function $g$. 
Also, there are model parameters $B, \beta, \gamma$ for the noise $N$; see \eqref{eqn:model_supersmooth}.
Recall that we utilize a kernel $K$ in our algorithm for noisy setup; see Sections \ref{sec:alg_noisy_known} and 
\ref{sec:alg_noisy_unknown}. Let $\phi_K$ denote the Fourier transform of $K$. Since $\phi_K$ is assumed 
to have compact support within $[-1, 1]$, and the Fourier transform of $L^1$ function is uniformly continuous, 
there exists $\kmax = \max_{t \in [-1,1]} \left| \phi_K(t) \right| < \infty$.

Our theorem statements contain various constants that depend on the model parameters. We summarize those constants below 
for quick reference:
\begin{align}
	\constcc &= C(\lipmin),	\qquad\text{see Lemma \ref{lem:mean_difference_tilde}}			\label{eqn:const_3}\\
	\constdd &= \frac{ B K_{max} \frange }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} },			\label{eqn:const_4}\\
%	\constee &= 2\sqrt{\pi} \left( \frac{\sqrt{2} + \exp\big(\frac{\constaa}{2}\big)}{\sqrt{\constaa}} 
%			+\frac{\sqrt{2} + \exp\big(\frac{\constbb}{2}\big)}{\sqrt{\constbb}} \right)
	\constee &= \frac{2\sqrt{2\pi}}{\lipmin} \bigg[ \frange \bigg( \sqrt{2} + \exp \Big( \frac{\lipmin^2}{4 \frange^2} \Big) \bigg) \nonumber\\
			&\qquad\qquad\qquad+ 2 \sigma \bigg( \sqrt{2} + \exp \Big( \frac{\lipmin^2}{16 \sigma^2} \Big) \bigg)  \bigg].		\label{eqn:const_5}
\end{align}
Note that $\constcc, \constdd, \constee$ do not depend on $m, n, p$.
%
%Also, we need some quantities depending on $m, n, p$, we let them be denotedy by $\ftnaa$, etc.

%%% ===============================================================
%%%	Noiseless setup
%%% ===============================================================
\subsection{Noiseless Setup: Full Version of Theorem \ref{thm:simple_noiseless}}
%We start by establishing two key results needed for establishing proof of Theorem \ref{thm:simple_noiseless}. To that end, 
%note that $\hat{q}_i(j)$ is the average of $\sum_{j' = 1}^n M(i,j')$ independent random variables as per our model. 
%Therefore, by Chernoff bound, for each $i$, it concentrates around its 
%expectation, which is the true parameter $\fcol{j}$ of interest. This explain
%the choice of \eqref{eqn:quantile_rowwise}-\eqref{eqn:quantile_est}. This is
%summarized in Lemma \ref{lem:quantile_noiseless}. 
%		
%By definition, $\breve{F}^{(i)}$ is simply the empirical cumulative distribution function. Hence, by 
%Glivenko-Cantelli theorem, it follows that it is a consistent estimator for $F^{(i)}$. Using the Dvoretzky-Kiefer-Wolfowitz 
%inequality (see Appendix \ref{appx:distribution}, Lemma \ref{lem:DKW}), we obtain concentration of $\breve{F}^{(i)}$
%around $F^{(i)}$. This is summarized in Lemma \ref{lem:noiseless_CDF}.
%
%We obtain a probabilistic tail bound by applying the union bound on the aforementioned concentration results. 
%Integrating the tail bounds leads to the following theorem.

\begin{theorem}[Main theorem 1; noiseless]\label{thm:MSE_noiseless}
Given $Z \in \Reals^{m \times n}$, let $\breve{\varphi}$ be defined as in \eqref{eqn:estimate_noiseless}. Then
\begin{align*}
	\MSE\left( \breve{\varphi} \right) 
		&\leq \frac{18 \lipmax^2 \exp\left(\frac{2}{9\lipmax^2}\right)}{(n-1)p }\\
		&\quad + 2  \frange^2 \exp(-mp)\\
		&\quad + 4  \frange^2 \exp\left( -(n-1)p \left( 1 - \exp \Big(-\frac{2}{9\lipmax^2}\Big) \right)\right).
\end{align*}
\end{theorem}
We sketch the proof in Section \ref{sec:proof_sketch} and the full details of the proof can be found in Appendix \ref{sec:full_proof_noiseless}.


\subsection{Noisy Setup with Known Noise Distribution: Full Version of Theorem \ref{thm:simple_known}}

\begin{theorem}[Main theorem 2; known noise]\label{thm:MSE_noisy_known}
Given $Z \in \Reals^{m \times n}$, let $\tilde{\varphi}$ be defined as in \eqref{eqn:estimate_noisy_known}. Then
\begin{align*}
	\MSE\left( \tilde{\varphi} \right)
	&\leq  16(\constcc + \constdd)^2 \lipmax^2 \left( \log \frac{np}{2} \right)^{-2/\beta}\\
		&\quad	+ 64\sqrt[4]{8} \constdd^2 \lipmax^2 \frac{\left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}}{(np)^{\frac{1}{4}}} + \frac{64 \constee^2 \lipmax^2}{mp}\\
		&\quad 	+  8\lipmax \constee \sqrt{\frac{3\lipmax \pi}{mnp}}	+ \frac{8\lipmax^2}{n} + \frac{288\lipmax^2}{n^2} \\
		&\quad	+ \big( \tfmax - \tfmin \big)^2 \left[ \exp\left( - \frac{mp}{8}\right)  + 2 \exp\left( - \frac{np}{8}\right) \right].
\end{align*}
\end{theorem}

First of all, we note that $\MSE\left( \tilde{\varphi} \right) \to 0$ as $m, n \to \infty$ as long as the sample complexity satisfies 
$p = \omega \Big(\max \big\{ \frac{1}{m}, \frac{1}{n}\big\}\Big)$. 
Also, we observe that the first term, i.e., $16(\constcc + \constdd)^2 \lipmax^2 \left( \log \frac{np}{2} \right)^{-2/\beta}$, is the leading term 
in the MSE upper bound and the other terms decay faster unless the matrix is highly imbalanced so that $mp = \cO\left( \log np \right)$. 
This MSE bound achieves the asymptotically optimal rate of convergence as long as $mp = \omega(\log np)$.
	
We sketch the proof in Section  \ref{sec:proof_sketch} and the full details of the proof can be found in Appendix \ref{sec:full_proof_noisy_known}.


\subsection{Noisy Setup with Unknown Noise Distribution: Full Version of Theorem \ref{thm:simple_unknown}}
By the complicated nature of our proof, there are many terms that appear in the upper bound of $\MSE(\hat{\varphi})$. 
To minimize readers' confusion in appreciating the convergence rate of our upper bound in Theorem \ref{thm:MSE_noisy_unknown}, 
we define six quantities: $\valphiAA, \valphiBB, \slackAA, \slackBB, \slackCC$ and $C_{m,n,p}$.


%
Then we define three slack constants
\begin{align}
	\slackAA 	&= \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  \frac{\left( \log (2np) \right)^{\frac{1}{\beta}}}{\big(\frac{np}{2} \big)^{\frac{17}{24}}},		\label{eqn:slackA}\\
	\slackBB 	&= \constcc \bigg( \log \Big(\frac{np}{2}\Big)\bigg)^{-\frac{1}{\beta}},	\label{eqn:slackB}\\
	\slackCC 	&=  \frac{2B \kmax(\tfmax - \tfmin)}{ \pi (4\gamma)^{\frac{1}{\beta}} } \frac{(\log (2np))^{\frac{1}{\beta}}}{ \big(\frac{np}{2} \big)^{\frac{1}{24}}} \nonumber\\
		&\quad\times \Big( 1 + ( 2np )^{\frac{7}{24}} \big( \valphi \big) \Big) ,		\label{eqn:slackC}
\end{align}
%
Lastly, we define a symbol to denote the residual terms.
\begin{align}
	C_{m,n,p} 
		&\triangleq	 \frac{256}{mnp} + n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)	\nonumber\\
		&\quad + \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg) 		\nonumber\\
		&\quad + \exp \left( - \frac{mnp}{3} \right) + \exp\left( - \frac{mp}{8} \right).	\label{eqn:Cmnp}
\end{align}
%
\begin{remark}\label{rem:slacks}
We observe that 
\begin{align*}
	\slackAA &= \cO \Big( \big( np \big)^{-\frac{17}{24}} \log^{\frac{1}{\beta}}(np) \Big),\\
	\slackBB &= \cO \Big( \log^{-\frac{1}{\beta}} (np) \Big),\\
	\slackCC &= \cO \Big( \big( np \big)^{-\frac{1}{24}} \log^{\frac{1}{\beta}}(np)\Big).
\end{align*}
\end{remark}

%%% ================

\begin{theorem}[Main theorem 3; unknown noise]\label{thm:MSE_noisy_unknown}
Given $Z$, let $\hat{\varphi}$ be defined as in \eqref{eqn:estimate_noisy_unknown}. Then 
\begin{align*}
	\MSE\left( \hat{\varphi} \right)
	&\leq  16 \lipmax^2 \big( \slackAA + \slackBB + \slackCC \big)^2 	 +  4\sqrt{2} \constdd^2  \frac{ \big( \log (2np) \big)^{\frac{2}{\beta}} }{ ( np )^{5/12}}\\
	&\quad 
		+ 8\lipmax \constee \sqrt{\frac{3\lipmax \pi}{mnp}} + \frac{64\lipmax^2 \constee^2}{mp} \\
	&\quad
		+  \frac{8\lipmax^2}{n} + \frac{288\lipmax ^2}{n^2} + C_{m,n,p} \big( \tfmax - \tfmin \big)^2.
\end{align*}
%The upper bound diminishes to $0$ as $mp, np \to \infty$ at the rate of $(\log np )^{-\frac{2}{\beta}}$.
\end{theorem}

\begin{remark}
We remark that $16\lipmax^2{\slackBB}^2$ is the asymptotically dominant term in the MSE upper bound stated in 
Theorem \ref{thm:MSE_noisy_unknown}. The leading term scales as $O \big( (\log np )^{-\frac{2}{\beta}} \big)$ and 
all the other terms decay at least at polynomial rate in the least. 
\end{remark}

We sketch the proof in Section \ref{sec:proof_sketch} and the full details of the proof can be found in Appendix \ref{sec:full_proof_noisy_unknown}.



==> contents/05_lower_bounds.tex <==
\section{Lower bounds: Details for Theorems \ref{thm:optimal_noiseless} and \ref{thm:optimal_deconvolution} }	\label{sec:lower_bounds}



\subsection{Proof of Theorem \ref{thm:optimal_noiseless}: Lower Bound on Function Approximation without Noise}\label{sec:noiseless_LB}
In this section, we show that for any slice of true latent function $g_1:= g(\frow{1}, \cdot) : [0,1] \to \Reals$ and for any set of sampling points $y_1, \ldots, y_{\nu} \in [0,1]$, 
there exists an adversarial function $g_1^{\dagger}: [0,1] \to \Reals$ such that $g_1(y) = g_1^{\dagger}(y)$ for all $y \in \{y_1, \ldots, y_\nu\}$, 
yet $\| g_1 - g_1^{\dagger} \|_2^2 \geq \frac{c}{\nu}$ for some universal constant $c$, independent of $g_1$ and $\nu$. 
This claim follows from a classical result in function approximation theory.

We define some notations before introducing the function approximation lemma.
Recall that the $L^1$ norm of a function $g: [0,1] \to \Reals$ is defined as $\| g \|_{L^1[0,1]} := \int_0^1 | g(x)| dx$ (see Eq. \eqref{eqn:L2_I} for comparison with $L^2$ norm).
We let $L^1[0,1] := \left\{ g: [0,1] \to \Reals: \| g \|_{L^1[0,1]} < \infty \right\}$ denote the space of functions with finite $L^1$ norm, i.e., integrable functions.
We also recall that $C^{\infty}[0,1]$ is the space of functions defined on $[0,1]$, which are infinitely differentiable. Lastly, we call a function 
$g$ to be $\delta$-Lipschitz if $\| g(y_1) - g(y_2) \| \leq \delta \| y_1 - y_2 \|$ for any two points $y_1, y_2$ in the domain of $g$.

\begin{lemma}[\citet{Kudryavtsev1995}, Lemma 4.4, simplified]\label{lem:Kudryatsev}
	There exists a universal constant $c$ such that for every $\nu \in \Nats$, and for any $y_1, \ldots, y_{\nu} \in [0,1]$, there exists a $\delta$-Lipschitz function $h \in L^1[0,1] \cap C^{\infty}[0,1]$ for which 
	\begin{enumerate}
		\item	$h(y_i) = 0$, for all $i=1, \ldots, \nu$, and
		\item	$\left\| h \right\|_{L^2[0,1]} \geq c \frac{\delta}{\sqrt{\nu}}$.
	\end{enumerate}
\end{lemma}

We use this lemma to prove the following theorem, which is the full version of Theorem \ref{thm:optimal_noiseless}. The proof of Theorem 
\ref{thm:optimal_noiseless} can be found in Appendix \ref{sec:noiseless_LB_proof}.

\begin{theorem}[Full version of Theorem \ref{thm:optimal_noiseless}]\label{thm:noiseless_LB}
	In the noiseless scenario, for any estimation algorithm $\varphi$, there exists a hard instance for which
	$$	\MSE(\varphi) \geq (1-p)	 \frac{c^2 \delta^2}{ (n-1)p}.	$$
\end{theorem}



\subsection{Proof of Theorem \ref{thm:optimal_deconvolution}: Lower Bound on Function Approximation with Noise}\label{sec:noisy_LB}



We use Lemma \ref{lem:deconv_hard} to prove Theorem \ref{thm:noisy_LB}, which is the full version of Theorem \ref{thm:optimal_deconvolution}. 
The proof of Theorem \ref{thm:noisy_LB} can be found in Appendix \ref{sec:noisy_LB_proof}.
\begin{theorem}[Full version of Theorem \ref{thm:optimal_deconvolution}]\label{thm:noisy_LB}
	In the additive noise scenario, for any estimation algorithm $\varphi$, there exists a hard instance for which
	\[	\MSE(\varphi) \geq \frac{(1-p) \lipmin^2 c^{3/2}}{6 \sqrt{2}}	\big( \log  (n-1)p \big)^{-3 / \beta}.	\]
\end{theorem}


==> contents/06_proof_idea.tex <==
\section{Sketch of the Proofs}\label{sec:proof_sketch}
\DG{resume here}
In this section, we briefly explain the reasons why our algorithm works and sketch the proofs of Theorems \ref{thm:MSE_noiseless}, 
\ref{thm:MSE_noisy_known} and \ref{thm:MSE_noisy_uhknown}. Basically we argue that each of the three steps 
in the algorithm succeeds. The full proof can be found in Appendices. The technicalities in the proofs might be interesting 
to some readers in its own right.

\subsection{Outline of the Proof}
\subsubsection{Step 1 Works}
Our column feature estimator is effectively a quantile estimator, which compares the matrix entry value with the others 
in the same row to estimate the ranking of each column. Due to the independence, this estimate concentrates to the true 
column feature with dispersion of order reciprocal to the square root of the number of observed entries.

In the noisy scenarios, direct comparison between raw matrix entries is not reliable because of the noise. We first take 
average over the columns and compare these averaged values in the same manner as above. The co-monotonicity assumption 
on the matrix -- there exists a column permutation which makes the matrix monotone increasing with respect to its column index --
enables this average-and-ranking approach. Note that this co-monotonicity is described in terms of the latent function in 
Eq. \eqref{eqn:biLipschitz}. Again, by the concentration of measure, we expect to achieve $O(1/\sqrt{n})$ concentration of 
this column feature estimator.

\subsubsection{Step 2 Works}
We estimate the latent function, or to be more precise, the cumulative distribution function of the pushforward measure 
by the latent function, in step 2 of our algorithm. When there is no noise, the empirical distribution is known to be a consistent 
estimator and we can achieve the convergence rate of $O(1/\sqrt{np})$ by Dvoretzky-Kiefer-Wolfowitz theorem.

When there is nontrivial noise with known distribution, we estimate the CDF by the kernel deconvolution estimator. 
Following the algorithm and analysis by Fan \cite{Fan1991}, we can obtain the convergence rate of $O(1/(\log(np))^{-2/\beta})$ 
for the super-smooth class of noise; Gaussian noise a member of this class with $\beta = 2$.

When there is nontrivial noise with unknown distribution, we estimate the CDF by the kernel deconvolution estimator with ridge parameter. 
Our analysis has some similarity with that of \cite{Delaigle2008}, but is much more detailed in the error analysis of $\hat{\phi}_N$. 
The estimated noise characteristic function $\hat{\phi}_N(t)$ uniformly converges to the true characteristic function $\phi_N(t)$, again 
by the concentration of measure. However, in order to formally prove the convergence rate of it, we needed to exploit many clever tricks, 
such as refined uses of concentration inequalities, conditioning on a high-probability-event and taking union bounds, $\varepsilon$-net 
argument, etc. 

\subsubsection{Step 3 Works}
From our analysis described above, we obtain a probabilistic tail bound on the error in the column feature estimation for column $j \in [n]$ 
and one on the error in the CDF estimation for row $i \in [m]$. By the bi-Lipschitz assumption, this probabilistic tail bound can be rewritten 
as one for the latent function estimation at the expense of a constant discount factor $\frac{1}{\lipmin}$. The tail upper bound for column feature estimation and the tail upper bound for latent function estimation are combined to yield a tail bound on the error in matrix entry estimation 
at $(i,j)$-th entry, by taking their union bounds. Integrating this tail bound from $0$ to $\infty$ with a proper change of variables, we establish 
an upper bound for the mean-squared error at $(i,j)$-th entry. Due to the exchangeability of data matrix, this provides an upper bound on the 
MSE defined in Eq. \eqref{eqn:MSE}.


\subsection{Supporting Lemmas of Theorems \ref{thm:MSE_noiseless}, \ref{thm:MSE_noisy_known}, and \ref{thm:MSE_noisy_unknown}}
\subsubsection{Quantile Estimation}



\subsubsection{CDF Estimation}
%\paragraph{Noiseless}



\subsubsection{Conditioning with High-probability Events}

We state a useful consequence of the above result. To that end, for any $i \in [m]$, define 
\begin{align}
	\Erow &\equiv \Big\{ |\cB_i| \geq \frac{np}{2}\Big\}	%\nonumber\\
			\text{~and~} \Erowp \equiv \Big\{ |\cB_i| \leq 2np\Big\}.	\label{eqn:sufficient_overlap}
\end{align}
In addition, for each $j \in [n]$, we define
\begin{align}\label{eqn:sufficient_overlap.col}
	\Ecol &\equiv \left\{|\cB^j| \geq \frac{mp}{2} \right\}.
\end{align}


\subsection{Proof Sketches}
\DG{TODO: fill this in}
\subsubsection{Proof Sketch of Theorem \ref{thm:MSE_noisy_unknown}}

==> contents/AA_background.tex <==
\section{Background and Intuition Behind the Algorithm}\label{sec:background}

\subsection{Kernel Deconvolution Estimator}
Putting it other way, we wish to recover distribution of random variable $X$, but we observe samples of
$Z = X + N$ instead of $X$. And we do know distribution of $N$. Due to independence, we know 
that $\phi_Z(t) = \phi_X(t) \phi_N(t)$ for all $t \in \Reals$, where $\phi_Z, \phi_X, \phi_N$ 
denote the characteristic function of random variable $Z, X$ and $N$ respectively. 

Since we know noise distribution, equivalently $\phi_N(\cdot)$, if we can estimate $\phi_Z(\cdot)$ from
observations, say $\hat{\phi}_Z(\cdot)$, then we can ``de-convolve'' it to obtain estimation $\phi_X(\cdot)$ as
\begin{align*}
\hat{\phi}_X(t) & = \frac{\hat{\phi}_Z(t)}{\phi_N(t)}, ~~t \in \Reals.
\end{align*}
Now to produce estimate $\hat{\phi}_Z(\cdot)$, the first step is a non-parametric estimator of distribution
of $Z$. The Kernel smoothing is a well-studied non-parametric approach which would attempt to 
estimate the density (which exists in our setting) through interpolation. Precisely,  given a kernel 
$K: \Reals \to \Reals_{\geq 0}$ and bandwidth parameter $h > 0$, the density of $Z$ is estimated as
\begin{align}\label{eq:kernel.0}
\hat{f}_Z(z) & = \frac{1}{hn} \sum_{i=1}^n K\left( \frac{z - Z_i}{h} \right), ~~ z \in \Reals.
\end{align}
{ Denote Fourier transformation operator $\cF: L^1(\Reals) \to C_b(\Reals)$ which maps the space of absolutely integrable functions $L^1(\Reals)$ to the space of continuous bounded functions. 
Recall that $\cF$ maps $f \in L^1(\Reals)$ to $\cF\{f\} \in C_b(\Reals)$
where for all $t \in \Reals$,
\[	\cF\Big\{f \Big\}(t)  = \int_{-\infty}^\infty \exp( \img\, t s) f(s) ds.	\]
We use notation $\img \equiv \sqrt{-1}$.
}
Similarly, for any absolutely integrable function $g \in L^1(\Reals)$ and for all $s \in \Reals$, it is possible to define an operator $\cF^{-1}: L^1(\Reals) \to C_b(\Reals)$ as
\[	\cF^{-1}\Big\{ g \Big\}(s) = \frac{1}{2\pi}\int_{-\infty}^\infty \exp(- \img\, t s) g(t) dt. 	\]

The Fourier inversion theorem ensures that $\cF^{-1} \cF f = f$ if $f$ satisfies certain conditions. For example, if the function is absolutely integrable and piecewise continuous (which is the case in our model), then $\cF^{-1} \left( \cF f \right) (s) = \frac{1}{2}\left( f(s_-) + f(s_+) \right)$.


Applying Fourier operator to \eqref{eq:kernel.0} and using linearity of $\cF$, we obtain 
\begin{align*}	
\hat{\phi}_Z(t) & = \cF \left\{ \hat{f}_Z \right\} 
		      = \frac{1}{hn} \sum_{i=1}^n \cF \left\{ K \left( \frac{\cdot - Z_i}{h}\right) \right\}.
\end{align*}
Now, applying inverse Fourier operator, $\cF^{-1}$, to $\hat{\phi}_Z/\phi_N$ we obtain 
\begin{align}
	\hat{f}_X &= \cF^{-1} \left\{ \frac{\hat{\phi}_Z}{\phi_N} \right\} \nonumber \\
		&= \frac{1}{hn} \sum_{i=1}^n \cF^{-1} \left\{ \frac{\cF \left\{ K \left( \frac{\cdot- Z_i}{h}\right) \right\}}{\phi_N} \right\} \nonumber \\
		&= \frac{1}{hn} \sum_{i=1}^n \cF^{-1} \left\{ \frac{ h \exp( \img\, Z_i \, \cdot \,) \phi_K(h\, \cdot\,)}{\phi_N} \right\}, \label{eq:kernel.1}
\end{align}
where we used the following properties of Fourier operator:
\begin{align*}
	\cF\left\{ f(\cdot - a) \right\}(t) & = \exp(\img\, a \, t) \cF\{ f\}(t) \\
	\cF\left\{ f( b \, \cdot \, ) \right\}(t) & = \frac{1}{|b|} \cF\left\{ f(\cdot)  \right\}\left( \frac{t}{b} \right).
\end{align*}
Applying similar properties to inverse Fourier operator, $\cF^{-1}$, we obtain
\begin{align}\label{eq:kernel.2}
	\cF^{-1} \left\{ \frac{ h  \exp( \img\, Z_i \, \cdot \,) \phi_K(h\, \cdot\,)}{\phi_N(\, \cdot \,) } \right\} (x), 
	& =  \cF^{-1} \left\{ \frac{ \phi_K(\, \cdot \,) }{\phi_N(\, \cdot \, h^{-1})} \right\} \left( \frac{x - Z_i}{h} \right). 
\end{align}
Define function $L$ as 
\begin{align}\label{eqn:kernel_known}	
L & \equiv  \cF^{-1} \left\{ \frac{ \phi_K(\, \cdot \,) }{\phi_N(\, \cdot \, h^{-1})} \right\}, \quad \text{i.e.,} \quad
L(z) = \frac{1}{2\pi} \int \exp(- \img\, t z ) \frac{\phi_K(t)}{\phi_N\left(\frac{t}{h}\right)} dt, ~~z \in \Reals.
\end{align}
From \eqref{eq:kernel.1} and \eqref{eq:kernel.2}, and definition of $L$, we obtain 
\begin{align}\label{eq:kernel.4}
				\hat{f}_X(x) &= \frac{1}{hn} \sum_{i=1}^n L\Big(\frac{x - Z_i}{h}\Big).
\end{align}
Indeed, this is known as deconvolution kernel density estimator in literature. We shall 
adopt prior results  \citet{Carroll1988, Fan1991, Delaigle2008} on its consistency to establish our 
results. Appendix \ref{appx:deconvolution} provides their summary.


\begin{remark}[Constraints on kernel $K$]\label{rem:kernel}  We choose kernel $K$ to satisfy the following conditions:
\begin{itemize}
\item[1.] It is symmetric, i.e. $K(x) = K(-x)$ for all $x \in \Reals$.
\item[2.] $\sup_{t \in \Reals} \left| \phi_K(t) \right| < \infty$.
\item[3.] Support of $\phi_K$ is assumed to be within $[-1, 1]$. 
For $K \in L_1(\Reals)$, $\cF\{K\}$ is uniformly continuous, so there exists 
$K_{max}=\max_{t \in [-1,1]} \left| \phi_K(t) \right| < \infty$.
\end{itemize}
\end{remark}


\subsection{Kernel Deconvolution with a Ridge Parameter: When the Noise Distribution is Unknown}
Since the noise distribution is unknown, we need an auxiliary procedure to estimate the noise density. Here we explain an algorithm to estimate the noise characteristic function $\hat{\phi}_N(t)$.

Suppose that we can repeatedly observe the same instance $X_i$ of target random variable up to independent additive noise, i.e., $Z_{ij} = X_i + N_{ij}$ with $N_{ij}$ independent. Although we don't know the value of $X_i$, we can see that the difference in the observed data entries is equal to the difference between two independent noise instances: $Z_{i1} - Z_{i2} = \left( X_i + N_{i 1} \right) - \left( X_i + N_{i2}\right) = N_{i1} - N_{i2}$. Assuming symmetry in the noise distribution, $N \equiv -N$ in distribution, and $N_{i1} - N_{i2}$ follows the same distribution with the sum of two independent copies of noise: $N_{i1} - N_{i2} \equiv N_{i1} + N_{i2}$. Therefore, $\phi_{N_{i1} - N_{i2}}(t) = \phi_N(t)^2$.

From symmetry of $N$, we know that $\phi_N(t)$, the Fourier transform of the noisy density is real-valued. 
In fact, we know $\phi_N(t)$ is not only real-valued but positive from the model assumption of the supersmooth noise (see Eq. \eqref{eqn:model_supersmooth}).
It implies $\phi_{N_1 - N_2} (t) = \phi_N(t)^2$ is also positive real-valued. Hence,
\begin{align*}
	\phi_{N_1 - N_2} (t) &= \Exp{e^{\img t (N_1 - N_2)}}\\
		&=  \Exp{\frac{e^{\img t (N_1 - N_2)} + e^{-it (N_1 - N_2)}}{2}}\\
		&= \Exp{ \cos t (N_1 - N_2)}.
\end{align*}
			
Therefore, we can estimate $\phi_N(t)$ by taking square root of the (the absolute value of) estimate $\hat{\phi}_{N_1 - N_2}(t)$, which is computed as the sample-analog estimator with $n$ independent copies of noise difference $\{ N_{i1} - N_{i2}\}_{i=1}^n$. 
Specifically,
\[	\hat{\phi}_N(t) = \hat{\phi}_{N_1 - N_2}(t)^{\frac{1}{2}} = \left| \frac{1}{n} \sum_{i=1}^n \cos \left[ t\left(N_{i1} - N_{i2}\right) \right] \right|^{\frac{1}{2}}.	\]
			
However, the repeated measurement assumption may not be realistic, because we may not be allowed to measure the same entry multiple times. 
Therefore, we imitate the setup of repeated measurements by considering two columns $j_1, j_2 \in [n]$ with similar column features $\fcol{j_1} \approx \fcol{j_2}$ so that
\begin{align*}
	Z(i,j_1) - Z(i,j_2) &= \left[ A(i, j_1) + N(i,j_1) \right] - \left[ A(i,j_2) + N(i,j_2) \right]\\
		&= \underbrace{ \left[ A(i, j_1) - A(i,j_2) \right] }_{\approx 0,~ \because \fcol{j_1} \approx \fcol{j_2} } + \left[ N(i,j_1) - N(i,j_2) \right]\\
		& \approx N(i,j_1) - N(i,j_2). 	
\end{align*}


==> contents/BB_proof_lower_bound.tex <==
\section{Deferred Proofs from Section \ref{sec:lower_bounds}: Information-theoretic Lower bounds on CDF Estimation}	\label{sec:proof_lower_bounds}

\subsection{Proof of Theorem \ref{thm:noiseless_LB}}\label{sec:noiseless_LB_proof}
\begin{proof}
	Choose a positive real number $\delta < \frac{\lipmax - \lipmin}{2}$. Consider a bounded function $g: [0,1]^2 \to \Reals$, which is 
	$(\lipmin + \delta, \lipmax - \delta)$ bi-Lipschitz with respect to the second argument.
	We suppose that given any data $\{ \frow{1} \}$, $\{ \frow{j} \}_{j \in [n]}$, $\{ g( \frow{1}, \fcol{j}): j \in [n] \text{ and } M(1,j) = 1 \}$, algorithm $\varphi$ can perfectly restore the function $g(\frow{1}, \cdot)$ from data.
	
	Let $\nu := \sum_{j = 2}^n M(1,j)$ denote the number of samples observed.
	By Lemma \ref{lem:Kudryatsev}, there exists a $\delta$-Lipschitz function $h \in L^1[0,1] \cap C^{\infty}[0,1]$ which satisfies
	\begin{enumerate}
		\item	$h( \fcol{j} ) = 0$, for all $j \in [n]$ such that $M(1,j) =1$, and
		\item	$\left\| h \right\|_{L^2[0,1]} \geq c \frac{\delta}{\sqrt{\nu}}$.
	\end{enumerate}
	Now we consider an adversarial function $g^{\dagger}: [0,1]^2 \to \Reals$ (for given data), which is defined as
	\[	g^{\dagger}(x, y) = g(x,y) + h(y)\Ind{x = \frow{1}}.	\]

	First of all, we remark that $g^{\dagger}$ is a valid latent function which satisfies every criterion in our model (see Section \ref{sec:model}), because $h$ is continuous and $\delta$-Lipschitz.
	If the latent function $g$ were replaced with $g^{\dagger}$ by an adversary, the algorithm $\varphi$ could not recognize that from given data because $h( \fcol{j} ) = 0$, for all $j \in [n]$ such that $M(1,j) =1$.
	Therefore, $\varphi$ would still return $\gphi = g$ instead of yielding $\gphi = g^{\dagger}$ even though the true latent function is now $g^{\dagger}$.
	
	This leads to the following lower bound, regardless of $\frow{1} \in [0,1]$:
	\begin{align*}
		\big\|	 \gphi_{\nu}( \frow{1}, \cdot) - g^{\dagger}(\frow{1}, \cdot) \big\|^2_{L^2[0,1]} 
		&=  	\big\|	 g ( \frow{1}, \cdot) - g^{\dagger}(\frow{1}, \cdot) \big\|^2_{L^2[0,1]}
		= 	\big\| h \big\|^2_{L^2[0,1]}	\geq  \frac{c^2 \delta^2}{\nu}.
	\end{align*}
	Inserting this back to Lemma \ref{lem:MSE_L2}, we can conclude the following MSE lower bound even if $\varphi$ is an algorithm which can perfectly estimate $g$ from a finite number of samples. 
	Recall that $\nu$ denotes the number of observations used to estimate $\gphi$ and it is a random variable distributed as per $Binomial(n-1, p)$.
	\begin{align*}
		\MSE\left( \varphi \right)	
			&\geq	(1-p) \bbE_{\frow{1}, \fcol{-1}, \nu} \left[ \left\|	 \gphi_{\nu}( \frow{1}, \cdot) - g^{\dagger}(\frow{1}, \cdot) \right\|^2_{L^2[0,1]}	\right]\\
			&\geq	(1-p) \bbE_{\fcol{-1}, \nu} \left[ \min_{\frow{1} \in [0,1]} \left\|	 \gphi_{\nu}( \frow{1}, \cdot) - g^{\dagger}(\frow{1}, \cdot) \right\|^2_{L^2[0,1]}	\right]\\
			&\geq	(1-p) \bbE_{\fcol{-1}, \nu} \left[ \frac{c^2 \delta^2}{\nu} \right]\\
			&\geq	(1-p) \bbE_{\nu} \left[ \frac{c^2 \delta^2}{\nu} \right]\\
			&\geq	(1-p) \frac{c^2 \delta^2}{ \bbE_{\nu} \left[ \nu \right]}		\qquad \because\text{Jensen's inequality}\\
			&= 		(1-p)	 \frac{c^2 \delta^2}{ (n-1)p}.
	\end{align*}
	The lower bound essentially quantifies the uncertainty between two functions $g$ and $g^{\dagger}$ which could have generated the same data to feed algorithm $\varphi$.
	We have shown a lower bound for an oracle algorithm, which has access to the latent features $\frow{1}$ and $\{\fcol{j} \}_{j \in [n]: M(1,j) = 1}$ and can perfectly restore a certain latent function.
	Since no algorithm can outperform an oracle, this lower bound holds for any algorithm, i.e., for any algorithm $\varphi$, there exists a hard instance to estimate. 
\end{proof}



\subsection{Proof of Theorem \ref{thm:noisy_LB}}\label{sec:noisy_LB_proof}
\begin{proof}
	We let $\hat{F}$ and $F$ denote the pseudo-inverse of $ \hat{g}\big( \frow{1}, \cdot \big)$ and $g\big( \frow{1}, \cdot \big)$, respectively.
	Since we assumed the latent function $g\big( \frow{1}, \cdot \big)$ is $(\lipmin, \lipmax)$ bi-Lipschitz for any $\frow{1} \in [0,1]$, its inverse function
	$F = g^{-1} \big( \frow{1}, \cdot \big)$ is continuous, monotone increasing over $[0,1]$ and $\big( \frac{1}{\lipmax}, \frac{1}{\lipmin} \big)$ bi-Lipschitz.
	Therefore, we can treat $F$ as an absolutely continuous distribution function and its derivative $f$ belongs to Fan's class $\cC_{m, \alpha, B}$ with 
	$m = 0, \alpha = 0$, and $B = \frac{1}{\lipmin}$.
	
	Suppose that given any data $\{ \frow{1} \}$, $\{ \frow{j} \}_{j \in [n]}$, $\{ g( \frow{1}, \fcol{j}): j \in [n] \text{ and } M(1,j) = 1 \}$, algorithm $\varphi$ returns an estimate of the latent function 
	$\gphi_{\nu}(\frow{1}, \cdot)$.
	Here, $\nu := \sum_{j = 2}^n M(1,j)$ in the subscript denotes the number of samples used for estimation of $\gphi_{\nu}$.
	
	Let $\Fphi_\nu := (\gphi_{\nu})^{-1}(\frow{1},  \cdot)$. We may assume $\gphi_{\nu}$ is nondecreasing, because $g$ is monotone increasing from the model assumption.
	In fact, $g\big( \frow{1}, \cdot \big)$ is assumed to be not only monotone increasing, but $(\lipmin, \lipmax)$ bi-Lipschitz. Therefore, $F$ is $\big(\frac{1}{\lipmax}, \frac{1}{\lipmin}\big)$ bi-Lipschitz.
	
	Let $z^* := \arg \max_{z \in \Reals} \bbE \left[ ( \Fphi_\nu (z) - F (z) )^2 \right]$. 
	Then let $y^* = F(z^*)$ and $\hat{y}^*_\nu := \Fphi_\nu (z^*)$ denote the image of $z^*$ under $F$ and $\Fphi_\nu$, respectively.
	Note that $\Fphi_\nu$ is a random function, and hence, $\hat{y}^*_\nu$ is a random variable.
	Subsequently, we define $\hat{z}^*_\nu := F^{-1}(\hat{y}^*_\nu)$.
	
	Without loss of generality, we may assume $y^* \leq \hat{y}^*_\nu$ and it follows that $\hat{z}^*_\nu \geq z^*$. Then for $y \in [y^*, \hat{y}^*_\nu]$, 
	\begin{align*}
		g\big( \frow{1}, y \big) - \gphi_\nu \big( \frow{1}, y \big) &\geq g\big( \frow{1}, y \big) - \gphi_\nu\big( \frow{1}, \hat{y}^*_\nu \big)\\
			& = g\big( \frow{1}, y \big) - g\big( \frow{1}, y^* \big)\\
			& \geq l (y - y^*).		
	\end{align*}
	From the definition of $L^2$ distance, it follows that
	\begin{align}
		\left\| \gphi_\nu \big( \frow{1}, \cdot \big) - g\big( \frow{1}, \cdot \big) \right\|_{L^2[0,1]}^2
			&= \int_0^1 \left| \gphi_\nu \big( \frow{1}, y \big) - g\big( \frow{1}, y \big) \right|^2 dy	\nonumber\\
			&\geq	\int_{y^*}^{\hat{y}^*_\nu} \left| \gphi_\nu \big( \frow{1}, y \big) - g\big( \frow{1}, y \big) \right|^2 dy	\nonumber\\
			&\geq	\int_{y^*}^{\hat{y}^*_\nu} l^2 \left| y - y^* \right|^2 dy	\nonumber\\
			&= \frac{l^2}{3} \left| \hat{y}^*_\nu - y^* \right|^3	\nonumber\\
			&= \frac{l^2}{3} \left| \Fphi_{\nu}(z^*) - F(z^*) \right|^3.	\label{eqn:L2_LB}
	\end{align}
	
	Recall from Lemma \ref{lem:MSE_L2} that for any algorithm $\varphi: Z \mapsto \Aphi$,
	\begin{align*}	
		\MSE\left( \varphi \right)	
			&\geq	(1-p) \bbE_{\frow{1}, \fcol{-1}, \nu} \left[  \left\|	 \gphi_{\nu}( \frow{1}, \cdot) - g(\frow{1}, \cdot) \right\|^2_{L^2[0,1]}	\right],
	\end{align*}
	where $\nu \sim Binomial(n-1, p)$ and $\fcol{-1}$ denotes $\{ \fcol{j}: j \in [n], j \neq 1\}$. 
	If we restrict our latent function to take the form $g\left( \frow{i}, \fcol{j} \right) = g_2 ( \fcol{j})$ for some $g_2: [0,1] \to \Reals$, then we can remove the expectation with respect to $\frow{1}$.
	From Eq. \eqref{eqn:L2_LB}, it follows that
	\begin{align*}
		\MSE\left( \varphi \right)
			&=		(1-p) \bbE_{\fcol{-1}, \nu} \left[ 	\frac{\lipmin^2}{3}	\left| \Fphi_{\nu}(z^*) - F(z^*) \right|^3		\right]\\
			&\geq	\frac{(1-p) \lipmin^2}{3}	\bbE_{\nu} \left[  \bbE_{\fcol{-1}}  \left[	\left| \Fphi_{\nu}(z^*) - F(z^*) \right|^2	\right]^{3/2}\right]	
				\qquad\because \text{Jensen's inequality}
	\end{align*}
	
	By Lemma \ref{lem:deconv_hard} -- more precisely, by \eqref{eqn:hardness_deconvolution} -- for any $\nu$, there exists a latent function $g_2$ 
	(and corresponding $f \in \cC_{0,0,\frac{1}{\lipmin}}$ such that for any oracle algorithm $\varphi$,
	\[\bbE_{\fcol{-1}}  \left[	\left| \Fphi_{\nu}(z^*) - F(z^*) \right|^2	\right] \geq \frac{c}{2} \left( \log \nu \right)^{-2 / \beta}.\]
	
	All in all, there exists a hard instance of latent function $g$ such that
	\begin{align*}
		\MSE\left( \varphi \right)
			&\geq	\frac{(1-p) \lipmin^2}{3}	\bbE_{\nu} \left[ \left( \frac{c}{2} \left( \log \nu \right)^{-2 / \beta} \right)^{3/2} \right]\\
			&=		\frac{(1-p) \lipmin^2 c^{3/2}}{6 \sqrt{2}}	\bbE_{\nu} \left[		\left( \log \nu \right)^{-3 / \beta}	\right]\\
			&\geq	\frac{(1-p) \lipmin^2 c^{3/2}}{6 \sqrt{2}}	\big( \log  \bbE_{\nu} \left[ \nu \right] \big)^{-3 / \beta}		\qquad\because \text{Jensen's inequality}\\
			&=	\frac{(1-p) \lipmin^2 c^{3/2}}{6 \sqrt{2}}	\big( \log  (n-1)p \big)^{-3 / \beta}.
	\end{align*}
We can apply Jensen's inequality because $\left( \log x \right)^{-3/\beta}$ is convex when $x > 1$, for any $\beta > 0$.
\end{proof}

==> contents/CC_proof_quantile_noiseless.tex <==
\section{Proof of Lemma \lowercase{\ref{lem:quantile_noiseless}}: Reliable Column Feature Estimation When There Is No Noise }\label{sec:proof_noiseless_quantile}
\begin{proof}[Proof of Lemma \ref{lem:quantile_noiseless}]
Recall from Eq. \eqref{eqn:quantile_rowwise} that when conditioned on $\frow{i}$, the quantile of $j$ estimated 
from row $i$ is a function of $|\cB_i| = \sum_{j' = 1}^n M(i,j')$ many independent random variables, 
$H\big( Z(i, j) - Z(i, j') \big)$:
\[\hat{q}_i(j) = \frac{\sum_{j'=1}^n M(i,j') H\big( Z(i, j) - Z(i, j') \big) }{\sum_{j' = 1}^n M(i,j')}.\]
Since $H\big( Z(i, j_1) - Z(i, j_2) \big)$ takes value in $\{ 0, \frac{1}{2}, 1\}$, it satisfies the bounded difference condition. To be more specific, let's consider a perturbation on the column feature associated with one index. For any $j_0 \in [n]$, if $j_0 \in \cB_i$ (i.e., if $M(i, j_0) = 1$), then
\[
	\left|  \left.\hat{q}_i(j)\right|_{\fcol{j_0}=a} - \left.\hat{q}_i(j)\right|_{\fcol{j_0}=b} \right|	\leq \frac{1}{\left| \cB_i \right|},
\]
for any value $a, b \in [0,1]$, while if $j_0 \not\in \cB_i$ (i.e., if $M(i, j_0) = 0$), then obviously
\[
	\left| \left.\hat{q}_i(j)\right|_{\fcol{j_0} = a} - \left.\hat{q}_i(j)\right|_{\fcol{j_0} = b} \right| = 0. 
\]
		
 Since  $\Exp {\hat{q}_i(j)} = \fcol{j}$, we can achieve the following probabilistic tail bound by an application of McDiarmid's inequality 
\[	
	\Prob{ \left| \hat{q}_i(j) -  \fcol{j} \right| \geq t  } \leq 2 \exp\big( -2 |\cB_i| t^2 \big).
\]
\end{proof}
	
	

==> contents/DD_proof_quantile_noisy.tex <==
\section{Proof of Lemma \lowercase{\ref{lem:quantile_noisy}}: Reliable Column Feature Estimation Even When There Is Noise }\label{sec:proof_noisy_quantile}

%\begin{lemma}\label{lem:quantile_noisy}
%	For any $t \geq \frac{4 \constee}{\sqrt{mp}}$,
%	\begin{align*}
%		\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t } 
%			&\leq \exp\left( - \frac{nt^2}{2}  \right) \\
%			&\quad+ \exp\bigg( -\frac{n}{6}\Big( t - \frac{2 \constee}{\sqrt{mp}} \Big) \bigg)\\
%			&\quad + \exp\left( - \frac{mp}{8} \right).	
%	\end{align*}
%\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:quantile_noisy}]
Recall the definition of $\hat{q}_{\marg}(j)$ from \eqref{eqn:Z_marg} and \eqref{eqn:estimate_marg}: for $j \in [n]$, we defined
\[
	\hat{q}_{\marg}(j) = \frac{1}{n}\sum_{j' = 1}^n H \left( Z_{\marg}(j) - Z_{\marg}(j') \right),
\]
where
\[
	Z_{\marg}(j) = \begin{cases}
		\frac{ \sum_{i=1}^m M(i,j) Z(i,j)}{\sum_{i=1}^m M(i,j)},	& \text{if } \cB^j \neq \emptyset\\
		\frac{1}{2},									&	\text{if } \cB^j = \emptyset.
	\end{cases}
\]
We also note that the marginalized latent function $g_{\marg}(y) := \int_0^1 g(x,y) dx$ is $(\lipmin, \lipmax)$-biLipschitz, and hence, invertible. 
For $j \in [n]$, let $\zeta^{(j)} = g_{\marg}^{-1}\left( Z_{\marg}(j)\right)$ for the purpose of analysis. We also define an imaginary estimator
\[
	\hat{q}_{*}(j) = \frac{1}{n}\sum_{j' = 1}^n H \left( \fcol{j} - \fcol{j'} \right).
\]
Note that $\zeta^{(j)}$ and $\hat{q}_{*}(j) $ are used solely for analysis.
		
By triangle inequality, the error in quantile estimation is upper bounded as
\[	\left| \hat{q}_{\marg}(j) - \fcol{j} \right| \leq \Big| \hat{q}_{\marg}(j) - \hat{q}_*(j) \Big| + \left| \hat{q}_*(j) - \fcol{j}\right|.	\]
If both $\Big| \hat{q}_{\marg}(j) - \hat{q}_*(j) \Big| \leq t_1$ and $\left| \hat{q}_*(j) - \fcol{j}\right| \leq t_2$ are satisfied, then $\left| \hat{q}_{\marg}(j) - \fcol{j} \right| \leq t_1 + t_2$. Therefore, for any $t_1, t_2 > 0$ and $t = t_1 + t_2$,
\begin{align}
	\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t }	
		&\leq \mathbb{P}\Big({\Big| \hat{q}_{\marg}(j) - \hat{q}_*(j) \Big| > t_1 }\Big) + \Prob{ \left| \hat{q}_*(j) - \fcol{j}\right| > t_2 }.	\label{eqn:partition1}	
\end{align}
Note that $\hat{q}_{*}(j)$ exponentially concentrates to $\fcol{j}$ as $n \to \infty$ by McDiarmid's inequality. Therefore, it suffices to find 
a probabilistic tail upper bound for $\left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right|$:		
\begin{align*}
	\left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right| &= \left| \frac{1}{n} \sum_{j' = 1}^n  \left[ H \left( Z_{\marg}(j) - Z_{\marg}(j') \right) - H \left( \fcol{j} - \fcol{j'} \right) \right] \right|\\
		&\leq \frac{1}{n} \sum_{j' = 1}^n \Bigg| \left[ H \left( Z_{\marg}(j) - Z_{\marg}(j') \right) - H \left( \fcol{j} - \fcol{j'} \right) \right] \Bigg|.
\end{align*}
For $j' \neq j$, 
\begin{equation}\label{eqn:prob_failure}
	\left| \left[ H \left( Z_{\marg}(j) - Z_{\marg}(j') \right) - H \left( \fcol{j} - \fcol{j'} \right) \right] \right| = 1 \quad\text{with probability }\pf,
\end{equation} 
and $0$ otherwise (it is uniformly $0$ for $j' = j$). Now, if we can find an upper bound $\pfs \geq \pf$, then for $t > \pfs$,
\begin{align*}
	\mathbb{P}\Big( \left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right| > t \Big) 
		& \leq \mathbb{P} \Big( Y > nt \Big)\\
		& \leq \exp\left( -\frac{n( t - \pfs)^2}{t + \pfs} \right),
\end{align*}
where $Y \sim Binomial(n, \pfs)$.

We let
\begin{equation}
	\constaa = \frac{\lipmin^2}{2 (\fmax - \fmin)^2}		\qquad\text{and}\qquad
	\constbb = \frac{\lipmin^2}{8\sigma^2}.		
\end{equation}
With these constants $\constaa, \constbb$, we define a monotone decreasing function $\Qf: \Ints_+ \to \Reals_+$ as 
\begin{equation}\label{eqn:Q_function}
	\Qf(x) = 2\sqrt{\pi} \left( \frac{1}{\sqrt{\constaa x}} + \frac{1}{\sqrt{\constbb x}} + \frac{e^{\constaa/2}}{\sqrt{mp \constaa }} 
		+  \frac{e^{\constbb/2}}{\sqrt{mp \constbb }} \right).
\end{equation}

Using the function $\Qf$ defined above, we make the following two claims:
\begin{itemize}
	\item Claim 1:
	For $j \in [n]$, the probability of failure (cf. see \eqref{eqn:prob_failure}) is bounded as $\pf \leq \Qf\Big( \big|\cB^j \big|\Big)$.
	\item Claim 2:
	For $t' \geq 2\Qf \left( \frac{mp}{2}\right)$,
	\[	
		\Prob{ \left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right| > t' } \leq \left.\exp\left( -\frac{n( t' - \pfs)}{3} \right) \right|_{\pfs = \Qf(\frac{mp}{2})} + \exp\left( - \frac{mp}{8} \right). 	\]
\end{itemize}
Combining Claims 1 and 2 with \eqref{eqn:partition1} (with the choice of $t_1 = t_2 = \frac{t}{2}$), we conclude that for any 
$t > 4\Qf(\frac{mp}{2}) = \frac{4\constee}{\sqrt{mp}}$,
\begin{align*}
	\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t }
		&\leq \Prob{\big| \hat{q}_{\marg}(j) - \hat{q}_*(j) \big| > \frac{t}{2} } + \Prob{ \big| \hat{q}_*(j) - \fcol{j}\big| > \frac{t}{2} }\\
		&\leq \exp\left( -\frac{n( \frac{t}{2} - \Qf(\frac{mp}{2}))}{3} \right)  + \exp\left( - \frac{nt^2}{2}  \right)
			+ \exp\left( - \frac{mp}{8} \right) .
\end{align*}
Realizing $\Qf(\frac{mp}{2}) = \frac{2\sqrt{\pi}}{\sqrt{mp}} \left( \frac{\sqrt{2} + e^{\constaa/2}}{\sqrt{\constaa}} + \frac{\sqrt{2} + e^{\constbb/2}}{\sqrt{\constbb}} \right)$ completes the proof.

In the rest of the proof, we prove the two claims.

\medskip
{\bf Proof of Claim 1.}
The estimator $\hat{q}_{\marg}(j)$ exploits the pairwise ordering information of column pair $(j,j')$ by taking the sign of $Z_{\marg}(j) - Z_{\marg}(j')$, which might be different from the true ordering $\sign\big( \fcol{j} - \fcol{j'} \big)$ due to the presence of noise. We analyze the probability of the order to be distrubed. Note that $\sign \Big( Z_{\marg}(j) - Z_{\marg}(j') \Big) = \sign \big( \zeta^{(j)} - \zeta^{(j')}\big)$ because $g_{\marg}$ is strictly monotone increasing.
		
Let $X_j := \zeta^{(j)} - \fcol{j}$. Then since $g_{\marg}$ is $(l,L)$-biLipschitz, for any $s > 0$,
\begin{align*}
	\Prob{X_j \geq s}	&\leq \Prob{ Z_{\marg}(j) - g_{\marg}\big(\fcol{j}\big) \geq ls}\\
		&= \Prob{	\frac{1}{|\cB^j|} \sum_{i' \in \cB^j} Z(i',j) - g_{\marg}\big(\fcol{j}\big) \geq ls }\\
		&\leq \Prob{	\frac{1}{|\cB^j|} \sum_{i' \in \cB^j} A(i',j) - g_{\marg}\big(\fcol{j}\big) \geq \frac{ls}{2} }
			+ \Prob{	\frac{1}{|\cB^j|} \sum_{i' \in \cB^j} N(i',j) \geq \frac{ls}{2} }\\
		&\leq \exp\left( - \frac{\big| \cB^j \big| l^2 s^2}{2( \fmax - \fmin )^2} \right) + \exp \left( -\frac{\big| \cB^j \big| l^2 s^2}{ 8 \sigma^2} \right).
\end{align*}
Also, we can achieve the same upper bound for $\Prob{X_j \leq -s}$. 

Since $X_j - X_{j'} = \big( \zeta^{(j)} - \zeta^{(j')}\big) - \big( \fcol{j} - \fcol{j'} \big)$, the pairwise order is conserved unless
\begin{align*}
	\begin{cases}
		X_j - X_{j'}	< - \big( \fcol{j} - \fcol{j'}\big),	& \text{when } \fcol{j} - \fcol{j'} \geq 0,\\
		X_j - X_{j'} > \fcol{j'} - \fcol{j},			& \text{when } \fcol{j} - \fcol{j'} < 0. 
	\end{cases}
\end{align*}
Given $\fcol{j}$, the probability of $\fcol{j'}$ be smaller than $\fcol{j}$ is equal to $\fcol{j}$, i.e., $\Prob{\fcol{j} - \fcol{j'} \geq 0} = \fcol{j}$. Therefore, the probability of the problematic event can be partitioned as
\begin{align}
	\Prob{ \sign\left( \zeta^{(j)} - \zeta^{(j')} \right) \neq \sign\left( \fcol{j} - \fcol{j'} \right) } 
		&= \Prob{\left. X_j - X_{j'} < - \left( \fcol{j} - \fcol{j'}\right) \right| \fcol{j} - \fcol{j'} \geq 0} \Prob{\fcol{j} - \fcol{j'} \geq 0 }	\label{eqn:proof_noisy_term.1}\\
		&\quad+\Prob{\left. X_j - X_{j'} > \fcol{j'} - \fcol{j} \right| \fcol{j} - \fcol{j'} < 0} \Prob{\fcol{j} - \fcol{j'} < 0 }.			\label{eqn:proof_noisy_term.2}
\end{align}
The conditional probability in \eqref{eqn:proof_noisy_term.1} can be upper bounded by
\begin{align*}
	\Prob{\left. X_j - X_{j'} < - \left( \fcol{j} - \fcol{j'}\right) \right| \fcol{j} - \fcol{j'} \geq 0}
	 	&\leq \Prob{\left. X_j  < - \frac{ \fcol{j} - \fcol{j'}}{2} \right| \fcol{j} - \fcol{j'} \geq 0}\\
	 	&\quad 	+  \Prob{\left. X_{j'} > \frac{ \fcol{j} - \fcol{j'}}{2} \right| \fcol{j} - \fcol{j'} \geq 0}.
\end{align*}
		
Meanwhile, if we define a new random variable $T := \frac{ \fcol{j} - \fcol{j'}}{2} $ and let $\tau$ denote an instance of $T$, then we can see that 
$f_T(\tau) = \frac{2}{\fcol{j}} \Ind{0 \leq T \leq \frac{\fcol{j}}{2}}$, conditioned on $\fcol{j} - \fcol{j'} \geq 0$.
\begin{align*}
	\Prob{ X_j  < - \tau \left| \fcol{j} - \fcol{j'} \geq 0 \right.}
		&= \sum_{k=0}^m \Prob{|\cB^j| = k} \Prob{ X_j  < - \tau \left| \fcol{j} - \fcol{j'} \geq 0, |\cB^j| = k \right.}\\
		&\leq \sum_{k=0}^m {m \choose k} p^k (1-p)^{m-k} \Big[ \exp \big( - \constaa k \tau^2 \big) + \exp \big( -\constbb k \tau^2 \big) \Big]\\
		&= \left[ p e^{-\constaa \tau^2} + (1-p) \right]^m +  \left[ p e^{-\constbb \tau^2} + (1-p) \right]^m\\
		&= \bigg[ 1 - \frac{mp \big( 1 - e^{-\constaa \tau^2}\big)}{m} \bigg]^m + \bigg[ 1 - \frac{mp \big( 1 - e^{-\constbb \tau^2}\big)}{m} \bigg]^m\\
		&\leq \exp\bigg[ -mp \big( 1 - e^{-\constaa \tau^2}\big) \bigg] + \exp \bigg[ - mp \big( 1 - e^{-\constbb \tau^2}\big) \bigg].
\end{align*}
		
As a result,
\begin{align}
	&\Prob{ \left. \sign\big( \zeta^{(j)} - \zeta^{(j')} \big) \neq \sign\big( \fcol{j} - \fcol{j'} \big) \right| |\cB^j| =k }	\nonumber\\
		&\qquad= \Prob{\fcol{j} - \fcol{j'} \geq 0 }
			\Prob{\left. X_j - X_{j'} < - \left( \fcol{j} - \fcol{j'}\right) \right| \fcol{j} - \fcol{j'} \geq 0, |\cB^j| =k} 	\label{eqn:proof_noisy_term.3}\\
		&\qquad\quad+  \Prob{\fcol{j} - \fcol{j'} < 0 }
			\Prob{\left. X_j - X_{j'} > \fcol{j'} - \fcol{j} \right| \fcol{j} - \fcol{j'} < 0, |\cB^j| =k}.	\label{eqn:proof_noisy_term.4}
\end{align}	
Note that $X_j < -\tau$ and $X_{j'} > \tau$ implies $X_j - X_{j'} < - 2\tau$ for any $\tau \in \Reals$. Therefore, it follows that 
$\Prob{ X_j - X_{j'} < - 2\tau} \leq \Prob{X_j < -\tau } + \Prob{X_{j'} > \tau}$ for any $\tau \in \Reals$. 

Now we will obtain an upper bound on Eq. \eqref{eqn:proof_noisy_term.3} by finding upper bounds on each terms and then taking the union bound.
First, we observe that $\frac{d\Prob{ \fcol{j} - \fcol{j'} = 2\tau \left| \fcol{j} - \fcol{j'} \geq 0 \right.}}{d \tau}= \frac{2}{\fcol{j}} \bI \big\{0 \leq \tau \leq \frac{\fcol{j}}{2}  \big\}$ 
and $\Prob{\fcol{j} - \fcol{j'} \geq 0 }=\fcol{j}$.
\begin{align}
	&\Prob{\left. X_j < - \frac{ \fcol{j} - \fcol{j'}}{2} \right| \fcol{j} - \fcol{j'} \geq 0, |\cB^j| =k} \Prob{\fcol{j} - \fcol{j'} \geq 0 }	\nonumber\\
	&\qquad= \int_{\tau} \Prob{ X_j  <  -\tau \left| \fcol{j} - \fcol{j'} = 2\tau, |\cB^j| =k\right.} 
			\frac{d\Prob{ \fcol{j} - \fcol{j'} = 2\tau \left| \fcol{j} - \fcol{j'} \geq 0 \right.}}{d \tau}	 \Prob{\fcol{j} - \fcol{j'} \geq 0 } d \tau	\nonumber\\
	&\qquad = 2\int_0^{\frac{\fcol{j}}{2}}  \Prob{ X_j  < - \tau \left| \fcol{j} - \fcol{j'} = 2\tau, |\cB^j| =k\right.} d\tau		\nonumber\\
	&\qquad \leq 2\int_0^{\frac{\fcol{j}}{2}} \exp\left( -\constaa k \tau^2 \right) + \exp \left( - \constbb k \tau^2 \right) d\tau	\nonumber\\
	&\qquad \leq 2\int_0^{\infty} \exp\left( -\constaa k \tau^2 \right) + \exp \left( - \constbb k \tau^2 \right) d\tau			\nonumber\\
	&\qquad = \sqrt{\pi} \left( \frac{1}{\sqrt{\constaa k}} + \frac{1}{\sqrt{\constbb k}} \right).		\label{eqn:proof_noisy_term.5}
\end{align}
		
Similarly, we can obtain an upper bound for $X_{j'}$. Note that column $j$ and $j'$ are independent (because $\fcol{j}$ 
and $\fcol{j'}$ are independently drawn) and that given $c > 0$, we have $1 - e^{-cu^2} \geq c e^{-c} u^2$, for all $u \in [0,1]$.
\begin{align}
	&\Prob{\left. X_{j'} > \frac{ \fcol{j} - \fcol{j'}}{2} \right| \fcol{j} - \fcol{j'} \geq 0, |\cB^j| =k} \Prob{\fcol{j} - \fcol{j'} \geq 0 }		\nonumber\\
	&\qquad= \int_{\tau} \Prob{ X_{j'}  > \tau \left| \fcol{j} - \fcol{j'} = 2\tau, |\cB^j| =k\right.}
			\frac{d\Prob{ \fcol{j} - \fcol{j'} = 2\tau \left| \fcol{j} - \fcol{j'} \geq 0 \right.}}{d \tau}	\Prob{\fcol{j} - \fcol{j'} \geq 0 } d \tau	\nonumber\\
	&\qquad = 2\int_0^{\frac{\fcol{j}}{2}}  \Prob{ X_{j'}  > \tau \left| \fcol{j} - \fcol{j'} = 2\tau, |\cB^j| =k\right.} d\tau		\nonumber\\
	&\qquad = 2\int_0^{\frac{\fcol{j}}{2}}  \Prob{ X_{j'}  > \tau \left| \fcol{j} - \fcol{j'} = 2\tau\right.} d\tau				\nonumber\\
	&\qquad \leq 2\int_0^{\frac{\fcol{j}}{2}} \exp\left[ -mp \left( 1 - e^{-\constaa \tau^2}\right) \right] + \exp \left[ - mp \left( 1 - e^{-\constbb \tau^2}\right) \right] d\tau	\nonumber\\
	&\qquad \leq 2\int_0^{\frac{\fcol{j}}{2}} \exp\left( -mp \constaa e^{-\constaa} \tau^2\right) + \exp \left( - mp \constbb e^{-\constbb} \tau^2 \right) d\tau	\nonumber\\
	&\qquad \leq 2\int_0^{\infty} \exp\left( -mp \constaa e^{-\constaa} \tau^2\right) + \exp \left( - mp \constbb e^{-\constbb} \tau^2 \right) d\tau			\nonumber\\
	&\qquad = \sqrt{\pi} \left( \frac{1}{\sqrt{mp \constaa e^{-\constaa}}} + \frac{1}{\sqrt{mp \constbb e^{-\constbb}}}   \right).		\label{eqn:proof_noisy_term.6}
\end{align}
In the last line, we used the fact that $\int_0^{\infty} e^{-ax^2} dx = \frac{1}{2}\sqrt{\frac{\pi}{a}}$; see \eqref{eqn:half_normal} .

Using \eqref{eqn:proof_noisy_term.5} and \eqref{eqn:proof_noisy_term.6}, we can find an upper bound on the term in \eqref{eqn:proof_noisy_term.3} as
\begin{align*}
	&\Prob{\fcol{j} - \fcol{j'} \geq 0 }\Prob{\left. X_j - X_{j'} < - \left( \fcol{j} - \fcol{j'}\right) \right| \fcol{j} - \fcol{j'} \geq 0, |\cB^j| =k}\\
	&\qquad\leq \sqrt{\pi} \left( \frac{1}{\sqrt{\constaa k}} + \frac{1}{\sqrt{\constbb k}} + \frac{1}{\sqrt{mp \constaa e^{-\constaa}}} + \frac{1}{\sqrt{mp \constbb e^{-\constbb}}}  \right).	
\end{align*}
		
We can obtain the same upper bound on the term in \eqref{eqn:proof_noisy_term.4}. It suffices to remark that
\begin{align*}
	\frac{d\Prob{ \fcol{j} - \fcol{j'} = -2\tau \left| \fcol{j} - \fcol{j'} < 0 \right.}}{d \tau} &= \frac{2}{1 - \fcol{j}} \Ind{0 \leq \tau \leq \frac{1 - \fcol{j}}{2} },\\
	\Prob{\fcol{j} - \fcol{j'} < 0 } &= 1-\fcol{j}.
\end{align*}
Then by the same logic,
\begin{align*}
	&\Prob{\fcol{j} - \fcol{j'} < 0 } \Prob{\left. X_j - X_{j'} > \fcol{j'} - \fcol{j} \right| \fcol{j} - \fcol{j'} < 0, |\cB^j| =k} \\
	&\qquad\leq \sqrt{\pi} \left( \frac{1}{\sqrt{\constaa k}} + \frac{1}{\sqrt{\constbb k}} + \frac{1}{\sqrt{mp \constaa e^{-\constaa}}} + \frac{1}{\sqrt{mp \constbb e^{-\constbb}}}  \right).
\end{align*}
		
Consequently, we can conclude our claim 1:
\begin{align*}
	q &= \Prob{ \sign\left( \zeta^{(j)} - \zeta^{(j')} \right) \neq \sign\left( \fcol{j} - \fcol{j'} \right)}\\
		&\leq 2\sqrt{\pi} \bigg( \frac{1}{\sqrt{\constaa \big| \cB^j \big|}} + \frac{1}{\sqrt{\constbb \big| \cB^j \big|}} + \frac{e^{\constaa/2}}{\sqrt{mp \constaa }} +  \frac{e^{\constbb/2}}{\sqrt{mp \constbb }} \bigg)\\
		&= \Qf \big( \big|\cB^j \big|\big).
\end{align*}
		
\medskip
{\bf Proof of Claim 2.}
We prove Claim 2 by the usual trick using the law of total probability. First, we recall the definition of conditioning event $\Ecol$ from \eqref{eqn:sufficient_overlap.col}:
\[	\Ecol \equiv \left\{|\cB^j| \geq \frac{mp}{2} \right\}.	\]
Then we observe that for $t' > \Qf(\frac{mp}{2})$,
\begin{align*}
	\Prob{ \left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right| > t' } 
	 	&\leq \Prob{ Y > nt' }\\
		&= \Prob{ Y > nt' \left| \Ecol \right.} \Prob{ \Ecol } + \Prob{ Y > nt' \left| \Ecol^c \right.} \Prob{ \Ecol^c }\\
		&\leq  \Prob{ Y > nt' \left| \Ecol \right.} +  \Prob{ \Ecol^c }\\
		&\leq \left. \exp\left( -\frac{n( t' - \pfs)^2}{t' + \pfs} \right) \right|_{\pfs = \Qf(\frac{mp}{2})} + \exp\left( - \frac{mp}{8} \right).
\end{align*}
In achieving the last inequality, we respectively use the fact that $\Qf$ is monotone decreasing and the Binomial Chernoff bound to bound the terms.
		
Moreover, we can see that $\frac{t' - \pfs}{t' + \pfs} \geq \frac{1}{3}$ for $t' \geq 2\pfs$. Therefore, for $t' > 2 \Qf(\frac{mp}{2})$,
\[	\Prob{ \left| \hat{q}_{\marg}(j) - \hat{q}_*(j) \right| > t' } \leq \exp\left( -\frac{n( t' - \Qf(\frac{mp}{2}))}{3} \right) + \exp\left( - \frac{mp}{8} \right). 	\]
\end{proof}
	

%%% The item below is not used any more
\iffalse{	
	\subsection{A Stronger Variant of Lemma \ref{lem:noisy_quantile_prelim}}
		For later use in the proof of Lemma \ref{lem:T_good}, we state an even stronger variant of the lemma \ref{lem:noisy_quantile_prelim} as a corollary.
	\begin{corollary}\label{coro:noisy_quantile_uniform}
		The marginal quantile estimator $\hat{q}_{\marg}(j)$ concentrates to $\theta_{col}^{(j)}$ uniformly for all $j \in [n]$ with high probability. Specifically, for any $s \geq (mp)^{-1/3}$ and $t \geq 16 s + 32 \exp\left( -c (mp)^{1/3} \right)$, 
		\begin{align*}
			&\Prob{ \exists j \in [n]:  \left| \hat{q}_{\marg}(j) - \fcol{j} \right| \geq t }\\
				&\quad	\leq	2n\exp\left( -\frac{n t^2}{2} \right) + n\exp\left(-\frac{nt}{12} \right) + n \exp\left( -\frac{mp}{8} \right)\\
				&\qquad	 + n \exp\left( - \frac{ns}{3}  \right) + 4n \exp\left(-c (mp)s^{2}\right),
	\end{align*}
	where $c = \min \left\{\frac{l^2}{16\left( D_{max} - D_{min} \right)^2}, \frac{l^2}{64\sigma^2} \right\}$.
	\end{corollary}
	
	\begin{proof}
		Again we will prove the corollary by applying the union bound:
		\begin{align*}
			&\Prob{ \exists j \in [n]: \left| \hat{q}_{\marg}(j) - \fcol{j} \right| \geq t }\\
			&	\leq \Prob{ \exists j \in [n]:  \left| \hat{q}_{\marg}(j) - \hat{q}_{\theta}(j) \right| \geq \frac{t}{2} }\\
				&\quad + \Prob{ \exists j \in [n]:  \left| \hat{q}_{\theta}(j) - \fcol{j} \right| \geq \frac{t}{2} }\\
			&	\leq \Prob{ \exists j \in [n]:  \left| \hat{q}_{\marg}(j) - \hat{q}_{\theta}(j) \right| \geq \frac{t}{2} }\\
				&\quad +  \Prob{ \left.\exists j \in [n]:   \left| \hat{q}_{\marg}(j) - \hat{q}_{\theta}(j) \right| \geq \frac{t}{2} \right| E} + \Prob{E^c}\\
			&	\leq \sum_{j=1}^n \Prob{ \left| \hat{q}_{\marg}(j) - \hat{q}_{\theta}(j) \right| \geq \frac{t}{2} }\\
				&\quad + \sum_{j=1}^n  \Prob{ \left. \left| \hat{q}_{\marg}(j) - \hat{q}_{\theta}(j) \right| \geq \frac{t}{2} \right| E} + \Prob{E^c}.
		\end{align*}
		The conclusion can be derived by plugging in Eqs. \eqref{eqn:bound1}, \eqref{eqn:conditionE}, and \eqref{eqn:discrepancy} to the last line.
	\end{proof}
}\fi

==> contents/EE_proof_CDF_known.tex <==
\section{Proof of Lemma \lowercase{\ref{lem:cdf_noisy_known}}: CDF Estimation When Noise Distribution is Known}\label{sec:proof_noisy_known_CDF}
In this section, we show that the estimated CDF $\tilde{F}^{(i)}$ is close to the true CDF $F^{(i)}$ by showing both the bias 
$\left| \bbE \big[ \tilde{F}^{(i)} (z)\big]- F^{(i)}(z) \right| $ and the variance of $\tilde{F}^{(i)} (z)$ are small. Lemmas \ref{lem:mean_difference_tilde} 
and \ref{lem:concentration_tilde} assert these claims based on consistency results for deconvolution; see Appendix \ref{appx:deconvolution} for more details. 
Equipped with the technical lemmas, we prove Lemma \ref{lem:cdf_noisy_known} in \ref{sec:proof_cdf_known}.


\subsection{Support Lemma to Control the Bias of $\tilde{F}^{(i)}$}\label{sec:known_bias}
\begin{lemma}[Bias is small]\label{lem:mean_difference_tilde} 
	For $i \in [m]$, let $\tilde{F}^{(i)}$ be defined as in \eqref{eqn:ECDF_known_noise}. Then there exists a universal constant $\constcc = C(\lipmin) > 0$ 
	such that
	\[	\sup_{z \in \Reals}\left| \Exp{\tilde{F}^{(i)} (z)} - F^{(i)}(z) \right| \leq \constcc \left( \log \left| \cB_i \right| \right)^{-1/\beta},\qquad\forall i \in [m].	\]
%	Here, $\beta$ is the smoothness parameter of the supersmooth noise.
\end{lemma}
The expectation in the lemma statement is taken with respect to the randomness in data generation process.
	
\begin{proof}
To begin with, we observe that
\begin{align}
	\bigg| \Exp{\tilde{F}^{(i)} (z)} - F^{(i)}(z) \bigg|	
		&=  \bigg| \Exp{\tilde{F}^{(i)} (z) - F^{(i)}(z)} \bigg|
		\Exp{\left( \tilde{F}^{(i)} (z) - F^{(i)}(z) \right)^2}^{1/2},	\label{eqn:mean_tilde}
\end{align}
because $\Exp{X^2}- \Exp{X}^2 \geq 0$. We control the term in the right hand side of \eqref{eqn:mean_tilde} by applying Theorem \ref{thm:Fan2}. 
For that purpose, we need to ensure that our density $f^{(i)}(z) = \frac{d}{dz}F^{(i)}(z)$ is in Fan's class for some $m, a$, and $B$; see \eqref{eqn:Fan_class} 
for the definition of Fan's density class. 
	
Note that $F^{(i)}$ is the inverse function of a slice of the latent function with a fixed row feature, $g_{x=\frow{i}}$, in our model. We assume it admits 
a probability density $f^{(i)}$. It is easy to see that $\frac{1}{\lipmax} \leq f^{(i)} (z) \leq \frac{1}{\lipmin}$ for all $z \in supp~f^{(i)}$ (and $f^{(i)}(z) = 0$ 
outside the support) because the inverse of $F^{(i)}$ is assumed $(\lipmin, \lipmax)$ bi-Lipschitz in our model. This $f^{(i)}$ belongs to Fan's class
\[	\cC_{m, \alpha, B} = \left\{ f(x): \left| f^{(m)}(x) - f^{(m)}\left( x + \delta \right)\right| \leq B \delta^{\alpha} \right\},		 \]
with the choice of $m = 0, \alpha = 0$, and $B = \frac{1}{\lipmin}$.

Therefore, for all $i \in [m]$, the density corresponding to $F^{(i)}$ belongs to a Fan's class, i.e., $f^{(i)} \in \cC_{0,0, \frac{1}{\lipmin}}$. As a result, 
we can apply Theorem \ref{thm:Fan2} on \eqref{eqn:mean_tilde} to conclude that for any $i \in [m]$,
\begin{align*}
	\sup_{z \in \Reals}\bigg| \Exp{\tilde{F}^{(i)} (z)} - F^{(i)}(z) \bigg| &\leq	\sup_{z \in \Reals} \Exp{\left( \tilde{F}^{(i)} (z) - F^{(i)}(z) \right)^2}^{1/2}\\
		&\leq \sup_{f \in \cC_{0,0, \frac{1}{\lipmin}}} \sup_{z \in \Reals} \Exp{\left( \tilde{F}_{\left|\cB_i\right|} (z) - F(z) \right)^2}^{1/2}\\
		&= \cO\left( \left( \log \left| \cB_i \right| \right)^{-1/\beta} \right),
\end{align*}
where $\tilde{F}_{\left|\cB_i\right|}$ denotes an estimate of $F$ with $\left|\cB_i\right|$ number of samples. 

Actually this bound is uniform over all possible realizations of $\frow{i} \in [0,1]$ because Fan's original result holds uniformly over the whole class 
$\cC_{0,0, \frac{1}{\lipmin}}$. We observe that the constant hidden in the big O notation is dependent only on the class $\cC_{0,0, \frac{1}{\lipmin}}$, 
hence, only on the model parameter $\lipmin$. Therefore, we can explicitly introduce a constant $\constcc = C(\lipmin)$, which does not depend 
on $i \in [m]$.
\end{proof}
	
	
\subsection{Support Lemma to Control the Variance of $\tilde{F}^{(i)}$}\label{sec:known_variance}
	
\begin{lemma}[Variance is small]\label{lem:concentration_tilde}
	For $i \in [m]$, let $\tilde{F}^{(i)}$ be defined as in \eqref{eqn:ECDF_known_noise}. Then for any $t > 0$, 
	\begin{align*}
		\mathbb{P} \bigg( \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t ~ \bigg| ~ | \cB_i | = \numi \bigg)	
			&\leq 2\exp\left( \frac{- \numi^{1/2} }{2\constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} } t^2	 \right).
	\end{align*}
\end{lemma}
	
\begin{proof} [Proof of Lemma \ref{lem:concentration_tilde}]
Recall that when conditioned on $\frow{i}$, the kernel smoothed ECDF $\tilde{F}^{(i)}$ evaluated at $z$ is a function of $\left| \cB_i \right|$ 
independent random variables $\{Z(i, j)\}_{j \in \cB_i}$, i.e., when $z$ is fixed, $\tilde{F}^{(i)}(z): \Reals^{\left| \cB_i \right|} \to \Reals$ such that
\begin{align*}
	\tilde{F}^{(i)}(z)\left[ Z(i,j_1), \ldots, Z(i,j_{\left| \cB_i \right|}) \right] 
		& = \int_{\tfmin}^{z \wedge \tfmax} \frac{1}{h \left| \cB_i \right|} \sum_{j\in \cB_i} L \left( \frac{w- Z(i,j)}{h} \right) dw,	
\end{align*}
where $L(z) = \frac{1}{2\pi} \int e^{-itz} \frac{\phi_K(t)}{\phi_N\left(\frac{t}{h}\right)}dt$ and $h$ is the bandwidth parameter for kernel $K$. 

First, we show that $\tilde{F}^{(i)}(z)$ satisfies the bounded difference condition (see Eq. \eqref{eqn:bounded_difference}). 
Let $\zeta^{n} = (\zeta_1, \ldots, \zeta_n)$ and $\zeta^{n}_j = (\zeta_1, \ldots, \zeta_j', \ldots, \zeta_{n})$ be two $n$-tuples of real numbers, 
which differ only at the $j$-th position. Then
\begin{align}
	\Big| \tilde{F}^{(i)}(z)[\zeta^{n}] - \tilde{F}^{(i)}(z)[\zeta^n_j] \Big|
		&= \Bigg| \frac{1}{h n} \int_{\tfmin}^{z \wedge \tfmax}  L \left( \frac{w- \zeta_j}{h} \right) - L \left( \frac{w- \zeta'_j}{h} \right) dw \Bigg|		\nonumber\\
		&= \Bigg| \frac{1}{h n} \int_{\tfmin}^{z \wedge \tfmax}  \frac{1}{2\pi} \int \Big(e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big) 
			\frac{\phi_K(t)}{\phi_N\left(\frac{t}{h}\right)}dt dw \Bigg|		\nonumber\\
		&\leq \frac{1}{2\pi h n} \int_{\tfmin}^{z \wedge \tfmax}  \int \Big|e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big| 
			\left|\frac{\phi_K(t)}{\phi_N\left(\frac{t}{h}\right)} \right| dt dw.	\label{eqn:difference_intermediate}
\end{align}
Because $e^{-\img tz}$ is on the unit circle in the complex plane for any real numbers $t$ and $z$, we have 
\begin{align*}
	\Big|e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big| 
		&\leq \Big|e^{-\img t \frac{w- \zeta_j}{h} }\Big| + \Big| e^{-\img t \frac{w- \zeta'_j}{h} }\Big|  = 2.
\end{align*}
 From the supersmoothness assumption on the noise in \eqref{eqn:model_supersmooth}, 
 we have $\left| \phi_N\left(\frac{t}{h}\right) \right| \geq B^{-1} \exp\left( -\gamma \left|\frac{t}{h}\right|^{\beta}\right)$. 
		
We choose the bandwidth parameter $h = \left(4\gamma \right)^{\frac{1}{\beta}}\left( \log n \right)^{-\frac{1}{\beta}}$ following Fan 
(Theorems \ref{thm:Fan1}, \ref{thm:Fan2}). Plugging these expresions into \eqref{eqn:difference_intermediate} leads to
\begin{align*}
	\Big| \tilde{F}^{(i)}(z)[\zeta^{n}] - \tilde{F}^{(i)}(z)[\zeta^n_j] \Big|
		&\leq \frac{\left( \log n \right)^{\frac{1}{\beta}}}{2\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n} \int_{\tfmin}^{z \wedge \tfmax}  
			\int_{-1}^{1} 2 B \kmax \exp\left( \frac{1}{4} \left|t \right|^{\beta} \log n\right) dt dw\\
		&\leq \frac{ B \kmax \left( \log n \right)^{\frac{1}{\beta}}}{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n} \int_{\tfmin}^{z \wedge \tfmax} 
			\left( 1 - (-1) \right) \max_{t \in [-1,1]}\exp\left( \frac{1}{4} \left|t \right|^{\beta} \log n\right) dw\\
		&= \frac{ B \kmax \left( \log n \right)^{\frac{1}{\beta}}}{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n}  
			\left( \left(z  \wedge \tfmax \right) - \tfmin \right) 2 n^{\frac{1}{4}}\\
		&\leq  \frac{ 2B \kmax (\tfmax - \tfmin) \left( \log n \right)^{\frac{1}{\beta}}}{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n^{\frac{3}{4}}}\\
		&=  \frac{ 2\constdd \left( \log n \right)^{\frac{1}{\beta}}}{n^{\frac{3}{4}}},	\qquad \text{for any }z \in [\tfmin, \tfmax].
\end{align*}
Applying McDiarmid's inequality (Lemma \ref{lem:McDiarmid}), we can conclude that,
\begin{align*}
	\mathbb{P} \bigg( \left| \tilde{F}^{(i)}(z)[\zeta^n] - \bbE_{\zeta^n}{\tilde{F}^{(i)}(z)[\zeta^n]} \right| \geq t \bigg)
		&\leq 2\exp\left( \frac{- n^{1/2} }{2\constdd^2 \left( \log n \right)^{\frac{2}{\beta}}} t^2	 \right).		
\end{align*}
This argument holds even when the generic variable $n$ is replaced with $\left| \cB_i \right|$ for each $i \in [m]$.
\end{proof}

We want to uniformly control the variance over all $z \in [\tfmin, \tfmax]$. Applying the $\varepsilon$-net argument, we obtain the following lemma 
as a corollary of Lemma \ref{lem:concentration_tilde}. Before stating the lemma, we define a function $\textrm{Res}: [n] \to \Reals$ as
\begin{equation}\label{eqn:resolution}
	\res{k} = \frac{ B \kmax  }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  k^{\frac{1}{4}} \left( \log k \right)^{\frac{1}{\beta}}.
\end{equation}

\begin{lemma}[Variance is uniformly small]\label{lem:sup_tilde}
For each $i \in [m]$, for any positive integer $\Nnet$ and for any $t > 0$,
\begin{align*}
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t 
		+  \frac{\res{\numi}\big( \tfmax - \tfmin \big)}{\Nnet} \bigg)^2 ~ \bigg| ~ | \cB_i | = \numi \bigg)
		&\leq 	2 \Nnet \exp\left( \frac{- \numi^{1/2} t^2 }{2 \constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} }  \right).
\end{align*}
\end{lemma}

\begin{proof} [Proof of Lemma \ref{lem:sup_tilde}]
First, we discretize the interval interval $[\tfmin, \tfmax]$ by constructing an $\varepsilon$-net. For any integer $\Nnet \geq 1$, define the set
\[	\cT_{\Nnet} := \left\{ \tfmin + \frac{2k - 1}{2 \Nnet}\left( \tfmax - \tfmin \right),~\forall k \in [\Nnet] \right\}.	\]
Then for any $\Nnet > 0$, $\cT_{\Nnet} \subset [\tfmin, \tfmax]$ and it forms a $\frac{\big( \tfmax - \tfmin \big)}{2\Nnet}$-net with $\left| \cT_{\Nnet} \right| = \Nnet$, 
i.e., for any $z \in \left[\tfmin, \tfmax\right]$, there exists $k \in [\Nnet]$ such that $\left| z - \frac{2k - 1}{2\Nnet}\left( \tfmax - \tfmin \right) \right| 
\leq \frac{\left( \tfmax - \tfmin \right)}{2\Nnet}$.

Next, we observe that
\begin{align*}
	\left\| \tilde{f}^{(i)} \right\|_{\infty} 	&= \bigg\| \frac{1}{h \left| \cB_i \right|} \sum_{j \in \cB_i} L \left( \frac{z - Z(i,j)}{h} \right) \bigg\|_{\infty} \\
		&\leq \frac{1}{h} \left\| L \right\|_{\infty}\\
		&= \frac{1}{2\pi h} \left\| \int_{-\infty}^{\infty} e^{-\img tz} \frac{\phi_K(t)}{\phi_N\left( \frac{t}{h} \right)} dt  \right\|_{\infty}\\
		&\leq \frac{1}{2\pi h} \int_{-\infty}^{\infty} \left| e^{-\img tz} \frac{\phi_K(t)}{\phi_N\left( \frac{t}{h} \right)} \right| dt\\
		&\leq \frac{1}{2\pi h} \int_{-1}^1 \frac{\kmax}{B^{-1} \exp \left(-\gamma \left| \frac{t}{h} \right|^{\beta} \right)} dt\\
		&\leq \frac{B \kmax \left( \log \left| \cB_i \right| \right)^{\frac{1}{\beta}}}{2\pi \left( 4\gamma \right)^{\frac{1}{\beta}} } 
			\int_{-1}^1 \exp\left( \frac{1}{4} \left| t \right|^{\beta} \log \left| \cB_i \right| \right) dt	\\
		&\leq	 \frac{ B \kmax \left( \log \left| \cB_i \right| \right)^{\frac{1}{\beta}}}{2\pi \left( 4\gamma \right)^{\frac{1}{\beta}} } \int_{-1}^1  \left| \cB_i \right|^{\frac{1}{4}} dt\\
		&=	\frac{ B \kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  \left| \cB_i \right|^{\frac{1}{4}} \left( \log \left| \cB_i \right| \right)^{\frac{1}{\beta}} \\
		&= \res{|\cB_i|}.
\end{align*}

When conditioned on $|\cB_i| = \numi$, this upper bound is universal for all realization of $N, M$. Therefore, when conditioned on $|\cB_i| = \numi$,
$\left\| \bbE\big[ \tilde{f}^{(i)} \big] \right\|_{\infty} \leq \res{\numi}$, too. By triangle inequality, $\left\| \tilde{f}^{(i)} - \Exp{ \tilde{f}^{(i)} } \right\|_{\infty} \leq 2 \res{\numi}$ 
and it follows from the definition of $\tilde{F}^{(i)}$ (see \eqref{eqn:ECDF_known_noise}) that 
\[	\sup_{z \in [\tfmin, \tfmax]} \bigg| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \bigg| 
	\leq \sup_{z \in \cT_{\Nnet}} \bigg| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \bigg| +  \frac{ \res{\numi}\big( \tfmax - \tfmin \big)}{\Nnet}.	\]
Therefore, if $\left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \leq \varepsilon$ for all $z \in \cT_n$, the supremum over the whole domain is bounded above 
up to an additional discretization error term. That is to say,  
\[	\sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \leq \varepsilon + \frac{\res{\numi} \big( \tfmax - \tfmin \big)}{\Nnet}.	\]
An application of the union bound on the contraposition of the previous statement yields
\begin{align*}
	&\Prob{ \sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t  
		+ \frac{\res{\numi}\big( \tfmax - \tfmin \big)}{\Nnet} ~ \bigg| ~ |\cB_i | = \numi }\\
		&\qquad\leq \Prob{ \sup_{z \in \cT_{\Nnet}} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t }\\
		&\qquad\leq \sum_{z \in \cT_{\Nnet}} \Prob{ \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t }\\
		&\qquad\leq  2 \Nnet \exp\left( \frac{- \numi^{1/2} t^2 }{2 \constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} } \right).
\end{align*}		
\end{proof}
	
	
	
	


\subsection{Proof of Lemma \ref{lem:cdf_noisy_known}}\label{sec:proof_cdf_known}
%\begin{lemma}\label{lem:cdf_noisy_known}
%	For any $i \in [m]$, and for any $t > 0$,
%	\begin{align*}
%		&\bbP \bigg( \sup_{z \in [\tfmin, \tfmax]} \big| \tilde{F}^{(i)} (z) - F^{(i)}(z) \big| > t + (\constcc + \constdd) \left( \log \numi \right)^{-1/\beta}
%			~ \bigg| ~ |\cB_i | = \numi \bigg)
%			\leq 2  \numi^{\frac{1}{4}} \left( \log \numi \right)^{\frac{2}{\beta}}
%				\exp\left( \frac{- \numi^{1/2} }{2 \constdd^2\left( \log \numi \right)^{\frac{2}{\beta}}} t^2 \right).
%	\end{align*}
%\end{lemma}

\begin{proof}[Proof of Lemma \ref{lem:cdf_noisy_known}]
We put Lemma \ref{lem:mean_difference_tilde} and Lemma \ref{lem:sup_tilde} together by applying the union bound. 
For any $\delta_1, \delta_2 > 0$, suppose that both $\left| F^{(i)} (z) - \Exp{\tilde{F}^{(i)} (z)} \right| \leq \delta_1$ and 
$\left| \tilde{F}^{(i)} (z) - \Exp{\tilde{F}^{(i)} (z)} \right| \leq \delta_2$ are satisfied. Then $\left| \tilde{F}^{(i)} (z) - F^{(i)} \right|
\leq \delta_1 + \delta_2$ by triangle inequality. Therefore, we can obtain the desired concentration inequality by applying 
the union bound on the contraposition of the above statement. 

Specifically, when $| \cB_i | = \numi$, we choose $\delta_1 = \constcc \left( \log \numi \right)^{-1/\beta}$ and $\delta_2 
= t + \frac{\res{\numi}\big( \tfmax - \tfmin \big)}{\Nnet}$ where $\Nnet = \numi^{\frac{1}{4}} \left( \log \numi \right)^{\frac{2}{\beta}}$. 
Note that $ \frac{\res{\numi}\big( \tfmax - \tfmin \big)}{  \numi^{\frac{1}{4}} \left( \log \numi \right)^{\frac{2}{\beta}} } = \constdd  
\left( \log \numi \right)^{-1/\beta}$. Therefore,
\begin{align*}
	&\Prob{\sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)} (z) - F^{(i)} \right| > t + (\constcc + \constdd) \left( \log \numi \right)^{-1/\beta} ~\bigg| ~ | \cB_i | = \numi }\\
		&\qquad \leq \Prob{\sup_{z \in [\tfmin, \tfmax]}\left| F^{(i)} (z) - \Exp{\tilde{F}^{(i)} (z)} \right| > \constcc \left( \log \numi \right)^{-1/\beta} ~ \bigg| ~ |\cB_i | = \numi}\\
		&\qquad \quad+ \Prob{\sup_{z \in [\tfmin, \tfmax]}\left| \tilde{F}^{(i)} (z) - \Exp{\tilde{F}^{(i)} (z)} \right| 
			> t + \constdd \left( \log \numi \right)^{-1/\beta}~ \bigg| ~ |\cB_i | = \numi}\\
		&\qquad\leq 2 \numi^{\frac{1}{4}} \left( \log \numi \right)^{\frac{2}{\beta}}
			 \exp\left( \frac{- \numi^{1/2} t^2 }{2\constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}}} \right).
\end{align*}
\end{proof}




==> contents/FF1_proof_CDF_unknown_helper.tex <==
\section{Proof of Lemma \lowercase{\ref{lem:cdf_noisy_unknown}}: 
	Reliable CDF Estimation When Noise Distribution is Unknown}\label{sec:proof_noisy_unknown_CDF}
%\DG{***TODO}
%
%\DG{This section is looooooooooooooooooooong}
In this section we prove Lemma \ref{lem:cdf_noisy_unknown}, which provides a uniform probabilistic upper bound on 
the CDF estimate $\hat{F}^{(i)}$. For that purpose, we first show that we can reliably estmate the noise characteristic function. 
Then we show that $\bbE \hat{F}^{(i)}$ is close to $F$. Lastly, we show that $\hat{F}^{(i)}$ concentrates around its 
expectation $\bbE\hat{F}^{(i)}$.

In Section \ref{sec:helper_lemmas}, we present some technical helper lemmas and their proofs. Based on these lemmas, 
we show that our estimate for the noise characteristic function as defined in \eqref{eqn:chN_est} uniformly converges to 
the true noise characteristic function in Section \ref{sec:est_characteristic_ftn}. Then we prove that the ignorance of 
the noise density introduces only a small bias in the CDF estimation by providing an upper bound on 
$\sup_{z \in \Reals}\big| \bbE [\hat{F}^{(i)} (z)] - \bbE[ \tilde{F}^{(i)}(z)] \big|$ in Section \ref{sec:bias_hat_tilde}. 
This observation implies an upper bound on $\sup_{z \in \Reals}\big| \bbE [\hat{F}^{(i)} (z)] - F^{(i)}(z) \big|$ 
in combination with Lemma \ref{lem:mean_difference_tilde}. In Section \ref{sec:unknown_variance}, we verify 
the uniform concentration of $\hat{F}^{(i)}$ to its expectation by the same argument as in Section \ref{sec:known_variance}; 
see Lemmas \ref{lem:concentration_tilde} and \ref{lem:sup_tilde}. In Section \ref{sec:conditioning}, we introduce 
appropriate conditioning events that are used to conclude the proof of Lemma \ref{lem:cdf_noisy_unknown}. 
All of them are high probability events according to the lemmas proved in the section. In the end, 
Lemma \ref{lem:cdf_noisy_unknown} is proved by putting all the lemmas in this section by applying the union bound.

%It is the proof of claim (2), for which most of this section is spared.

\subsection{Helper Lemmas}\label{sec:helper_lemmas}
\subsubsection{The Size of the Base Set $\cT_i$ for Noise Density Estimation}\label{sec:base_size}
Recall that we define the set $\cT_i$ in \eqref{eqn:set_Ti} as a set to estimate the noise distribution by emulating 
the setup of repeated measurements. In this section, we present two lemmas to show that $|\cT_i|$ has an appropriate size. 
On the one hand, Lemma \ref{lem:T_large} shows there are sufficiently many triples in $\cT_i$ enabling the estimation; 
on the other hand, Lemma \ref{lem:T_not_too_big} ensures that there are not too many triples in $\cT \supset \cT_i$ and 
hence we can control all of them simultaneously. 

Later, these lemmas will be used in combination with Lemma \ref{lem:dN_max} to ensure that the noise distribution 
can be estimated from triples in $\cT_i$ with high probability; see Remark \ref{rem:noise_error_control}.
	
\begin{lemma}\label{lem:IandJ}
	The sets $J$ and $I$ defined in Algorithm \ref{alg:setT_main} are sufficiently large with high probability. 
	Specifically, given $m,n,p$, we have
	\begin{align*}
		\mathbb{P}\bigg(|J| \leq \frac{n}{2} \left[ 1 - \exp\left( - \frac{mp}{8} \right) \right] \bigg) 
			&\leq \exp\bigg( - \frac{n}{8} \left[ 1 - \exp\left( - \frac{mp}{8} \right) \right] \bigg),
	\end{align*}
	and given $|J|$,
	\begin{align*}
		\mathbb{P}\bigg(|I| \leq \frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \bigg) 
			&\leq \exp\bigg( - \frac{m}{8} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \bigg).
	\end{align*}
\end{lemma}

\begin{proof}
Recall the construction procedure of the set $\cT$ (see Algorithm \ref{alg:setT_main}).	
The number of column indices in $J$ is given as the sum of indicator variables
\begin{equation}\label{eqn:J}
	|J| := \sum_{j \in [n]} \Ind{\big| \cB^{j} \big| \geq \frac{mp}{2}}.	
\end{equation}
Note that $|\cB^j| = \sum_{i \in [m]} M(i,j)$ is distributed as $Binomial(m, p)$. It follows from the binomial Chernoff bound that
\[	\Prob	{\big| \cB^{j} \big| \geq \frac{mp}{2}	} \geq 1 - \exp\left( - \frac{mp}{8} \right).	\] 
Therefore, we can view the $n$ indicator variables in \eqref{eqn:J} as independent Bernoulli variables, each of which 
takes value $1$ with probability greater than $1 - \exp\left( - \frac{mp}{8} \right)$.
		
Therefore, $|J| \sim Binomial(n, p')$ for some $p' \geq 1 - \exp\left( - \frac{mp}{8} \right)$. It follows that
\begin{align*}
	\Prob{|J| \leq \frac{n}{2} \left[ 1 - \exp\left( - \frac{mp}{8} \right) \right] } &\leq \Prob{ |J| \leq \frac{np'}{2}}
		 \leq \exp\left( - \frac{np'}{8} \right) 
		 \leq \exp\left( - \frac{n}{8} \left[ 1 - \exp\left( - \frac{mp}{8} \right) \right] \right).
\end{align*}
		
In the same vein, the number of column indices in $I$ is given as the sum of indicator variables
\[	|I| := \sum_{i \in [m]} \Ind{\left| \cB_{i} \cap J \right| \geq \frac{|J|p}{2}}.	\]
Now $|\cB_i \cap J| = \sum_{j \in J} M(i,j)$ is distributed as $Binomial(m, \tilde{p})$ with $\tilde{p} \geq p$, because 
$\tilde{p} = \Prob{M(i,j) = 1 \left| j \in J \right.} \geq \Prob{M(i,j) = 1} = p$.
These $m$ indicator variables are independent Bernoulli variables, each of which takes value $1$ with probability greater than
\[	\Prob	{\left| \cB_{i} \cap J \right| \geq \frac{|J|p}{2}} 
		\geq \Prob	{\left| \cB_{i} \cap J \right| \geq \frac{|J| \tilde{p}}{2}	}
		\geq 1 - \exp\left( - \frac{|J|\tilde{p}}{8} \right)
		\geq 1 - \exp\left( - \frac{|J|p}{8} \right).	\]
Therefore, $|I| \sim Binomial(m, \tilde{p}')$ with $\tilde{p}' \geq 1 - \exp\left( - \frac{|J|p}{8} \right)$.
It follows that
\begin{align*}
	\mathbb{P}\Bigg( |I| \leq \frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \Bigg) 
		&\leq \mathbb{P}\Big( | I | \leq \frac{m\tilde{p}'}{2} \Big)
		 \leq \exp\left( - \frac{m\tilde{p}'}{8} \right) 
		 \leq \exp\Bigg( - \frac{m}{8} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \Bigg).
\end{align*}
\end{proof}


\begin{lemma}\label{lem:T_large} For any $i \in [m]$, 
	\[	\left| \cT_i \right| \geq 	\Bigg(\frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] - 1 \Bigg)	
		\Bigg\lceil \frac{|J|p}{4} - \frac{1}{2} \bigg( \bigg\lfloor \sqrt{\frac{|J|p}{2}}\bigg\rfloor + 1 \bigg)\Bigg\rceil,	\]
	with probability at least $1 - \exp\Big( - \frac{m}{8} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \Big)$.
\end{lemma}
	
\begin{proof}
Recall the construction procedure of the set $\cT$ and $\cT_i$ described in Algorithm \ref{alg:setT_main}.
Given $i' \in I$, we let $\sigma_{i'}: \cB_{i'} \cap J \to \left[ |\cB_{i'} \cap J | \right]$ denote a map that maps 
the column index in $\cB_{i'} \cap J \subseteq [n]$ to integers $1, 2, \ldots, |\cB_{i'} \cap J |$ such that $\sigma(j_1) < \sigma(j_2)$ implies that $\hat{q}_{\marg}\left( j_1 \right) \leq \hat{q}_{\marg}\left( j_2 \right)$. Note that $\sigma_{i'}$ is a bijection and is invertible where its inverse $\sigma_{i'}^{-1}: [|\cB_{i'} \cap J |] \to \cB_{i'} \cap J \subseteq [n]$.
		
First of all, we show that there cannot exist more than $\left\lfloor \sqrt{\left| \cB_{i'} \cap J \right|} \right\rfloor$ $k$'s (where $k \in \left[ \left| \cB_{i'} \cap J \right| -1 \right]$) such that 
\begin{equation}\label{eqn:bad_condition}
	\Big| \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k+1) \right) - \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k) \right) \Big| 
		> \frac{1}{\sqrt{\left|\cB_{i'} \cap J \right| }}. 
\end{equation}
Let $[a,b)$ denote the half-open interval, that is to say, $[a,b):= \left\{ x \in \Reals : a \leq x < b \right\}$. If $k_1 \neq k_2$, 
\[	
	\Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1 + 1) \right)\Big) 
	\cap \Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2 + 1) \right)\Big) = \emptyset,	
\]
and hence,
\begin{align*}
	&\mu \left( \Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1 + 1) \right)\Big) \cup \Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2 + 1) \right)\Big) \right)\\
		&\qquad = \mu \left( \Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_1 + 1) \right)\Big) \right)
		+ \mu \left(\Big[ \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2) \right), \hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k_2 + 1) \right)\Big) \right),
\end{align*}
where $\mu$ is the Lebesgue measure on $\Reals$, and $\mu \left( [a, b) \right) = ( b -a ) \Ind{b \geq a}$. Let $\cS_{i'}$ 
denote the set of $k$'s in $\left[ \left| \cB_{i'} \cap J \right| -1 \right]$, which satisfies Eq. \eqref{eqn:bad_condition}. 
		
Let's Assume that $ \left| \cS_{i'} \right| \geq \left\lfloor \sqrt{\left| \cB_{i'} \cap J \right|} \right\rfloor + 1$. Since $\hat{q}_{\marg}\left( \sigma_{i'}^{-1}(k) \right) \in [0,1], \forall k \in \big[|\cB_{i'} \cap J | \big]$,
\begin{align*}
	1 	&= \mu \big( [0,1 ) \big)\\
		&\geq \mu \bigg( \bigcup_{k \in \left| \cB_{i'} \right| - 1} 
			\Big[ \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k)\right), \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k+1)\right)  \Big)\bigg)\\
		&\geq \mu \bigg( \bigcup_{k \in \cS_{i'}} \Big[ \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k)\right), 
			\hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k+1)\right)  \Big)  \bigg)\\
		&= \sum_{k \in \cS_{i'}} \Big( \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k+1)\right) 
			- \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k)\right) \Big)\\
		&\geq \left( \left\lfloor \sqrt{\left| \cB_{i'} \cap J \right|} \right\rfloor + 1 \right) 
			\bigg( \frac{1}{\sqrt{\left|\cB_{i'} \cap J \right| }} \bigg)\\
		&> 1,
\end{align*}
which is a contradiction. Therefore, it is proved that $\left| \cS_{i'} \right| \leq \left\lfloor \sqrt{\left|\cB_{i'} \cap J \right| } \right\rfloor.$
For those $k \in \left[ \left|\cB_{i'} \cap J \right| - 1 \right] \setminus \cS_{i'}$, we have 
\[
	\hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k+1)\right)- \hat{q}_{\marg}\left(\sigma_{i'}^{-1}(k)\right) \leq \frac{1}{\sqrt{|\cB_{i'} \cap J |}}.
\] 
In case both $k, k+1\in  \left[ \left|\cB_{i'} \cap J \right| - 1 \right] \setminus \cS_{i'}$, either 
$\big(i', \sigma_{i'}^{-1}(k), \sigma_{i'}^{-1}(k+1)\big) \in \cT$ or $\big(i', \sigma_{i'}^{-1}(k+1), \sigma_{i'}^{-1}(k+2)\big) \in \cT$, 
but not both. However, no more than half of $k \in \big[ \left|\cB_{i'} \cap J \right| - 1 \big] \setminus \cS_{i'}$ is excluded and 
there exist at least $ \Big\lceil \frac{\left|\cB_{i'} \cap J \right| - 1 - \left\lfloor \sqrt{\left|\cB_{i'} \cap J \right| }\right\rfloor}{2}\Big\rceil $ 
number of $k$'s such that $\left(i', \sigma_{i'}^{-1}(k), \sigma_{i'}^{-1}(k+1)\right) \in \cT$.
		
From Lemma \ref{lem:IandJ}, we know that $|I| > \frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right]$ 
with high probability ($i$ might be also in $I$). We also know from the argument above that for each $i' \in I$, 
there exist at least $ \Big\lceil \frac{\left|\cB_{i'} \cap J\right| - 1 - \left\lfloor \sqrt{\left|\cB_{i'}  \cap J \right| }\right\rfloor}{2}\Big\rceil \geq   \Big\lceil \frac{\frac{|J|p}{2} - 1 - \lfloor \sqrt{\frac{|J|p}{2} }\rfloor}{2}\Big\rceil $ number of $k$'s such that $\left(i', \sigma_{i'}^{-1}(k), \sigma_{i'}^{-1}(k+1)\right) \in \cT$. All in all, we can conclude that
\[	
	\left| \cT_i \right| \geq 	\bigg(\frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] - 1 \bigg)	
		\Bigg\lceil \frac{|J|p}{4} - \frac{1}{2} \bigg( \bigg\lfloor \sqrt{\frac{|J|p}{2} }\bigg\rfloor + 1 \bigg)\Bigg\rceil,	
\]
with probability at least $1 - \exp\Big( - \frac{m}{8} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \Big)$.
\end{proof}
	
We have shown that the set $\cT_i$ is sufficiently large with high probability. On the other hand, we can also show that 
$|\cT|$ is not too large compared to the total number of observed entries in the matrix ($=mnp$) with high probability. 
See Lemma \ref{lem:T_not_too_big}.


	
\subsubsection{Useful Properties for Noise Density Estimation Based on $\cT$}\label{sec:control_discrepancy}
		
The set $\cT$ is carefully constructed for estimating the noise distribution. 
For the analysis of the quality of estimated characteristic function of the noise, we define the following quantities: 
for $i \in [m]$, let
\begin{equation}\label{eq:notation_quality_noise}
	\dAi \triangleq \max_{\left(i', j_1, j_2 \right) \in \cT_i} \big| A(i', j_1) - A(i', j_2) \big|,	\qquad\text{and}\qquad
	\dNi \triangleq \max_{\left(i', j_1, j_2 \right) \in \cT_i} \big| N(i', j_1) - N(i', j_2) \big|.
\end{equation}
The following two lemmas show that these two quantities are not too large with high probability. In particular, 
Lemma \ref{lem:dA_max} shows that $\dAi$ is vanishingly small as $m, n \to \infty$, while Lemma \ref{lem:dN_max} 
shows that $\dNi$ scales only logarithmically fast with respect to the size of the set $\cT$. By Lemma \ref{lem:T_not_too_big}, 
this implies that $\dNi$ grows no faster than $\sigma \sqrt{\log(mnp)}$ (up to a multiplicative constant) with high probability.
	
\begin{lemma}\label{lem:dA_max}
	For $t > 0$,
	\begin{align*}
		\Prob{ \dAi > t +  \lipmax \sqrt{\frac{2}{\left| J \right| p}}+ 4\lipmax \Qf\left(\frac{mp}{2}\right)}
		&\leq	\big| J \big| \exp\Bigg( - \frac{n}{8\lipmax^2} \bigg( t + 4\lipmax \Qf\left(\frac{mp}{2}\right) \bigg)^2 \Bigg)
			+ \big| J \big|\exp\left( -\frac{nt}{12\lipmax}\right) .
	\end{align*}
\end{lemma}

\begin{proof}
From the Lipschitz assumption on the latent function, we have
\begin{align*}
	\big| A(i', j_1) - A(i', j_2) \big|	&\leq \lipmax \left| \fcol{j_1} - \fcol{j_2} \right|.
\end{align*}
It suffices to find an upper bound on $\big| \fcol{j_1} - \fcol{j_2} \big|$ to control $\dAi$. However, this is a latent quantity, 
which is not observable from data. Instead, we take a detour using triangle inequality:
\begin{align*}
	\big| \fcol{j_1} - \fcol{j_2} \big|	&\leq  \big| \fcol{j_1} - \hat{q}_{\marg}(j_1) \big| + \Big| \hat{q}_{\marg}(j_1) - \hat{q}_{\marg}(j_2) \Big| + \big| \hat{q}_{\marg}(j_2) - \fcol{j_2} \big| .
\end{align*}
Observe that $\big| \fcol{j} - \hat{q}_{\marg}(j) \big|$ is small for all $j \in J$ due to the concentration of quantile estimates; 
see Lemma \ref{lem:quantile_noisy}. In the rest of the proof, we show $\big| \hat{q}_{\marg}(j_1) - \hat{q}_{\marg}(j_2) \big|$ 
is small for all $(i', j_1, j_2) \in \cT$ because of the careful construction of $\cT$. 
		
First of all, note that $|\cB_i \cap J| \geq \frac{|J|p}{2}$ for any $i \in I$ by construction of $\cT$. Therefore, for any $(i', j_1, j_2) \in \cT$,
\[	
	\big| \hat{q}_{\marg}\left( j_1 \right) - \hat{q}_{\marg}\left( j_2 \right) \big|	
		\leq \frac{1}{\sqrt{\left| \cB_i \cap J \right|}}	
		\leq \sqrt{\frac{2}{\left| J \right| p}}.	
\]
In other words,
\[	\bbP \Bigg( \bigcup_{\left(i', j_1, j_2 \right) \in \cT_i} \bigg\{ \big| \hat{q}_{\marg}\left( j_1 \right) - \hat{q}_{\marg}\left( j_2 \right) \big| > \sqrt{\frac{2}{\left| J \right| p}} \bigg\}\Bigg) = 0.	\]
		
Next, recall the definition of function $\Qf$ from \eqref{eqn:Q_function}:
\[
	\Qf(x) = 2\sqrt{\pi} \left( \frac{1}{\sqrt{\constaa x}} + \frac{1}{\sqrt{\constbb x}} + \frac{e^{\constaa/2}}{\sqrt{mp \constaa }} 
		+  \frac{e^{\constbb/2}}{\sqrt{mp \constbb }} \right).
\]
Note that the set $J$ is defined as $J = \left\{ j \in [n]: |\cB^j| \geq \frac{mp}{2}\right\}$ (see Algorithm \ref{alg:setT_main}). 
By Lemma \ref{lem:quantile_noisy}, for any $t > 4 \Qf(\frac{mp}{2}) = \frac{4\constee}{\sqrt{mp}}$,
\begin{align*}
	\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t ~\bigg|~ j \in J} 
		\leq \exp\left( - \frac{nt^2}{2}  \right) + \exp\left( -\frac{n( \frac{t}{2} - \Qf\left(\frac{mp}{2}\right))}{3} \right).	
\end{align*}
It is worthwhile to remark that $\exp\left( - \frac{mp}{8} \right)$ term is removed from the original statement of Lemma 
\ref{lem:quantile_noisy}. The term was originally introduced from the probability $\Prob{ \Ecol^c }$ (see the Claim 2 
in the proof of Lemma \ref{lem:quantile_noisy}), however, that term disappears here due to the conditioning $j \in J$. 
By applying the union bound, it follows that
\begin{align*}
	\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t, ~\forall j \in J}
	 	&\leq	\sum_{j \in J}	\Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > t ~\bigg|~ j \in J}\\
		&\leq	\big| J \big| \bigg[ \exp\bigg( - \frac{nt^2}{2}  \bigg) 
			+ \exp\bigg( -\frac{n}{3}\Big( \frac{t}{2} - \Qf\left(\frac{mp}{2}\right)\Big) \bigg) \bigg].
\end{align*}
		
From the argument above, if $\big| \hat{q}_{\marg}(j) - \fcol{j} \big| \leq t_1$ for all $j \in J$ and $\big| \hat{q}_{\marg}\left( j_1 \right) 
- \hat{q}_{\marg}\left( j_2 \right) \big| \leq t_2$ for all triple $(i', j_1, j_2) \in \cT$, then $\big| A(i', j_1) - A(i', j_2) \big| 
\leq \lipmax (2t_1 + t_2)$ for all $(i', j_1, j_2) \in \cT$.
Consequently, for $t > \lipmax\sqrt{\frac{2}{\left| J \right| p}}+ 4\lipmax \Qf\left(\frac{mp}{2}\right)$,
\begin{align*}
	&\Prob{ \dAi > t}\\
		&\qquad	= \bbP \bigg( \max_{\left(i', j_1, j_2 \right) \in \cT_i} \big| A(i', j_1) - A(i', j_2) \big| > t \bigg)\\
		&\qquad	\leq\bbP \Bigg( \bigcup_{\left(i', j_1, j_2 \right) \in \cT_i} \left\{ \big| \fcol{j_1} - \fcol{j_2} \big| > \frac{t}{\lipmax} \right\}\Bigg)\\
		&\qquad\leq 	\bbP \Bigg( \bigcup_{\left(i', j_1, j_2 \right) \in \cT_i} \bigg\{ \Big| \hat{q}_{\marg}\left( j_1 \right) 
			- \hat{q}_{\marg}\left( j_2 \right) \Big| > \sqrt{\frac{2}{\left| J \right| p}} \bigg\}\Bigg)
			+ \Prob{ \left| \hat{q}_{\marg}(j) - \fcol{j} \right| > \frac{1}{2} \left[ \frac{t}{\lipmax} 
			- \sqrt{\frac{2}{\left| J \right| p}} \right], ~\forall j \in J}\\
		&\qquad\leq	\big| J \big| \exp\left( - \frac{n}{8\lipmax^2} \left( t - \lipmax\sqrt{\frac{2}{\left| J \right| p}} \right)^2 \right)
			+ \big| J \big|\exp\left( -\frac{n}{12\lipmax} \left( t - \lipmax\sqrt{\frac{2}{\left| J \right| p}} 
			- 4\lipmax \Qf\left(\frac{mp}{2}\right) \right)\right) .	
\end{align*}
Changing the variables $t' = t - \lipmax\sqrt{\frac{2}{\left| J \right| p}}+ 4\lipmax \Qf\left(\frac{mp}{2}\right)$, we conclude the proof.
\end{proof}




\begin{lemma}\label{lem:dN_max}
	$\dNi$ does not exceed $4\sigma \sqrt{\log 4 |\cT| }$ with high probability. Specifically,
	\[	\Prob{ \dNi >  4\sigma \sqrt{\log 4 |\cT| }} \leq \frac{1}{4 |\cT|}.	\]
\end{lemma}
\begin{remark}\label{rem:noise_error_control}
	Combined with Lemmas \ref{lem:T_large} and \ref{lem:T_not_too_big}, Lemma \ref{lem:dN_max} asserts that 
	$ \dNi < 4\sigma \sqrt{\log 4 mnp }$ with high probability, i.e. $1 - O\Big(\frac{1}{mnp}\Big)$.
\end{remark}

\begin{proof}
For any $t > 0$, if $\big| N(i',j_1) \big|, \big| N(i',j_2) \big| \leq \frac{t}{2}$ for all $(i', j_1, j_2) \in \cT$, then $\dNi \leq t$. Considering its contrapositive,
\begin{align*}
	\Prob{ \dNi > t }		
		&\leq	\Prob{\exists (i', j_1, j_2) \in \cT: \big| N(i',j_1) \big| \geq \frac{t}{2} 
			\text{ or } \big| N(i',j_2) \big| \geq \frac{t}{2}}\\
		&\leq	\sum_{(i', j_1, j_2) \in \cT}  \left[ \Prob{ \big| N(i',j_1) \big| \geq \frac{t}{2} } 
			+ \Prob{ \big| N(i',j_2) \big| \geq \frac{t}{2}}\right]\\
		&\leq	2 \big| \cT \big|  \bbP \Big( \big| N(i,j) \big| \geq \frac{t}{2} \Big)\\
		&\leq	4 \big| \cT \big| \exp \left( - \frac{t^2}{8 \sigma^2} \right).
\end{align*}
The last line follows from the sub-gaussianity of the noise and the Chernoff bound. Choosing $t = 4\sigma \sqrt{\log 4 |\cT|}$ completes the proof.
\end{proof}

==> contents/FF2_proof_CDF_unknown_noise_density.tex <==
%%% =======================================================
%%%	Part 2
%%% =======================================================
%\newpage
\subsection{Uniform convergence of $\hat{\phi}(t)$ to $\phi(t)$}\label{sec:est_characteristic_ftn}
\subsubsection{Outline of the section}
Recall the definition of $\hat{F}^{(i)}$ from \eqref{eqn:ECDF_unknown_noise}, \eqref{eqn:unknown_density} and \eqref{eqn:kernel_estimated}:
\[
	\hat{F}^{(i)}(z) = \begin{cases}
		\int_{\tfmin}^{z } \hat{f}^{(i)}(w) dw,	& \text{if } z < \tfmax,\\
		1,							& \text{if } z \geq \tfmax,
	\end{cases}
\]
where
\[
	\hat{f}^{(i)}(z) = \frac{1}{h |\cB_i|} \sum_{j\in \cB_i} \deconvker \left( \frac{z- Z(i,j)}{h} \right), ~\text{where}~ 
	\deconvker(z) = \frac{1}{2\pi} \int e^{-\img tz} \frac{\phi_K(t)}{\hat{\phi}_{N,i}\left(\frac{t}{h}\right) + \rho}dt.
\]
It is defined almost in the same with $\tilde{F}^{(i)}$ defined in \eqref{eqn:ECDF_known_noise} except for that we use $\deconvker$ as the deconvolution kernel 
instead of $L$ defined in \eqref{eqn:kernel_known}. Note that $\deconvker$ is defined with the estimated characteristic function of the noise $\hat{\phi}_{N,i}$ 
instead of the true noise characteristic function $\phi_N$, which is unavailable in the current setup. A ridge parameter $\rho$ is introduced to avoid division-by-zero. 

In this section, we investigate the estimated noise characteristic function $\hat{\phi}_{N, i}(t)$ and conclude that $\hat{\phi}_{N, i}(t)$ uniformly converges to $\phi_N(t)$. 
First, we recall the definition of $\hat{\phi}_{N, i}(t)$ from \eqref{eqn:chN_est}: for $i \in [m]$,
\begin{equation*}
	\hat{\phi}_{N, i}(t) = \bigg| \frac{1}{\left| \cT_i \right|} \sum_{ (i', j_1, j_2 ) \in \cT_i} 
		\cos \Big[ t \big( Z(i', j_1) - Z(i', j_2)  \big) \Big] \bigg|^{1/2},
\end{equation*}
where $\cT_i$ is the set of triples $(i, j_1, j_2)$ such that $A(i, j_1) \approx A(i, j_2)$ as described in Algorithm \ref{alg:setT_main}. Based on the results 
developed in this section, we argue that $\hat{F}^{(i)} \approx \tilde{F}^{(i)}$ in Section \ref{sec:bias_hat_tilde}.

As a tool for analysis, we define 
\begin{equation}\label{eqn:noise_ideal}
	\idealNest(t) = \bigg| \frac{1}{\left| \cT_i \right|} \sum_{ (i', j_1, j_2)  \in \cT_i} \cos \big[ t \left( N(i', j_1) - N(i', j_2)  \right) \big] \bigg|^{1/2}.
\end{equation}
For later use, we also define 
\begin{equation}\label{eqn:Phi_star}
	\IdealNest(t) = \frac{1}{\left| \cT_i \right|} \sum_{ (i', j_1, j_2) \in \cT_i} \cos \big[ t \left( N(i', j_1) - N(i', j_2)  \right) \big],
\end{equation}
so that $\idealNest(t) = \big| \IdealNest(t) \big|^{\frac{1}{2}}$. Note that $\idealNest(t)$ can be thought as an imaginary estimator of $\phi_N$, 
but is not computable (neither is $\IdealNest(t)$) as we do not have access to $N(i,j)$.

This section is organized as follows. First, we show that $\idealNest(t) \approx \phi_N(t)$ in Section \ref{sec:imag_to_true} and that $\hat{\phi}_{N, i}(t)  
\approx \idealNest(t) \approx \phi_N(t)$ in Section \ref{sec:est_to_imag}. Then we conclude that $\hat{\phi}_{N, i}(t) \approx \phi_N(t)$ by combining 
the usual trick of triangle inequality and the union bound, as summarized in Lemma \ref{lem:Ephi}.


\subsubsection{Intermediate Analysis Part I: $\idealNest(t) \approx \phi_N(t)$}\label{sec:imag_to_true}
\begin{lemma}\label{lem:ideal_true}
For any $i \in [m]$ and for any $s > 0$,
%$\idealNest$ is close to $\phi_N$ with high probability. Specifically, for any $t \in \Reals$ 
\begin{align*}
	\Prob{ \big|\IdealNest(t) - \phi_N(t)^2 \big| > s ~ \Big| ~ \big| \cT_i \big| = T_i } 
		\leq 2 \exp \bigg(- \frac{T_i s^2}{2} \bigg).
%	\Prob{\big| \idealNest(t) - \phi_N(t) \big| > s~ \Big| ~ \big| \cT_i \big| = T_i}
%		&\leq 2 \exp \bigg(- \frac{T_i s^4}{2} \bigg).
\end{align*}
\end{lemma}

\begin{proof}
Recall that we assumed supersmooth noise; see\eqref{eqn:model_supersmooth}. Therefore, $\phi_N(t) \geq B^{-1} \exp \left( -\gamma |t|^{\beta} \right) > 0$ 
for all $t \in \Reals$. Also, we observe from \eqref{eqn:noise_ideal} that $\idealNest(t) \geq 0$ for all $t \in \Reals$.
By the trivial inequality that $|a-b| \leq |a+b|$ for $a, b \geq 0$, it follows that
\begin{align*}
	\big| \idealNest(t) - \phi_N(t) \big| &\leq \Big(\big| \idealNest(t) - \phi_N(t) \big| \big| \idealNest(t) + \phi_N(t) \big| \Big)^{\frac{1}{2}}\\
		&= \big| \idealNest(t)^2 - \phi_N(t)^2 \big|^{\frac{1}{2}}\\
		&\leq \big| \IdealNest(t)  - \phi_N(t)^2 \big|^{\frac{1}{2}}.
\end{align*}
for any $t \in \Reals$. The last inequality follows from $\Big| \big| \IdealNest(t)  \big| - \phi_N(t)^2 \Big| \leq \Big| \IdealNest(t) - \phi_N(t)^2 \Big|$, because $\phi_N(t) > 0$.
		
From the symmetry of the noise distribution and the independence between $N(i,j_1)$ and $N(i,j_2)$ for $(i,j_1, j_2) \in \cT_i$, 
\begin{align*}
	\Exp{ \cos \big[ t \left( N(i, j_1) - N(i, j_2)  \right)}
		&= \Exp{ \frac{1}{2} \exp \big( t \left( N(i, j_1) - N(i, j_2) \right)  \big) +  \frac{1}{2} \exp \big( -t \left( N(i, j_1) - N(i, j_2) \right)  \big) }\\
		&= \frac{1}{2} \mathbb{E}\big[tN(i, j_1)\big] \mathbb{E}\big[-tN(i, j_2)\big] + \mathbb{E}\big[-tN(i, j_1)\big] \mathbb{E}\big[tN(i, j_2)\big]\\
		&= \phi_N(t)^2.
\end{align*}
Therefore, $\bbE\big[ \IdealNest(t) \big] = \phi_N(t)^2$ for all $t \in \Reals$.
		
Since $\Big| \cos \big[ t \left( N(i, j_1) - N(i, j_2)  \right) \Big| \leq 1$, we can apply Hoeffding's inequality (Lemma \ref{lem:Hoeffding_bounded}) to achieve 
\[	\Prob{ \big|\IdealNest(t) - \phi_N(t)^2 \big| > s ~ \Big| ~ \big| \cT_i \big| = T_i } 
		\leq 2 \exp \bigg(- \frac{T_i s^2}{2} \bigg), \quad \text{for all }t \in \Reals. 	\]		
%All in all, for any $t \in \Reals$ and for any $s > 0$,
%\begin{align*}
%	\Prob{\big| \idealNest(t) - \phi_N(t) \big| > s~ \Big| ~ \big| \cT_i \big| = T_i}
%		&\leq \Prob{\big| \idealNest(t)^2 - \phi_N(t)^2 \big| > s^2~ \Big| ~ \big| \cT_i \big| = T_i}\\
%		&\leq \Prob{ \big|\IdealNest(t) - \phi_N(t)^2 \big| > s^2~ \Big| ~ \big| \cT_i \big| = T_i }\\
%		&\leq 2 \exp \bigg(- \frac{T_i s^4}{2} \bigg).
%\end{align*}
\end{proof}


Now we make Lemma \ref{lem:ideal_true} uniformly holds for all $t$ in a bounded interval in $\Reals$ by the $\eps$-net argument.
%\DG{definitions?}
For each $i \in [m]$, we define
\begin{equation}\label{eqn:dNi}
	\dNi	\triangleq   \max_{ (i', j_1, j_2) \in \cT_i} \Big| N(i', j_1) - N(i', j_2) \Big|
\end{equation}

\begin{lemma}\label{lem:sup_ideal}
For any $i \in [m]$, for any positive integer $\Nnet$, and for any $\Lambda, s \geq 0$,
\begin{align*}
	\bbP\bigg( \sup_{t \in [-\Lambda, \Lambda]} \big| \idealNest(t) - \phi_N(t) \big|^2
		> s +  \frac{\Lambda}{\Nnet} \big( |\Lambda| \dNi^2 + 2\sigma B \big) ~ \bigg| ~ \big| \cT_i \big| = T_i \bigg)
		\leq 2 \Nnet \exp \bigg(- \frac{T_i s^2}{2} \bigg),
\end{align*}
where $\sigma, B$ are noise model parameters.
\end{lemma}

\begin{proof}
First, we discretize the interval interval $[-\Lambda, \Lambda]$ by constructing an $\varepsilon$-net. For any positive integer $\Nnet$, we define
\begin{equation}\label{eqn:eps_net_Lambda}
	\cT_{\Nnet, \Lambda} \triangleq \left\{ \frac{(2k - 1 - \Nnet)\Lambda}{2\Nnet} \in \Reals ~\text{ such that }~ k \in [\Nnet] \right\}.
\end{equation}
Then $\cT_{\Nnet, \Lambda}$ forms a $\frac{\Lambda}{\Nnet}$-net of $[-\Lambda, \Lambda]$: (1) $\cT_{\Nnet, \Lambda} \subset [-\Lambda, \Lambda]$; 
and (2) for any $z \in [-\Lambda, \Lambda]$, there exists $z' \in \cT_{\Nnet, \Lambda}$ such that $\left| z - z' \right| \leq \frac{\Lambda}{\Nnet}$.
Moreover, $\left| \cT_{\Nnet, \Lambda} \right| = \Nnet$. 

Next, we consider the function $\IdealNest(t) - \phi_N^2(t)$ and its derivative. First, we observe that
\begin{align}
	\bigg| \frac{d}{dt} \IdealNest(t) \bigg|
		&= \bigg|  \frac{1}{\left| \cT_i \right|} \sum_{ \left(i, j_1, j_2) \right) \in \cT_i} \frac{d}{dt} \cos \big[ t  \left( N(i, j_1) - N(i, j_2) \right) \big] \bigg| \nonumber\\
		&= \bigg|  \frac{-1}{\left| \cT_i \right|} \sum_{ \left(i, j_1, j_2) \right) \in \cT_i} \sin \big[ t  \left( N(i, j_1) - N(i, j_2) \right)  \big] \left( N(i, j_1) - N(i, j_2) \right) \bigg| \nonumber\\
		&\leq \max_{ \left(i, j_1, j_2) \right) \in \cT_i} \big| t \big | \big| N(i, j_1) - N(i, j_2) \big|^2	\nonumber\\
		&= |t| \dNi^2.	\label{eqn:rate_upper.1}
\end{align}
Also, we observe that
\begin{align}
	\bigg| \frac{d}{dt}  \phi_N^2(t) \bigg|	
		&= 2 \bigg| \phi_N(t) \frac{d}{dt} \phi_N(t) \bigg|	\nonumber\\
		&\leq 2 \big| \phi_N(t) \big| \bigg| \frac{d}{dt} \int_{-\infty}^{\infty} e^{-\img t x} dF_N(x) \bigg|	\nonumber\\
		&\leq 2 \big| \phi_N(t) \big| \bigg| \int_{-\infty}^{\infty} (-\img x) e^{\img t x} dF_N(x) \bigg|		\qquad\text{by definition of }\phi_N(t)	\nonumber\\
		&\leq 2 \big| \phi_N(t) \big| \int_{-\infty}^{\infty} \big| x \big|  dF_N(x)	\nonumber\\
		&\leq 2\sigma B \exp\big( - \gamma |t|^{\beta} \big).	\label{eqn:rate_upper.2}
\end{align}
The last line follows from the sub-gaussian noise assumption:
\[	\int_{-\infty}^{\infty} \big| x \big|  dF_N(x) = \Exp{ \big| N \big| } \leq \bbE\big[ N^2 \big]^{\frac{1}{2}} \leq \sigma.	\]

By \eqref{eqn:rate_upper.1}, \eqref{eqn:rate_upper.2} and triangle inequality, it follows that
\begin{align*}
	\sup_{t \in [-\Lambda, \Lambda]} \bigg| \frac{d}{dt} \left( \IdealNest(t) - \phi_N^2(t) \right) \bigg|
		&\leq \sup_{t \in [-\Lambda, \Lambda]} \Bigg( \bigg| \frac{d}{dt} \IdealNest(t) \bigg| + \sup_{t \in [-\Lambda, \Lambda]} \bigg| \frac{d}{dt} \phi_N^2(t) \bigg| \Bigg)\\
		&\leq \sup_{t \in [-\Lambda, \Lambda]} \Big(  |t| \dNi^2 + 2\sigma B \exp\big( - \gamma |t|^{\beta} \big) \Big)\\
		&\leq |\Lambda| \dNi^2 + 2\sigma B.
\end{align*}		
Then it follows from the continuity of $\IdealNest(t) - \phi_N^2(t)$ that 
\begin{align}
	\sup_{t \in [-\Lambda, \Lambda]} \Big| \IdealNest(t) - \phi_N^2(t) \Big| 
		&\leq \sup_{t \in \cT_{\Nnet, \Lambda}} \Big| \IdealNest(t) - \phi_N^2(t) \Big| 
			+  \frac{\Lambda}{\Nnet}\sup_{t \in [-\Lambda, \Lambda]} \bigg| \frac{d}{dt} \left( \IdealNest(t) - \phi_N^2(t) \right) \bigg|	\nonumber\\
		&\leq \sup_{t \in \cT_{\Nnet, \Lambda}} \Big| \IdealNest(t) - \phi_N^2(t) \Big| +  \frac{\Lambda}{\Nnet} \big( |\Lambda| \dNi^2 + 2\sigma B \big).	\label{eqn:eps_net.1}
\end{align}
%We let $\left\| \Delta^{* (i)}_{N, \Lambda} \right\|_{\infty}$ denote the upper bound on the error term, i.e., 
%\[	\left\| \Delta^{* (i)}_{N, \Lambda} \right\|_{\infty}:= \frac{\Lambda}{N} \left[ |\Lambda| \dNi^2 + 2\sigma B \right].	\]


Now we observe that $\phi_N(t) > 0$ for all $t \in \Reals$ by the supersmooth assumption described in \eqref{eqn:model_supersmooth}.
Also, $\idealNest(t) = | \IdealNest(t) |^{1/2} \geq 0$ by \eqref{eqn:noise_ideal}, \eqref{eqn:Phi_star}. Therefore, for all $t \in \Reals$,
\[
	 \big| \IdealNest(t) - \phi_N^2(t) \big|  \geq  \big| |\IdealNest(t)| - \phi_N^2(t) \big| 
	 	= \big| \idealNest(t) + \phi_N(t) \big|\big| \idealNest(t) - \phi_N(t) \big| 
		\geq \big| \idealNest(t) - \phi_N(t) \big|^2.
\]
Therefore, for any $s \geq 0$,
\begin{align*}
	&\bbP\bigg( \sup_{t \in [-\Lambda, \Lambda]} \big| \idealNest(t) - \phi_N(t) \big|^2 
		> s +  \frac{\Lambda}{\Nnet} \big( |\Lambda| \dNi^2 + 2\sigma B \big) ~ \bigg| ~ \big| \cT_i \big| = T_i \bigg)\\
		&\qquad\leq \bbP\bigg( \sup_{t \in [-\Lambda, \Lambda]} \big| \IdealNest(t) - \phi_N^2(t) \big| 
			> s +  \frac{\Lambda}{\Nnet} \big( |\Lambda| \dNi^2 + 2\sigma B \big) ~ \bigg| ~ \big| \cT_i \big| = T_i \bigg)\\
		&\qquad\leq \bbP\bigg( \sup_{t \in \cT_{\Nnet, \Lambda}} \big| \IdealNest(t) - \phi_N^2(t) \big| > s ~ \bigg| ~ \big| \cT_i \big| = T_i  \bigg)		
			\qquad\qquad\because\eqref{eqn:eps_net.1}\\
		&\qquad\leq \sum_{t \in  \cT_{\Nnet, \Lambda}} \Prob{ \big| \IdealNest(t) - \phi_N^2(t) \big| > s ~ \Big| ~ \big| \cT_i \big| = T_i }		
			\qquad\qquad\because\text{union bound}\\
		&\qquad\leq 2 \sum_{t \in \cT_{\Nnet, \Lambda}} \exp \bigg(- \frac{T_i s^2}{2} \bigg)		
			\qquad\qquad\qquad\qquad\qquad\because\text{Lemma }\ref{lem:ideal_true}\\
		&\qquad\leq 2 \Nnet \exp \bigg(- \frac{T_i s^2}{2} \bigg).	
			\qquad\qquad\qquad\qquad\because |\cT_{\Nnet, \Lambda}| = \Nnet
\end{align*}
\end{proof}



\subsubsection{Intermediate Analysis Part 2: $\hat{\phi}_{N, i}(t) \approx \idealNest(t)$}\label{sec:est_to_imag}	
In the same manner as we define $\IdealNest$ in \eqref{eqn:Phi_star}, we define
\begin{equation}\label{eqn:Phi}
	\HatNest (t)= \frac{1}{\left| \cT_i \right|} \sum_{ (i', j_1, j_2)  \in \cT_i} \cos \big[ t \left( Z(i', j_1) - Z(i', j_2)  \right) \big],
\end{equation}
so that $\hat{\phi}_{N, i}(t) = \big| \HatNest(t) \big|^{\frac{1}{2}}$. We also define the following quantity for each $i \in [m]$:
\begin{equation}\label{eqn:dAi}
	\dAi	\triangleq   \max_{ (i', j_1, j_2) \in \cT_i} \Big| A(i', j_1) - A(i', j_2) \Big|
\end{equation}

\begin{lemma}\label{lem:practical_ideal}
	For any $i \in [m]$, and for any $s \geq 0$,
	\begin{align*}
		\bbP\bigg( \big| \HatNest (t) - \IdealNest(t)  \big| > s +  \max_{(i', j_1, j_2)\in \cT_i} \frac{t^2}{2} \dAi^2 ~ \bigg|~  |\cT_i| = T_i \bigg)
			\leq 2 \exp \left( - \frac{T_i s^2}{ 2 t^2 \dAi^2 }  \right).
	\end{align*}
\end{lemma}

\begin{proof}
Observe that $\hat{\phi}_{N, i}(t), \idealNest(t) \geq 0$ for all $t \in \Reals$ by definition; see \eqref{eqn:chN_est} and \eqref{eqn:noise_ideal}. 
Therefore, for all $t \in \Reals$,
\begin{align*}
	\Big| \HatNest (t) - \IdealNest(t) \Big|
		&\geq \Big| \big|\HatNest (t)\big| - \big| \IdealNest(t)\big| \Big| 
		= \Big| \hat{\phi}_{N, i}(t)^2 - \idealNest(t)^2 \Big|
		= \Big| \hat{\phi}_{N, i}(t) - \idealNest(t) \Big| \Big| \hat{\phi}_{N, i}(t) + \idealNest(t) \Big|\\
		&\geq \Big| \hat{\phi}_{N, i}(t) - \idealNest(t) \Big|^2.
\end{align*}
In this proof, we establish a high-probability upper bound on $\big| \HatNest (t) - \IdealNest(t) \big|$ by (1) finding an upper bound on its expectation and then 
(2) showing a sharp concentration of $\big| \HatNest (t) - \IdealNest(t) \big|$ to its expectation.

Recall from our model that $Z(i,j) = A(i,j) + N(i,j)$ for $(i,j)$ such that $M(i,j) = 1$. For $(i', j_1, j_2) \in \cT_i$, we can write
\begin{align*}
	Z(i', j_1) - Z(i', j_2) = \big[ N(i', j_1) - N(i', j_2) \big] +  \big[ A(i', j_1) - A(i', j_2) \big].
\end{align*}
Then by definition of $\IdealNest$ and $\HatNest (t)$, and by the trigonometric identity $\cos a - \cos b = -2 \sin \frac{a+b}{2} \sin \frac{a-b}{2}$, 
\begin{align}
	&\HatNest (t) - \IdealNest(t) 		\nonumber\\
		&\qquad	= \frac{1}{\left| \cT_i \right|} \sum_{ \left(i', j_1, j_2) \right) \in \cT_i} 
			\bigg\{ \cos \Big( t \big[ Z(i', j_1) - Z(i', j_2) \big] \Big) - \cos\Big( t \big[ N(i', j_1) - N(i', j_2) \big] \Big)  \bigg\}		\nonumber\\
		&\qquad	= \frac{-2}{\left| \cT_i \right|} \sum_{ \left(i', j_1, j_2) \right) \in \cT_i} \sin \left( t \big[ N(i', j_1) - N(i', j_2) \big]  + \frac{ t \big[ A(i', j_1) - A(i', j_2) \big] }{2}  \right) 
			\sin \left( \frac{ t \big[ A(i', j_1) - A(i', j_2) \big] }{2}\right).	\label{eqn:Phi_difference}
\end{align}
To avoid unnecessary complication, for $(i', j_1, j_2) \in [m] \times [n]^2$, we shall write 
\begin{equation}\label{eqn:Delta_AN}
	\Dijj A \triangleq A(i', j_1) - A(i', j_2)	\qquad\text{and}\qquad	\Dijj N \triangleq N(i', j_1) - N(i', j_2).
\end{equation}

\medskip
{\bf 1) Upper bound on $\bbE \big[ \HatNest (t) - \IdealNest(t) \big]$:} 
First, we note that the noise is independent of the signal (and hence, latent features) in our model. Therefore, $\big\{ N(i',j_1), N(i',j_2) \big\}_{(i',j_1, j_2) \in \cT_i}$ 
is independent of $\big\{ \frow{i'}, \fcol{j_1}, \fcol{j_2} \big\}_{(i', j_1, j_2) \in \cT_i}$. 
Now we consider the conditional expectation of $ \HatNest (t) - \IdealNest(t)$ given the latent features $\frow{1:m}$ and $\fcol{1:n}$. From the symmetry in the noise distribution,
\begin{align*}
	\bbE \Big[ \HatNest (t) - \IdealNest(t) ~\Big|~ \frow{1:m}, \fcol{1:n} \Big]
		&=  \bbE\Bigg[\frac{-2}{\left| \cT_i \right|} \sum_{ \left(i', j_1, j_2) \right) \in \cT_i} \sin \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \sin \bigg( \frac{t \Dijj A}{2}\bigg) 
			~\bigg|~ \frow{1:m}, \fcol{1:n} \Bigg]	\\
		&=  \bbE \Bigg[ \frac{-1}{\left| \cT_i \right|} \sum_{ \left(i', j_1, j_2) \right) \in \cT_i} \left[ \sin \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) + \sin \bigg( -t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \right] \\
				&\qquad\times	\sin \bigg(  \frac{t \Dijj A}{2}\bigg) ~\bigg|~ \frow{1:m}, \fcol{1:n} \Bigg]		\\
		&\stackrel{(a)} {=} \bbE\Bigg[\frac{-2}{\left| \cT_i \right|} \sum_{ \left(i', j_1, j_2) \right) \in \cT_i} \cos \big( t \Dijj N \big) \sin^2 \bigg( \frac{t \Dijj A}{2}\bigg)~\bigg|~ \frow{1:m}, \fcol{1:n} \Bigg].
\end{align*}
Here, (a) follows from the trigonometric identity, $\sin (a + b) + \sin (a - b) = 2 \sin a \cos b$. Since $\big| \cos \big( t \Dijj N \big)  \big| \leq 1$ and 
$ \big| \sin \big( \frac{t \Dijj A}{2}\big) \big| \leq \big| \frac{t \Dijj A}{2} \big|$, it follows that
\begin{align*}
	\bigg| \bbE \Big[ \HatNest (t) - \IdealNest(t) ~\Big|~ \frow{1:m}, \fcol{1:n} \Big] \bigg|
		&\leq \frac{2}{|\cT_i|} \sum_{(i', j_1, j_2) \in \cT_i} \bigg| \frac{t \Dijj A}{2} \bigg|^2\\
		&\leq \max_{(i', j_1, j_2)\in \cT_i} \frac{t^2}{2}\big(A(i', j_1) - A(i', j_2) \big)^2.
\end{align*}
Note that this upper bound is true regardless of $\frow{1:m}, \fcol{1:n}$. Therefore,
\begin{equation}\label{eqn:expectation_term.1}
	\Big| \bbE \big[ \HatNest(t) - \IdealNest(t) \big] \Big|	\leq \max_{(i', j_1, j_2)\in \cT_i} \frac{t^2}{2} \dAi^2.
\end{equation}

\medskip
{\bf 2) Concentration of $ \HatNest(t) - \IdealNest(t) $ to $\bbE \big[ \HatNest (t) - \IdealNest(t) \big]$:} 
Observe from \eqref{eqn:Phi_difference} that $\HatNest (t) - \IdealNest(t) $ is the sum of $|\cT_i|$ independent random variables due to the manner $\cT_i$ is constructed. 
Moreover, each summand is a bounded random variable as $\big| \sin x \big| \leq x \wedge 1$. Then applying the Hoeffding's inequality (Lemma \ref{lem:Hoeffding_bounded}), 
we can see that for any $t \in \Reals$ and any $s \geq 0$,
\begin{align}
	\mathbb{P} \Big( \big|  \HatNest(t) - \IdealNest(t) - \Exp{ \HatNest(t) - \IdealNest(t) } \big| > s \Big)
		&\leq 2 \exp \left( - \frac{ 2 \Big( \frac{|\cT_i| s}{2} \Big)^2}{ \sum_{(i' ,j_1, j_2) \in \cT_i} \big( t \Dijj A \big)^2 }  \right)		\nonumber\\
		&\leq 2 \exp \left( - \frac{ |\cT_i| s^2}{ 2 t^2 \dAi^2 }  \right).		\label{eqn:conc_bound}
\end{align}
		
\medskip
{\bf 3) Concluding the Proof:} 
By the usual argument (triangle inequality + union bound), for any $s \geq 0$,
\begin{align*}
	&\bbP\bigg( \big| \HatNest (t) - \IdealNest(t)  \big| > s +  \max_{(i', j_1, j_2)\in \cT_i} \frac{t^2}{2} \dAi^2 \bigg)\\
		&\qquad\leq \bbP\bigg( \Big| \bbE \big[ \HatNest(t) - \IdealNest(t) \big] \Big|	 >  \max_{(i', j_1, j_2)\in \cT_i} \frac{t^2}{2} \dAi^2 \bigg)
			+ \bbP \bigg( \Big| \big( \HatNest (t) - \IdealNest(t)  \big) - \bbE \big[ \HatNest(t) - \IdealNest(t) \big] \Big| > s \bigg)\\
		&\qquad\leq 2 \exp \left( - \frac{ |\cT_i| s^2}{ 2 t^2 \dAi^2 }  \right).	\qquad\qquad\because \eqref{eqn:expectation_term.1}, ~\eqref{eqn:conc_bound}
\end{align*}

\end{proof}
	
Again, we derive a uniform bound from Lemma \ref{lem:practical_ideal} in the same manner as we obtain Lemma \ref{lem:sup_ideal} out of Lemma \ref{lem:ideal_true}. 
Recall the definition of $\dNi$ and $\dAi$ from \eqref{eqn:dNi} and \eqref{eqn:dAi}, respectively: for each $i \in [m]$,
\begin{equation*}
	\dNi	\triangleq   \max_{ (i', j_1, j_2) \in \cT_i} \Big| N(i', j_1) - N(i', j_2) \Big|		\qquad\text{and}\qquad
	\dAi	\triangleq   \max_{ (i', j_1, j_2) \in \cT_i} \Big| A(i', j_1) - A(i', j_2) \Big|.
\end{equation*}

\begin{lemma}[Uniform convergence of the noise estimate]\label{lem:sup_noise}
For any $i \in [m]$, for any positive integer $\Nnet$, and for any $\Lambda, s \geq 0$,
\begin{align*}
	\bbP\bigg( \sup_{t \in [-\Lambda, \Lambda]} \big| \HatNest (t) - \IdealNest(t)  \big|  
		> s +   \frac{\Lambda^2}{\Nnet} \Big(2 \dNi + \dAi \Big) \dAi ~ \bigg| ~ \big| \cT_i \big| = T_i \bigg)
		\leq 2 \Nnet \exp \left( - \frac{T_i s^2}{ 2 \Lambda^2 \dAi^2 }  \right).
\end{align*}
\end{lemma}

%	\change{We note that, as we refine the net by letting $N \to \infty$, 
%	$\left\| \Delta^{(i)}_N \right\|_{\infty} \to \frac{\Lambda^2 \dAi^2}{2}$, which sets the fundamental lower bound on 
%	$\sup_{t \in [-\Lambda, \Lambda]} \big| \hat{\phi}_{N, i}(t) -  \idealNest(t) \big|$. That is to say, 
%	$\big\| \hat{\phi}_{N, i}(t) -  \idealNest(t) \big\|_{\infty} \approx \Lambda \dAi$. Indeed, such is a limit on 
%	the deconvolution obtained due to the inherent noise represented by term $ \dAi$ and some such limit is naturally expected. }
	We note that, as we refine the net by letting $N \to \infty$, 
	$\left\| \Delta^{(i)}_N \right\|_{\infty} \to \frac{\Lambda^2 \dAi^2}{2}$, which sets the fundamental lower bound on 
	$\sup_{t \in [-\Lambda, \Lambda]} \big| \hat{\phi}_{N, i}(t) -  \idealNest(t) \big|$. That is to say, 
	$\big\| \hat{\phi}_{N, i}(t) -  \idealNest(t) \big\|_{\infty} \approx \Lambda \dAi$. Indeed, such is a limit on 
	the deconvolution obtained due to the inherent noise represented by term $ \dAi$ and some such limit is naturally expected. 

\begin{proof} [Proof of Lemma \ref{lem:sup_noise}]
As in the proof of Lemma \ref{lem:sup_ideal}, we discretize the interval interval $[-\Lambda, \Lambda]$ by constructing an $\varepsilon$-net; see \eqref{eqn:eps_net_Lambda}. 
For any positive integer $\Nnet$, we define $\cT_{\Nnet, \Lambda} \triangleq \left\{ \frac{(2k - 1 - \Nnet)\Lambda}{2\Nnet} \in \Reals ~\text{ such that }~ k \in [\Nnet] \right\}$. 
Observe that $\cT_{\Nnet, \Lambda}$ forms a $\frac{\Lambda}{\Nnet}$-net of $[-\Lambda, \Lambda]$: (1) $\cT_{\Nnet, \Lambda} \subset [-\Lambda, \Lambda]$; 
and (2) for any $z \in [-\Lambda, \Lambda]$, there exists $z' \in \cT_{\Nnet, \Lambda}$ such that $\left| z - z' \right| \leq \frac{\Lambda}{\Nnet}$.
Moreover, $\left| \cT_{\Nnet, \Lambda} \right| = \Nnet$. 
		
Next, we consider the derivative of $\HatNest (t) - \IdealNest(t)$. First, we recall the expression of $\HatNest (t) - \IdealNest(t)$ as written in \eqref{eqn:Phi_difference}
and the notation $\Dijj A$, $\Dijj N$ introduced in \eqref{eqn:Delta_AN}. Then we observe that
\begin{align*}
	\frac{d}{dt} \Big[ \HatNest (t) - \IdealNest(t) \Big]
	&= \frac{d}{dt} \Bigg[  \frac{-2}{| \cT_i |} \sum_{ (i', j_1, j_2) \in \cT_i} \sin \bigg( t \Dijj N + \frac{t \Dijj A}{2}  \bigg) \sin \bigg( \frac{t \Dijj A}{2}\bigg) \Bigg]\\
	&= \frac{-2}{\left| \cT_i \right|} \sum_{ (i', j_1, j_2) \in \cT_i} \Bigg[ \bigg( \Dijj N+ \frac{\Dijj A}{2} \bigg)\cos \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \sin \bigg( \frac{t \Dijj A}{2}\bigg)\\
		&\qquad\qquad\qquad\qquad\qquad\qquad\qquad + \frac{\Dijj A}{2}\sin \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \cos \bigg( \frac{t \Dijj A}{2}\bigg)\Bigg].
\end{align*}
Therefore,
\begin{align*}
	& \sup_{t \in [-\Lambda, \Lambda]} \left| \frac{d}{dt} \Big[ \HatNest (t) - \IdealNest(t) \Big] \right| \\
		&\qquad\stackrel{(a)}{\leq}  2 \sup_{t \in [-\Lambda, \Lambda]} \Bigg\{ \max_{ (i', j_1, j_2) \in \cT_i} 
				\bigg| \Dijj N+ \frac{\Dijj A}{2} \bigg| \bigg| \cos \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \bigg| \bigg| \sin \bigg( \frac{t \Dijj A}{2}\bigg) \bigg|\\
			&\qquad\qquad\qquad\qquad\qquad\qquad\qquad 
				+ \max_{ (i', j_1, j_2) \in \cT_i} \bigg| \frac{\Dijj A}{2} \bigg| \bigg| \sin \bigg( t \Dijj N+ \frac{t \Dijj A}{2} \bigg) \bigg| \bigg| \cos \bigg( \frac{t \Dijj A}{2}\bigg) \bigg| \Bigg\}\\
		&\qquad\stackrel{(b)}{\leq} 2 \sup_{t \in [-\Lambda, \Lambda]} \Bigg\{  \max_{ (i', j_1, j_2) \in \cT_i } 	 \bigg| \Dijj N+ \frac{\Dijj A}{2} \bigg| \bigg| \frac{t \Dijj A}{2}\bigg| 
			+  \max_{ (i', j_1, j_2) \in \cT_i} \bigg| \frac{\Dijj A}{2} \bigg| \bigg| t \Dijj N+ \frac{t \Dijj A}{2} \bigg| \Bigg\}\\
		&\qquad\stackrel{(c)}{\leq} \sup_{t \in [-\Lambda, \Lambda]} \big|t\big| \Big(2 \dNi + \dAi \Big) \dAi\\
		&\qquad\leq \Lambda \Big(2 \dNi + \dAi \Big) \dAi.
\end{align*}
Here, (a) follows from the triangle inequality; (b) follows from the observation that $|\sin x | \leq |x|$ and $|\cos x| \leq 1$; and (c) follows from the definition of $\dNi, \dAi$; 
see \eqref{eqn:dNi} and \eqref{eqn:dAi}.
		
Since the function $\HatNest (t) - \IdealNest(t) $ is continuous, 
\begin{align}
	\sup_{t \in [-\Lambda, \Lambda]} \big| \HatNest (t) - \IdealNest(t)  \big| 
		&\leq \sup_{t \in \cT_{\Nnet, \Lambda}} \big| \HatNest (t) - \IdealNest(t)  \big| 
			+  \frac{\Lambda}{\Nnet}\sup_{t \in [-\Lambda, \Lambda]} \bigg| \frac{d}{dt} \left( \HatNest (t) - \IdealNest(t)  \right) \bigg|	\nonumber\\
		&\leq \sup_{t \in \cT_{\Nnet, \Lambda}} \big| \HatNest (t) - \IdealNest(t)  \big| +  \frac{\Lambda^2}{\Nnet} \Big(2 \dNi + \dAi \Big) \dAi.	\label{eqn:eps_net.2}
\end{align}
Therefore, for any $s \geq 0$,
\begin{align*}
	&\bbP\bigg( \sup_{t \in [-\Lambda, \Lambda]} \big| \HatNest (t) - \IdealNest(t)  \big|  
		> s +   \frac{\Lambda^2}{\Nnet} \Big(2 \dNi + \dAi \Big) \dAi ~ \bigg| ~ \big| \cT_i \big| = T_i \bigg)\\
		&\qquad\leq \bbP\bigg(  \sup_{t \in \cT_{\Nnet, \Lambda}} \big| \HatNest (t) - \IdealNest(t)  \Big| > s ~ \bigg| ~ \big| \cT_i \big| = T_i  \bigg)		
			\qquad\qquad\because\eqref{eqn:eps_net.2}\\
		&\qquad\leq \sum_{t \in  \cT_{\Nnet, \Lambda}} \Prob{ \big| \HatNest (t) - \IdealNest(t)  \big| > s ~ \big| ~ \big| \cT_i \big| = T_i }		
			\qquad\qquad\because\text{union bound}\\
		&\qquad\leq 2 \sum_{t \in \cT_{\Nnet, \Lambda}} \exp \left( - \frac{T_i s^2}{ 2 t^2 \dAi^2 }  \right)		
			\qquad\qquad\qquad\qquad\qquad\because\text{Lemma }\ref{lem:practical_ideal}\\
		&\qquad\leq 2 \Nnet \exp \left( - \frac{T_i s^2}{ 2 \Lambda^2 \dAi^2 }  \right).	
			\qquad\qquad\qquad\qquad\because |\cT_{\Nnet, \Lambda}| = \Nnet
\end{align*}
\end{proof}
	
\subsubsection{Concluding the Section}
We conclude this section with the following lemma, which asserts the uniform convergence of $\hat{\phi}_{N,i}(t)$ to $\phi_N(t)$ for $t \in [-\Lambda, \Lambda]$.

\begin{lemma}\label{lem:Ephi}
	For any $i \in [m]$, for any positive integers $\Nnet$, and for any $\Lambda, s_1, s_2 \geq 0$,
	\begin{align*}
		&\Prob{ \sup_{t \in [-\Lambda, \Lambda]}  \big| \hatNest (t) - \phi_N(t) \big|^2  
			>   s_1 + s_2 + \frac{1}{\Nnet}\Big( \Lambda^2\big(\dAi + \dNi \big)^2 + 2 \Lambda\sigma B \Big) ~ \bigg| ~ \big| \cT_i \big| = T_i } \\
			&\qquad\leq 2 \Nnet \exp \bigg(- \frac{T_i s_1^2}{2} \bigg) + 2 \Nnet \exp \left( - \frac{T_i s_2^2}{ 2 \Lambda^2 \dAi^2 }  \right).
	\end{align*}
\end{lemma}

\begin{proof}
To begin with, we observe that for all $t \in \Reals$,
\begin{align*}
	\big| \hatNest (t) - \phi_N(t) \big|^2 
		&\leq	\big| \hatNest (t) + \phi_N(t) \big|\big| \hatNest (t) - \phi_N(t) \big|	\leq	\big| |\HatNest (t)| - \phi_N(t)^2  \big| 
		\leq	\big| \HatNest (t) - \phi_N(t)^2  \big|	\\
		&\leq \big| \HatNest(t) - \IdealNest(t) \big| + \big| \IdealNest(t)  - \phi_N(t)^2 \big|
\end{align*}
because $\phi_N(t) > 0$ and $ \hatNest (t) \geq 0$; see \eqref{eqn:model_supersmooth} and \eqref{eqn:chN_est}. Taking the supremum over 
$t \in [-\Lambda, \Lambda]$, we obtain 
\[
	\sup_{t \in [-\Lambda, \Lambda]} \big| \hatNest (t) - \phi_N(t) \big|^2  
		\leq \sup_{t \in [-\Lambda, \Lambda]} \big| \HatNest(t) - \IdealNest(t) \big| 
		+ \sup_{t \in [-\Lambda, \Lambda]} \big| \IdealNest(t)  - \phi_N(t)^2 \big|.
\]
Applying the union bound, we know that for any $s'_1, s'_2 \geq 0$,
\begin{align*}
	&\Prob{ \sup_{t \in [-\Lambda, \Lambda]}  \big| \hatNest (t) - \phi_N(t) \big|^2  > s'_1 + s'_2 } \\
		&\qquad\leq \Prob{ \sup_{t \in [-\Lambda, \Lambda]}  \big| \IdealNest(t)  - \phi_N(t)^2 \big| > s'_1}
			+\Prob{ \sup_{t \in [-\Lambda, \Lambda]}  \big| \HatNest(t) - \IdealNest(t) \big| > s'_2} .
\end{align*}
We conclude the proof by applying Lemma \ref{lem:sup_ideal} and \ref{lem:sup_noise} with the choice of 
\[	
	s'_1 = s_1 + \frac{\Lambda}{\Nnet} \big( |\Lambda| \dNi^2 + 2\sigma B \big), \qquad\text{and}\qquad
	s'_2 = s_2 +  \frac{\Lambda}{\Nnet}  \big| \Lambda \big| \Big(2 \dNi + \dAi \Big) \dAi.
\]
\end{proof}

==> contents/FF3_proof_CDF_unknown_conditioning.tex <==
%%% =======================================================
%%%	Part 3
%%% =======================================================
%\newpage
\subsection{Conditioning Events}\label{sec:conditioning}
In this section, we define some events used in our analysis. Given the problem size $m,n$, and the model parameters $p, \sigma, \lipmin$, 
we define the following events. Note that we define $\EcTi$ and $\Ephi$ for each $i \in [m]$, while all the other events are defined 
without dependence on $i \in [m]$.
\begin{align*}
	&\EJ  \triangleq \bigg\{ |J| \geq \frac{1}{4} n \bigg\},\\
	&\EcTi \triangleq \bigg\{ |\cT_i| \geq \frac{1}{512} mnp \bigg\},\\
	&\EcT \triangleq \bigg\{ |\cT| \leq mnp \bigg\},\\
	&\EdA \triangleq \bigg\{ \max_{ (i,j_1, j_2) \in \cT} \big| A(i,j_1) - A(i,j_2) \big| 
		\leq 	 \frac{ 4 \lipmax \constee }{\sqrt{mp}} + 2\sqrt{2} \lipmax \bigg(\frac{1}{\sqrt{np}} + \frac{1}{\sqrt[4]{np}}\bigg)  \bigg\},\\
	&\EdN \triangleq \bigg\{ \max_{ (i,j_1, j_2) \in \cT} \big| N(i,j_1) - N(i,j_2) \big| \leq 	 4\sigma \sqrt{\log (4 mnp) }  \bigg\},\\
	&\Ephi \triangleq \bigg\{ \sup_{t \in [-\Lambda_0, \Lambda_0]}  \big| \hatNest (t) - \phi_N(t) \big|^2  \leq   \valphiAA + \valphiBB  \bigg\}
\end{align*}
where $\Lambda_0 = (4\gamma)^{-\frac{1}{\beta}}(\log n )^{\frac{1}{\beta}}$ and 
\begin{align*}
	\valphiAA	&=	\frac{32 \big( 1 + 4\lipmax(\constee + \sqrt{2}) \big) }{(4\gamma)^{\frac{1}{\beta}}}
		\frac{(\log n )^{\frac{1}{\beta}}}{\sqrt{mnp}} \bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}},	\\
	\valphiBB	&= \frac{1}{n \log(mnp)} \bigg[\frac{16 \big( \lipmax (\constee + \sqrt{2}) + \sigma \big)^2 }{(4\gamma)^{\frac{2}{\beta}}} 
		\log(4mnp) (\log n )^{\frac{2}{\beta}}	+ \frac{2 \sigma B }{(4\gamma)^{\frac{1}{\beta}}}(\log n )^{\frac{1}{\beta}} \bigg],
\end{align*}
as defined in \eqref{eqn:valphi_A}, \eqref{eqn:valphi_B}.
	
%%%	Event 1
\begin{lemma}[Corollary of Lemma \ref{lem:IandJ}]\label{lem:event_J}
Suppose that $p \geq \frac{8 \log 2}{m}$. Then
\begin{equation*}%\label{eqn:EJc}
	\Prob{\EJ^c}  \leq \exp\bigg( - \frac{n}{16} \bigg).
\end{equation*}
\end{lemma}


%%%	Event 2
\begin{lemma}[Corollary of Lemma \ref{lem:T_large}]\label{lem:event_Ti}
Suppose that $m \geq 8$ and $p \geq \frac{16}{n}$. Then
\begin{equation*}%\label{eqn:EcTic}
	\Prob{\EcTi^c \big| \EJ}
		\leq \exp\bigg( - \frac{m}{16} \bigg).	
\end{equation*}
\end{lemma}
\begin{proof}
Conditioned on $\EJ$, $|J| \geq \frac{1}{4}n$, and hence, $|J|p \geq \frac{np}{4}$. Therefore, when conditioned on $\EJ$,
\begin{align*}
	&\frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] - 1  \geq \frac{m}{4} - 1 \geq \frac{m}{8},		\quad \text{and }\\
	&\Bigg\lceil \frac{1}{2} \bigg( \frac{|J|p}{2} - \bigg\lfloor \sqrt{\frac{|J|p}{2}}\bigg\rfloor - 1 \bigg)\Bigg\rceil
		\geq \Bigg\lceil \frac{1}{2} \bigg( \frac{np}{8} - \bigg\lfloor \sqrt{\frac{np}{8}}\bigg\rfloor - 1 \bigg)\Bigg\rceil
		\geq \frac{1}{4} \left( \frac{np}{8} - 1 \right) \geq \frac{np}{64}.
\end{align*}
For any $i \in [m]$ Lemma \ref{lem:T_large} asserts that 
\begin{align*}
	\Prob{\EcTi^c \big| \EJ}
		&= \Prob{ |\cT_i| < \frac{1}{512} mnp ~\bigg|~ |J| \geq \frac{1}{4}n }\\
		&\leq \Prob{ \left| \cT_i \right| < 	\bigg(\frac{m}{2} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] - 1 \bigg)
			\bigg\lceil \frac{|J|p}{4} - \frac{1}{2} \bigg( \bigg\lfloor \sqrt{\frac{|J|p}{2}}\bigg\rfloor + 1 \bigg)\bigg\rceil  ~\bigg|~	|J| \geq \frac{1}{4}n }	\\
		&\leq  \exp\bigg( - \frac{m}{8} \left[ 1 - \exp\left( - \frac{|J|p}{8} \right) \right] \bigg)\bigg|_{|J| \geq \frac{1}{4}n}
		\leq \exp\bigg( - \frac{m}{16} \bigg).
\end{align*}
\end{proof}

%%%	Event 3
\begin{lemma}\label{lem:T_not_too_big}\label{lem:event_T}
Suppose that $m, n, p$ are given. Then
\begin{equation*}%\label{eqn:EcTc}
	\Prob{\EcT^c} 	\leq	\exp \left( - \frac{mnp}{3} \right).	
\end{equation*}
\end{lemma}

\begin{proof}
It is clear from the description of algorithm (see Algorithm \ref{alg:setT_main}) that for each $(i,j)$, there can exist at most 
one element $(i', j_1, j_2) \in \cT$ such that either $(i,j)=(i', j_1)$ or $(i,j) = (i', j_2)$. Moreover, if there exists $(i', j_1, j_2)$ 
satisfying either of those two conditions, $M(i,j) = 1$. As a result, $|\cT| \leq \frac{1}{2} \sum_{i,j} M(i,j)$, which is the sum of 
$mn$ independent and identically distributed Bernoulli random variable with probability $p$. Applying the binomial 
Chernoff bound yields
\[	
	\Prob{\EcT^c} = \Prob{|\cT| > mnp} 
		\leq 	\bbP \bigg( \sum_{i,j} M(i,j) > 2 mnp \bigg) 
		\leq \exp \left( - \frac{mnp}{3} \right).
\]
\end{proof}

%%%	Event 4
\begin{lemma}\label{lem:event_dA}
For given $m, n, p$,
\begin{equation*}%\label{eqn:EdAc}
	\Prob{ \EdA^c | \EJ }	 \leq  n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg).
\end{equation*}
\end{lemma}

\begin{proof}
Conditioned on $\EJ$, $|J| \geq \frac{n}{4}$. Also, recall from \eqref{eqn:Q_function} that 
$ \Qf\left(\frac{mp}{2}\right) = \frac{\constee}{\sqrt{mp}}$. Therefore, 
\begin{equation}\label{eqn:intermediate_event4}
	\lipmax\sqrt{\frac{2}{\left| J \right| p}}+ 4\lipmax \Qf\left(\frac{mp}{2}\right)
		\leq  \frac{2\lipmax\sqrt{2}}{\sqrt{np}} + 4\lipmax \constee \frac{1}{\sqrt{mp}}
		= 2\lipmax \bigg( \frac{2\constee}{\sqrt{mp}} +  \frac{\sqrt{2}}{\sqrt{np}}\bigg).
\end{equation}
We also note that for any $i \in [m]$, 
\begin{equation}\label{eqn:max_A_Ti_T}
	\dAi = \max_{ (i',j_1, j_2) \in \cT_i} \big| A(i', j_1) - A(i', j_2) \big| \leq \max_{ (i,j_1, j_2) \in \cT} \big| A(i,j_1) - A(i,j_2) \big|.
\end{equation}
Then it follows that
\begin{align*}
	\Prob{ \EdA^c | \EJ }	
	&=	\Prob{\max_{ (i,j_1, j_2) \in \cT} \big| A(i,j_1) - A(i,j_2) \big| 
		> 2\lipmax \bigg( \frac{2\constee}{\sqrt{mp}} +  \frac{\sqrt{2}}{\sqrt{np}}\bigg) + \frac{2 \sqrt{2}\lipmax}{\sqrt[4]{np}} ~\bigg|~ |J| \geq \frac{n}{4}}	\\
	&\stackrel{(a)}{\leq}		\Prob{\max_{ (i,j_1, j_2) \in \cT} \big| A(i,j_1) - A(i,j_2) \big| 
		> \lipmax \sqrt{\frac{2}{\left| J \right| p}}+ 4\lipmax \Qf\left(\frac{mp}{2}\right) + \frac{2 \sqrt{2}\lipmax}{\sqrt[4]{np}} ~\bigg|~ |J| \geq \frac{n}{4}}\\
	&\stackrel{(b)}{\leq}	\big| J \big| \exp\Bigg( - \frac{n}{8\lipmax^2} \bigg( \frac{2 \sqrt{2}\lipmax}{\sqrt[4]{np}}  + 4\lipmax \Qf\left(\frac{mp}{2}\right) \bigg)^2 \Bigg)
		+ \big| J \big|\exp\left( -\frac{n}{12\lipmax} \frac{2 \sqrt{2}\lipmax}{\sqrt[4]{np}} \right) \\
	&\stackrel{(c)}{\leq} n \exp\Bigg( - \frac{n}{8\lipmax^2} \bigg( \frac{2 \sqrt{2}\lipmax}{\sqrt[4]{np}} \bigg)^2 \Bigg)
		+ n \exp\left( -\frac{n^{\frac{3}{4}}}{3 \sqrt{2} ~p^{\frac{1}{4}}} \right) \\
	&\stackrel{(d)}{\leq} n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg).
\end{align*}
We use \eqref{eqn:intermediate_event4} in (a); the inequality in (b) follows from Lemma \ref{lem:dA_max}; (c) follows from the fact that $J \subset [n]$, 
i.e., $|J| \leq n$ and that $\Qf\left(\frac{mp}{2}\right) \geq 0$; and (d) is trivial because $0 \leq p \leq 1$.
\end{proof}


%%%	Event 5
\begin{lemma}\label{lem:event_dN}
Given $m, n, p$, for any $i \in [m]$,
\begin{equation*}%\label{eqn:EdNc}
	\Prob{\EdN^c ~\big|~ \EcTi, \EcT }	 \leq   \frac{128}{mnp}.
\end{equation*}
\end{lemma}
\begin{proof}
Note that $|\cT| \geq |\cT_i| \geq \frac{mnp}{512}$ when conditioned on $\EcTi$ for any $i \in [m]$. Also, we observe that $|\cT| \leq mnp$ 
when conditioned on $\EcT$. 
\begin{align*}
	\Prob{\EdN^c ~\big|~ \EcTi, \EcT }
		&=\Prob{  \max_{ (i,j_1, j_2) \in \cT} \big| N(i,j_1) - N(i,j_2) \big| > 4\sigma \sqrt{\log (4 mnp) }  ~\Big|~ \EcTi, \EcT }\\
		&\stackrel{(a)}{\leq} \Prob{ \dNi  > 4\sigma \sqrt{\log (4 mnp) }  ~\Big|~ \EcTi, \EcT }\\
		&\stackrel{(b)}{\leq} \Prob{ \dNi  > 4\sigma \sqrt{\log 4 |\cT| }   ~\Big|~ \EcTi, \EcT }\\
		&\stackrel{(c)}{\leq} \frac{1}{4 |\cT|} \bigg|_{\EcTi, \EcT}\\
		&\stackrel{(d)}{\leq} \frac{128}{mnp}.
\end{align*}
Here, (a) follows from the definition of $\dNi$ and the inclusion relation $\cT_i \subset \cT$ (see \eqref{eqn:max_A_Ti_T}); we use 
$|\cT| \geq \frac{mnp}{512}$ in (b) and (d); and (c) is implied by Lemma \ref{lem:dN_max}.
\end{proof}



\begin{remark}
	Let $\Theta = \{ \frow{1}, \ldots, \frow{m}, \fcol{1}, \ldots, \fcol{n} \}$ denote the latent variables. 
	We note that the probabilistic tail bounds in Lemmas \ref{lem:event_J}, \ref{lem:event_Ti}, \ref{lem:event_T}, 
	\ref{lem:event_dA}, \ref{lem:event_dN} are derived in the manner that are independent of the latent variables $\Theta$. 
	Therefore, the upper bounds hold regardless of the value $\Theta$ take, i.e., the upper bounds are still valid 
	even if conditioned on $\Theta$.
\end{remark}


\begin{lemma}\label{lem:Ephi_small}
For all $i \in [m]$,
\begin{equation*}
	\Prob{ \Ephi^c \big| \EcTi, \EdA, \EdN}	\leq \frac{128}{mnp}.
\end{equation*}
\end{lemma}

\begin{proof}
To begin with, we recall that given $i \in [m]$,
\begin{align}
	\text{when conditioned on }&\EcTi,	&|\cT_i|	&\geq 	\frac{mnp}{512},	\label{eqn:condition_Ti}\\
	\text{when conditioned on }&\EdA,	&\dAi	&\leq		 \frac{ 4 \lipmax \constee }{\sqrt{mp}} 
		+ 2\sqrt{2} \lipmax \bigg(\frac{1}{\sqrt{np}} + \frac{1}{\sqrt[4]{np}}\bigg),	\label{eqn:condition_dAi}\\
	\text{when conditioned on }&\EdN,	&\dNi	&\leq		4\sigma \sqrt{\log (4 mnp) }.	\label{eqn:condition_dNi}
\end{align}
Next, we let 
\begin{align*}
	\Nnet &=	n \log(mnp),\\
	s_1	&=	\frac{32}{\sqrt{mnp}} \bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}},	\\
	s_2	&=	\frac{32}{\sqrt{mnp}} \bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}} 
				\bigg(\frac{\log n }{4\gamma}\bigg)^{\frac{1}{\beta}}  
				\bigg[ \frac{ 4 \lipmax \constee }{\sqrt{mp}} + 2\sqrt{2} \lipmax \bigg(\frac{1}{\sqrt{np}} + \frac{1}{\sqrt[4]{np}}\bigg)\bigg].
\end{align*}
Note that the kernel bandwidth parameter $h = (4\gamma)^{\frac{1}{\beta}}(\log | \cB_i | )^{-\frac{1}{\beta}}$ and that we are letting 
$\Lambda = (4\gamma)^{-\frac{1}{\beta}}(\log n )^{\frac{1}{\beta}} \geq \frac{1}{h}$. It is easy to verify the following:
\begin{align}
	s_1^2 &= \frac{1024}{mnp} \log\Big( \frac{\Nnet mnp}{32} \Big)
		\stackrel{(a)}{\geq} \frac{2}{|\cT_i|}  \log\Big( \frac{\Nnet mnp}{32} \Big),	\label{eqn:observ_s1}\\
	s_2^2 &= \frac{1024}{mnp} \log\Big( \frac{\Nnet mnp}{32} \Big) \frac{1}{h^2}
		\bigg[ \frac{ 4 \lipmax \constee }{\sqrt{mp}} + 2\sqrt{2} \lipmax \bigg(\frac{1}{\sqrt{np}} + \frac{1}{\sqrt[4]{np}}\bigg)\bigg]^2
		\stackrel{(b)}{\geq} \frac{\dAi^2}{h^2}\frac{2}{|\cT_i|}  \log\Big( \frac{\Nnet mnp}{32} \Big),	\label{eqn:observ_s2}
\end{align}
where (a) is true when conditioned on $\EcTi$; and (b) is true when conditioned on $\EcTi$ and $\EdA$. 
See \eqref{eqn:condition_Ti} and \eqref{eqn:condition_dAi}. By the observations in \eqref{eqn:observ_s1} and \eqref{eqn:observ_s2},
\[
	2 \Nnet \exp \bigg(- \frac{ |\cT_i| s_1^2}{2} \bigg) + 2 \Nnet \exp \bigg( - \frac{|\cT_i| s_2^2}{ 2 \Lambda^2 \dAi^2 }  \bigg)
		\leq \frac{128}{mnp}.
\]

Lastly, we observe that when $p \geq \max\big\{ \frac{1}{m}, \frac{1}{n} \big\}$,
\begin{align*}
	&s_2	\leq \frac{128 \lipmax (\constee + \sqrt{2})}{\sqrt{mnp}} \bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}} 
				\bigg(\frac{\log n }{4\gamma}\bigg)^{\frac{1}{\beta}},	\qquad\text{and}\\
	&\dAi + \dNi
		\leq 4 \big( \lipmax (\constee + \sqrt{2}) + \sigma \big) \sqrt{\log(4mnp)}
\end{align*}
because $\frac{1}{\sqrt{mp}}, \frac{1}{\sqrt{np}}, \frac{1}{\sqrt[4]{np}} \leq 1 \leq \sqrt{\log(4mnp)}$. Then it follows that
\begin{align*}
	&s_1 + s_2	
		\leq \frac{32 \big( 1 + 4\lipmax(\constee + \sqrt{2}) \big) }{(4\gamma)^{\frac{1}{\beta}}}
		\frac{(\log n )^{\frac{1}{\beta}}}{\sqrt{mnp}} \bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}}	\qquad\text{and}\\
	&\frac{1}{\Nnet}\Big( \Lambda^2 \big(\dAi + \dNi \big)^2 + 2 \Lambda \sigma B \Big)\\
		&\qquad\leq \frac{1}{n \log(mnp)} \bigg[\frac{16 \big( \lipmax (\constee + \sqrt{2}) + \sigma \big)^2 }{(4\gamma)^{\frac{2}{\beta}}} 
		\log(4mnp) (\log n )^{\frac{2}{\beta}}	+ \frac{2 \sigma B }{(4\gamma)^{\frac{1}{\beta}}}(\log n )^{\frac{1}{\beta}} \bigg].
\end{align*}
Then the conclusion follows from Lemma \ref{lem:Ephi}.
\end{proof}


==> contents/FF4_proof_CDF_unknown_bias_variance.tex <==
%%% =======================================================
%%%	Part 4
%%% =======================================================
%\newpage
\subsection{Support Lemma to Control the Bias from $\tilde{F}$ to $\hat{F}$}\label{sec:bias_hat_tilde}
Recall the definition of $\tilde{F}^{(i)}$ and $\hat{F}^{(i)}$ from \eqref{eqn:ECDF_known_noise} and \eqref{eqn:ECDF_unknown_noise}. 
In this section, we argue that $\bbE \hat{F}^{(i)}(z)$ is uniformly (with respect to $z \in \Reals$) close to $\bbE\tilde{F}^{(i)}(z)$ in expectation. 
	
\begin{lemma}[Bias is small]\label{lem:hat_tilde}
Let $h$ and $\rho$ denote the kernel bandwidth parameter and the ridge parameter used to define $\hat{F}^{(i)}$ in \eqref{eqn:ECDF_unknown_noise}. 
Then for all $i \in [m]$,
\begin{align*}
	\bigg| \sup_{z \in \Reals} \Exp{\hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z) }\bigg|
		\leq	\frac{\kmax(\tfmax - \tfmin)}{ \pi h } \max_{t \in [-1, 1]} \Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg|.
\end{align*}
\end{lemma}
	
\begin{proof}[Proof of Lemma \ref{lem:hat_tilde}]
First, we observe from the definition of $\tilde{F}^{(i)}$ and $\hat{F}^{(i)}$ (see \eqref{eqn:ECDF_known_noise} and \eqref{eqn:ECDF_unknown_noise}) that given $i \in [m]$,
\begin{align}
	\hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z)
		&= \int_{\tfmin}^{z \wedge \tfmax} \hat{f}^{(i)}(w) - \tilde{f}^{(i)}(w) dw	\nonumber\\
		&= \int_{\tfmin}^{z \wedge \tfmax} \frac{1}{ h |\cB_i|} \sum_{j \in \cB_i}
			\bigg[ \hat{L} \left( \frac{w - Z(i,j)}{h} \right) - L \left( \frac{w - Z(i,j)}{h} \right) \bigg] dw	\nonumber\\
		&= \frac{1}{2\pi h |\cB_i|} 
		\Bigg( \int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} e^{-\img t \frac{w - Z(i,j)}{h}} \left[ \frac{\phi_K(t)}{\hat{\phi}_{N,i}(\frac{t}{h}) + \rho} - \frac{\phi_K(t)}{\phi_N(\frac{t}{h}) } \right] dt~dw \Bigg)	\label{eqn:term.integral}
\end{align}

Now we consider the conditional expectation of \eqref{eqn:term.integral}. We let $\Flatent = \{ \frow{1}, \ldots, \frow{m}, \fcol{1}, \ldots, \fcol{n} \}$ denote the latent variables.
Noting that the support of $\phi_K$ is contained in $[-1,1]$ and that the integrand is a bounded continuous function, we exchange the order of integrals in \eqref{eqn:term.integral}:
\begin{align}
	&\Exp{ \hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z)  }\nonumber\\
		&= \frac{1}{2\pi h |\cB_i|} 	\int_{\tfmin}^{z \wedge \tfmax} \bbE\Bigg[ \sum_{j \in \cB_i} \int_{-\infty}^{\infty} 
			e^{-\img t \frac{w - Z(i,j)}{h}} \phi_K(t) \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}dt \Bigg] dw	\nonumber\\
		&= \frac{1}{2\pi h |\cB_i|} 	\int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \bbE\Bigg[ \int_{-\infty}^{\infty} e^{-\img t \frac{w - Z(i,j)}{h}} \phi_K(t) 
			\frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}dt  \Bigg] dw	\nonumber\\
		&=\frac{1}{2\pi h |\cB_i|} 	 \int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} \bbE \Bigg[ e^{-\img t \frac{w - Z(i,j)}{h}} \phi_K(t) 
			\frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]} \Bigg] dt~dw	\nonumber\\
		&=\frac{1}{2\pi h |\cB_i|} 	 \int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} \bbE_{\Theta} \Bigg[ \bbE \Bigg[ e^{-\img t \frac{w - Z(i,j)}{h}} \phi_K(t) 
			\frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]} ~\bigg|~ \Flatent \Bigg] \Bigg] dt~dw	\nonumber\\
		&\stackrel{(a)}{=} \frac{1}{2\pi h |\cB_i|} 	\int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} e^{-\img t \frac{w}{h}}\phi_K(t)  
			\bbE_{\Theta} \Bigg[ \bbE\big[ e^{\img \frac{t}{h}Z(i,j)} ~\big|~ \Flatent \big]	
			\bbE\bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]} ~\bigg|~ \Flatent \bigg] \Bigg]dt~dw.	\label{eqn:term.integral2}
\end{align}
Here, (a) follows from the conditional independence between $Z(i,j)$ and $\hatNest(t)$. Observe that $\hatNest(t)$ is a function of $\{ N(i',j_1) - N(i',j_2)\}_{(i',j_1, j_2) \in \cT_i}$. 
By the construction of the set $\cT_i$ described in \eqref{eqn:set_Ti}, $\cT_i$ is conditionally independent of $Z(i',j)$ with $i' = i$ when conditioned on the latent variables $\Flatent$. 
Therefore, $\hatNest(t)$ is conditionally independent of $Z(i,j)$ for any $j \in [n]$, too.

Now we observe that $Z(i,j) = A(i,j) + N(i,j) = g(\frow{i}, \fcol{j}) + N(i,j)$ when conditioned on $\Theta$. Therefore,
and therefore,
\begin{align}
	\Exp{ e^{\img \frac{t}{h}Z(i,j)} ~\big| ~ \Theta} &= \Exp{ e^{\img \frac{t}{h}A(i,j)}e^{\img \frac{t}{h}N(i,j)} ~\big| ~ \Theta}
		= e^{\img \frac{t}{h}g(\frow{i}, \fcol{j})}	\Exp{e^{\img \frac{t}{h}N(i,j)} ~\big|~\Theta}
		= e^{\img \frac{t}{h}g(\frow{i}, \fcol{j})}	\Exp{e^{\img \frac{t}{h}N(i,j) } }		\nonumber\\
		&= e^{\img \frac{t}{h}g(\frow{i}, \fcol{j})}\phi_N\bigg( \frac{t}{h} \bigg).			\label{eqn:mgf_condition}
\end{align}
By \eqref{eqn:term.integral2} and \eqref{eqn:mgf_condition},
\begin{align}
	\Exp{\hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z) }
		&= \frac{1}{2\pi h |\cB_i|} 	\int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} \bbE\Big[ e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}} \Big] \phi_K(t)  \phi_N\Big(\frac{t}{h}\Big)
			\bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{\phi_N(\frac{t}{h}) \big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]} \Bigg] dt~dw	\nonumber\\
		&= \frac{1}{2\pi h |\cB_i|} 	\int_{\tfmin}^{z \wedge \tfmax} \sum_{j \in \cB_i} \int_{-\infty}^{\infty} \bbE \Big[ e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}} \Big] \phi_K(t) 
			\bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] dt~dw.	\label{eqn:bias_hat_tilde_intermediate}
\end{align}
Next, we take supremum over $z \in \Reals$ to obtain
\begin{align*}
	&\bigg| \sup_{z \in \Reals} \Exp{\hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z) } \bigg|	\\
	&\leq	 \frac{1}{2\pi h}	\Bigg| \sup_{z \in \Reals}   \int_{\tfmin}^{z \wedge \tfmax}  \frac{1}{ |\cB_i|} \sum_{j \in \cB_i}  \int_{-\infty}^{\infty} \bbE\Big[e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}} \Big] \phi_K(t)
		\bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] dt~dw \Bigg|		\\
	&\leq	\frac{\tfmax - \tfmin}{ 2 \pi h } \max_{j \in \cB_i} \int_{-\infty}^{\infty} \Bigg| \bbE \Big[ e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}} \Big] \phi_K(t) 
		\bbE \Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg| dt		\\
	&\leq	\frac{\tfmax - \tfmin}{ 2 \pi h } \int_{-\infty}^{\infty} \max_{j \in \cB_i}  \bigg| \bbE\Big[e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}}\Big] \bigg| \big| \phi_K(t) \big| 
		\Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg| dt		\\
	&\leq	\frac{\tfmax - \tfmin}{ 2 \pi h } \int_{-\infty}^{\infty} \max_{j \in \cB_i}  \bbE\bigg[  \Big|e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}}\Big| \bigg] \big| \phi_K(t) \big| 
		\Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg| dt		\\
	&\stackrel{(a)}{\leq}	\frac{\tfmax - \tfmin}{ 2 \pi h } \int_{-\infty}^{\infty} \big| \phi_K(t) \big| 
		\Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg| dt		\\
	&\stackrel{(b)}{\leq}	\frac{\tfmax - \tfmin}{ 2 \pi h } \int_{-1}^{1} \kmax \Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg| dt			\\
	&\leq	\frac{\kmax(\tfmax - \tfmin)}{ \pi h } \max_{t \in [-1, 1]} \Bigg| \bbE\Bigg[ \frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \Bigg] \Bigg|.	
\end{align*}
Here, (a) follows from that $ \Big| e^{\img t \frac{g(\frow{i}, \fcol{j}) - w}{h}} \Big| \leq 1$; and (b) follows from that $\phi_K(t) = 0$ for $t \not\in [-1, 1]$ and that $\kmax=\max_{t \in [-1,1]} \left| \phi_K(t) \right|$.
\end{proof}


%%%	====================================================
%%%	Conditioned version
%%%	====================================================
\subsubsection{Further Simplification by Conditioning on $\Ephi$}
\begin{lemma}[Bias is small]\label{lem:bias_hat_conditioned}
Given $i \in [m]$, let the kernel bandwidth parameter $h = (4\gamma)^{\frac{1}{\beta}}(\log |\cB_i|)^{-\frac{1}{\beta}}$ 
and the ridge parameter $\rho = |\cB_i|^{-\frac{7}{24}}$. Then
\begin{align*}
	&\bbP\Bigg( \bigg| \sup_{z \in \Reals} \Exp{\hat{F}^{(i)}(z) - \tilde{F}^{(i)}(z) }\bigg| \\
	&\qquad\qquad> \frac{2B \kmax(\tfmax - \tfmin)}
	{ \pi (4\gamma)^{\frac{1}{\beta}} } \Big( |\cB_i|^{\frac{1}{4}} \big( \valphi \big) + |\cB_i|^{-\frac{1}{24}}\Big)(\log |\cB_i|)^{\frac{1}{\beta}} 
	~\bigg|~ \Ephi\Bigg)	 = 0.
\end{align*}
\end{lemma}

Note that $\Big( |\cB_i|^{\frac{1}{4}} \big( \valphi \big) + |\cB_i|^{-\frac{1}{24}}\Big) =\cO \Big(\frac{1}{n^{1/4} \sqrt{mp}} \log^{\frac{1}{2} 
+ \frac{2}{\beta}}(mn^2 p )+ \frac{1}{n^{3/4}} \log^{\frac{3}{\beta}} n\Big)$; see \eqref{eqn:valphi_A}, \eqref{eqn:valphi_B}, and Remark \ref{rem:valphi}.

\begin{proof}
First, we note that
\[	
	\frac{ \phi_N(\frac{t}{h}) -\big[ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho \big]}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } 
	= \frac{ \phi_N(\frac{t}{h}) - \hat{\phi}_{N,i}(\frac{t}{h}) -  \rho }{ \phi_N(\frac{t}{h}) - \big[ \phi_N(\frac{t}{h}) - \hat{\phi}_{N,i}(\frac{t}{h}) - \rho \big] }.
\]
Then we observe from the supersmooth assumption on the noise (cf. \eqref{eqn:model_supersmooth}) that
\begin{equation}\label{eqn:lower_phiN}	
	\phi_N \left(\frac{t}{h} \right)  \geq \frac{1}{B}\exp\bigg(- \gamma \Big|\frac{t}{h}\Big|^{\beta} \bigg) 
		= \frac{1}{B}\exp \bigg(- \frac{1}{4} t^{\beta} \log |\cB_i| \bigg)
	 	= \frac{1}{B} |\cB_i|^{-\frac{1}{4}t^{\beta}} \geq \frac{1}{B} |\cB_i|^{-\frac{1}{4}},		\qquad\text{for all }t \in [-1, 1].
\end{equation}

Note that when conditioned on $\Ephi$,
\begin{equation}\label{eqn:upper_phi_hphi}
	\max_{t \in [-1, 1]}\bigg| \phi_N \Big(\frac{t}{h} \Big) - \hat{\phi}_{N,i} \Big(\frac{t}{h} \Big) \bigg| \leq \valphi.
\end{equation} 
Since we choose the ridge parameter $\rho = |\cB_i|^{-\frac{7}{24}}$ in our algorithm,
\[	\bigg| \phi_N \Big(\frac{t}{h} \Big) \bigg| \geq 2 \bigg( \bigg| \phi_N \Big(\frac{t}{h}\Big) - \hat{\phi}_{N,i}\Big(\frac{t}{h}\Big)\bigg| + \rho \bigg)
		\geq 2 \bigg|~ \phi_N \Big(\frac{t}{h}\Big) - \hat{\phi}_{N,i}\Big(\frac{t}{h}\Big) - \rho~ \bigg|,	\qquad\text{ for all } t \in [-1, 1].	\]
Therefore,
\begin{align}
	\max_{t \in [-1, 1]} \left| \frac{ \phi_N(\frac{t}{h}) - \hat{\phi}_{N,i}(\frac{t}{h}) - \rho}{ \hat{\phi}_{N,i}(\frac{t}{h}) + \rho } \right|
		&\leq \max_{t \in [-1, 1]} \left| \frac{ \phi_N(\frac{t}{h}) - \hat{\phi}_{N,i}(\frac{t}{h}) - \rho}{ \frac{1}{2}\phi_{N}(\frac{t}{h}) } \right|
				\nonumber\\
		&\leq 2 \max_{t \in [-1, 1]} \Bigg( \bigg|\phi_N \Big(\frac{t}{h}\Big) \bigg|^{-1} 
			\bigg|\phi_N \Big(\frac{t}{h}\Big) - \hat{\phi}_{N,i}\Big(\frac{t}{h}\Big) - \rho \bigg| \Bigg)	
				\nonumber\\
		&\leq  2  \max_{t \in [-1, 1]} \Bigg( \bigg|\phi_N \Big(\frac{t}{h}\Big) \bigg|^{-1} \Bigg)
			\max_{t \in [-1, 1]} \Bigg( \bigg|\phi_N \Big(\frac{t}{h}\Big) - \hat{\phi}_{N,i}\Big(\frac{t}{h}\Big) \bigg| \Bigg) 
			+ 2\rho \max_{t \in [-1, 1]} \Bigg( \bigg|\phi_N \Big(\frac{t}{h}\Big) \bigg|^{-1} \Bigg) 
				\nonumber\\
		&\stackrel{(a)}{\leq} 2B |\cB_i|^{\frac{1}{4}} \big( \valphi \big)	+ 2 B |\cB_i|^{-\frac{1}{24}}	\label{eqn:term_upper}
\end{align}
when conditioned on $\Ephi$; (a) follows from \eqref{eqn:lower_phiN}, \eqref{eqn:upper_phi_hphi}, and the choice of the 
ridge parameter $\rho = |\cB_i|^{-\frac{7}{24}}$.

Inserting \eqref{eqn:term_upper} to the upper bound stated in Lemma \ref{lem:hat_tilde} concludes the proof.
\end{proof}
		

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Support Lemma to Control the Variance of $\hat{F}^{(i)}$}\label{sec:unknown_variance}
	
\begin{lemma}[Variance is small]\label{lem:concentration_hat}
	For $i \in [m]$, let $\hat{F}^{(i)}$ be defined as in \eqref{eqn:ECDF_unknown_noise}. Then for any $t > 0$, 
	\begin{align*}
		\mathbb{P} \bigg( \left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \geq t ~ \bigg| ~ | \cB_i | = \numi \bigg)	
			&\leq 2\exp\left( \frac{- \numi^{5/12} }{2\constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} } t^2	 \right).
	\end{align*}
\end{lemma}
	
\begin{proof} [Proof of Lemma \ref{lem:concentration_hat}]
We follow the same logic as in the proof of Lemma \ref{lem:concentration_tilde}. Recall that when conditioned on $\frow{i}$, 
the kernel smoothed ECDF $\hat{F}^{(i)}$ evaluated at $z$ is a function of $\left| \cB_i \right|$ independent random variables 
$\{Z(i, j)\}_{j \in \cB_i}$, i.e., when $z$ is fixed, $\hat{F}^{(i)}(z): \Reals^{\left| \cB_i \right|} \to \Reals$ such that
\begin{align*}
	\hat{F}^{(i)}(z)\left[ Z(i,j_1), \ldots, Z(i,j_{\left| \cB_i \right|}) \right] 
		& = \int_{\tfmin}^{z \wedge \tfmax} \frac{1}{h \left| \cB_i \right|} \sum_{j\in \cB_i} \hat{L} \left( \frac{w- Z(i,j)}{h} \right) dw,	
\end{align*}
where $\hat{L}(z) = \frac{1}{2\pi} \int e^{-\img tz} \frac{\phi_K(t)}{\hat{\phi}_N\left(\frac{t}{h}\right)+\rho}dt$ and $h$ is the bandwidth parameter for kernel $K$. 

First, we show that $\hat{F}^{(i)}(z)$ satisfies the bounded difference condition (see Eq. \eqref{eqn:bounded_difference}). 
Let $\zeta^{n} = (\zeta_1, \ldots, \zeta_n)$ and $\zeta^{n}_j = (\zeta_1, \ldots, \zeta_j', \ldots, \zeta_{n})$ be two $n$-tuples of real numbers, 
which differ only at the $j$-th position. Then
\begin{align}
	\Big| \hat{F}^{(i)}(z)[\zeta^{n}] - \hat{F}^{(i)}(z)[\zeta^n_j] \Big|
		&= \Bigg| \frac{1}{h n} \int_{\tfmin}^{z \wedge \tfmax}  \hat{L} \left( \frac{w- \zeta_j}{h} \right) - \hat{L} \left( \frac{w- \zeta'_j}{h} \right) dw \Bigg|		\nonumber\\
		&= \Bigg| \frac{1}{h n} \int_{\tfmin}^{z \wedge \tfmax}  \frac{1}{2\pi} \int \Big(e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big) 
			\frac{\phi_K(t)}{\hat{\phi}_N\left(\frac{t}{h}\right) + \rho}dt dw \Bigg|		\nonumber\\
		&\leq \frac{1}{2\pi h n} \int_{\tfmin}^{z \wedge \tfmax}  \int \Big|e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big| 
			\left|\frac{\phi_K(t)}{\hat{\phi}_N\left(\frac{t}{h}\right) + \rho} \right| dt dw.	\label{eqn:difference_intermediate.unknown}
\end{align}
Since $e^{-\img tz}$ is on the unit circle in the complex plane for any real numbers $t$ and $z$, we have 
\begin{align*}
	\Big|e^{-\img t \frac{w- \zeta_j}{h} } - e^{-\img t \frac{w- \zeta'_j}{h} }\Big| 
		&\leq \Big|e^{-\img t \frac{w- \zeta_j}{h} }\Big| + \Big| e^{-\img t \frac{w- \zeta'_j}{h} }\Big|  = 2.
\end{align*}

Note that $\phi_K$ is supported within $[-1,1]$ and $\phi_K(t) = 0$ for $t \not\in [-1,1]$. Also, observe that $\hat{\phi}_N \left( \frac{t}{h} \right) \geq 0$ 
for all $t$ by definition, and hence, $\hat{\phi}_N \left( \frac{t}{h} \right) + \rho \geq \rho$. We choose the ridge parameter $\rho = n^{-7/24}$ (here, $n = |\cB_i|$, 
which stands for the number of samples in a row) and the bandwidth parameter $h = \left(4\gamma \right)^{\frac{1}{\beta}}\left( \log n \right)^{-\frac{1}{\beta}}$ 
following Fan (Theorems \ref{thm:Fan1}, \ref{thm:Fan2}). Plugging these expresions into \eqref{eqn:difference_intermediate.unknown} leads to
\begin{align*}
	\Big| \hat{F}^{(i)}(z)[\zeta^{n}] - \hat{F}^{(i)}(z)[\zeta^n_j] \Big|
		&\leq \frac{\left( \log n \right)^{\frac{1}{\beta}}}{2\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n} \int_{\tfmin}^{z \wedge \tfmax}  
			\int_{-1}^{1} 2 \kmax n^{7/24} dt dw\\
		&\leq \frac{ \kmax \left( \log n \right)^{\frac{1}{\beta}}}{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n^{17/24}} \int_{\tfmin}^{z \wedge \tfmax} 
			\left( 1 - (-1) \right)  dw\\
		&\leq \frac{ 2 \kmax (\tfmax - \tfmin ) \left( \log n \right)^{\frac{1}{\beta}}}{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} n^{17/24}}  \\
		&=   \frac{ 2 \constdd \left( \log n \right)^{\frac{1}{\beta}}}{ n^{17/24}} ,	
			\qquad \text{for any }z \in [\tfmin, \tfmax].
\end{align*}

Applying McDiarmid's inequality (Lemma \ref{lem:McDiarmid}), we can conclude that,
\begin{align*}
	\mathbb{P} \bigg( \left| \hat{F}^{(i)}(z)[\zeta^n] - \bbE_{\zeta^n}{\hat{F}^{(i)}(z)[\zeta^n]} \right| \geq t \bigg)
		&\leq 2\exp\left( \frac{- n^{5/12} }{2\constdd^2 \left( \log n \right)^{\frac{2}{\beta}}} t^2	 \right).		
\end{align*}
This argument holds for every $i \in [m]$, with the generic variable $n$ replaced by the corresponding $ |\cB_i|$.
\end{proof}

We want to uniformly control the variance over all $z \in [\tfmin, \tfmax]$. Applying the $\varepsilon$-net argument, we obtain the following lemma 
as a corollary of Lemma \ref{lem:concentration_hat}. We define $\widehat{\textrm{Res}}: [n] \to \Reals$ in a similar manner as we define $\textrm{Res}$ in \eqref{eqn:resolution}:
\begin{equation}\label{eqn:resolution_hat}
	\hres{k} =  \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  k^{\frac{7}{24}} \left( \log k \right)^{\frac{1}{\beta}}.
\end{equation}

\begin{lemma}[Variance is uniformly small]\label{lem:sup_hat}
For each $i \in [m]$, for any positive integer $\Nnet$ and for any $t > 0$,
\begin{align*}
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t 
		+  \frac{\hres{\numi}\big( \tfmax - \tfmin \big)}{\Nnet} ~ \bigg| ~ | \cB_i | = \numi \bigg)
		&\leq 	2 \Nnet \exp\left( \frac{- \numi^{5/12} t^2 }{2 \constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} }  \right).
\end{align*}
\end{lemma}

\begin{proof} [Proof of Lemma \ref{lem:sup_hat}]
Again, the proof has the same structure as in the proof of Lemma \ref{lem:sup_hat}]. For any given positive integer $\Nnet \geq 1$, define the set
\[	\cT_{\Nnet} := \left\{ \tfmin + \frac{2k - 1}{2 \Nnet}\left( \tfmax - \tfmin \right),~\forall k \in [\Nnet] \right\}.	\]
Then for any $\Nnet > 0$, $\cT_{\Nnet} \subset [\tfmin, \tfmax]$ and it forms a $\frac{\big( \tfmax - \tfmin \big)}{2\Nnet}$-net with $\left| \cT_{\Nnet} \right| = \Nnet$, 
i.e., for any $z \in \left[\tfmin, \tfmax\right]$, there exists $k \in [\Nnet]$ such that $\left| z - \frac{2k - 1}{2\Nnet}\left( \tfmax - \tfmin \right) \right| 
\leq \frac{\left( \tfmax - \tfmin \right)}{2\Nnet}$.

Next, we observe that
\begin{align*}
	\left\| \hat{f}^{(i)} \right\|_{\infty} 	
		&= \bigg\|\frac{1}{h \left| \cB_i \right|} \sum_{j \in \cB_i} \hat{L} \left( \frac{z - Z(i,j)}{h} \right) \bigg\|_{\infty}\\
		&\leq \frac{1}{h} \big\| \hat{L} \big\|_{\infty}
		= \frac{1}{2\pi h} \bigg\| \int_{-\infty}^{\infty} e^{-\img tz} \frac{\phi_K(t)}{\hat{\phi}_{N,i}\left( \frac{t}{h} \right) + \rho } dt  \bigg\|_{\infty}\\
		&\leq \frac{1}{2\pi h} \int_{-\infty}^{\infty} \big| e^{-\img tz}\big| \bigg| \frac{\phi_K(t)}{\hat{\phi}_{N,i}\left( \frac{t}{h} \right) + \rho } \bigg| dt\\
		&\leq \frac{1}{2\pi h} \int_{-\infty}^{\infty} \bigg| \frac{\phi_K(t)}{\rho } \bigg| dt		\qquad\qquad\qquad\because \hat{\phi}_{N,i}\left( \frac{t}{h} \right) \geq 0\\
		&\leq \frac{1}{2\pi h} \int_{-1}^1 \kmax \left| \cB_i \right|^{\frac{7}{24}} dt\\%
		&\leq \frac{ \left( \log \left| \cB_i \right| \right)^{\frac{1}{\beta}}}{2\pi \left( 4\gamma \right)^{\frac{1}{\beta}} } \int_{-1}^1 \kmax \left| \cB_i \right|^{\frac{7}{24}}  dt	
				\qquad\because	h = \left( 4\gamma\right)^{\frac{1}{\beta}} \left( \log \left| \cB_i \right| \right)^{-\frac{1}{\beta}}	\\
		&\leq \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  \left| \cB_i \right|^{\frac{7}{24}} \left( \log \left| \cB_i \right| \right)^{\frac{1}{\beta}} \\
		&= \hres{ |\cB_i| }.
\end{align*}


When conditioned on $|\cB_i| = \numi$, this upper bound is universal for all realization of $N, M$. Therefore, when conditioned on $|\cB_i| = \numi$,
$\left\| \bbE\big[ \hat{f}^{(i)} \big] \right\|_{\infty} \leq \hres{\numi}$, too. By triangle inequality, $\left\| \hat{f}^{(i)} - \Exp{ \hat{f}^{(i)} } \right\|_{\infty} 
\leq 2 \hres{\numi}$ and it follows from the definition of $\hat{F}^{(i)}$ (see \eqref{eqn:ECDF_unknown_noise}) that 
\[	\sup_{z \in [\tfmin, \tfmax]} \bigg| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \bigg| 
	\leq \sup_{z \in \cT_{\Nnet}} \bigg| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \bigg| +  \frac{ \hres{\numi}\big( \tfmax - \tfmin \big)}{\Nnet}.	\]
Therefore, if $\left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \leq \varepsilon$ for all $z \in \cT_n$, the supremum over the whole domain is bounded above 
up to an additional discretization error term. That is to say,  
\[	\sup_{z \in [\tfmin, \tfmax]} \left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \leq \varepsilon + \frac{\hres{\numi} \big( \tfmax - \tfmin \big)}{\Nnet}.	\]
An application of the union bound on the contraposition of the previous statement yields
\begin{align*}
	&\Prob{ \sup_{z \in [\tfmin, \tfmax]} \left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \geq t  
		+ \frac{\hres{\numi}\big( \tfmax - \tfmin \big)}{\Nnet} ~ \bigg| ~ |\cB_i | = \numi }\\
		&\qquad\leq \Prob{ \sup_{z \in \cT_{\Nnet}} \left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \geq t }\\
		&\qquad\leq \sum_{z \in \cT_{\Nnet}} \Prob{ \left| \hat{F}^{(i)}(z) - \Exp{\hat{F}^{(i)}(z)} \right| \geq t }\\
		&\qquad\leq  2 \Nnet \exp\left( \frac{- \numi^{5/12} t^2 }{2 \constdd^2 \left( \log \numi \right)^{\frac{2}{\beta}} } \right).
\end{align*}		
\end{proof}



==> contents/FF5_proof_CDF_unknown.tex <==
%%% =======================================================
%%%	Part 5
%%% =======================================================
%\newpage	
\subsection{Completing the Proof of Lemma \ref{lem:cdf_noisy_unknown}}


\begin{proof}[Proof of Lemma \ref{lem:cdf_noisy_unknown}]
We observe that $\hat{F}^{(i)}(z) = F^{(i)}(z) = 0$ for all $z \leq \tfmin$ and $\hat{F}^{(i)}(z) = F^{(i)}(z) = 1$ for all $z \geq \tfmax$. Therefore,
\[	\sup_{z \in \Reals} \big| \hat{F}^{(i)} (z) - F^{(i)}(z) \big| = \sup_{z \in [\tfmin, \tfmax] } \big| \hat{F}^{(i)} (z) - F^{(i)}(z) \big|.	\]
By the usual trick of telescoping (and then applying triangle inequality), we have
\begin{align}
	&\sup_{z \in [\tfmin, \tfmax] } \big| \hat{F}^{(i)} (z) - F^{(i)}(z) \big|	\label{eqn:triangle}\\
		&\qquad\leq \sup_{z \in [\tfmin, \tfmax] } \big| \hat{F}^{(i)} (z) - \Exp{ \hat{F}^{(i)} (z)} \big|
			+ \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{ \hat{F}^{(i)} (z) - \tilde{F}^{(i)}(z) } \big|
			+ \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{\tilde{F}^{(i)}(z)} - F^{(i)}(z) \big|.	\nonumber
\end{align}
Applying the union bound, the following inequality follows from \eqref{eqn:triangle}. For any $t \geq 0$ and any $s_1, s_2, s_3 \geq 0$,
\begin{align}
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \hat{F}^{(i)} (z) - F^{(i)}(z) \big| > t + s_1 + s_2 + s_3 \bigg)
		&\leq 	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \hat{F}^{(i)} (z) - \Exp{ \hat{F}^{(i)} (z)} \big| > t + s_1 \bigg)		\label{eqn:hat_term.1}\\
		&\quad + 	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{ \hat{F}^{(i)} (z) - \tilde{F}^{(i)}(z) } \big| > s_2 \bigg)		\label{eqn:hat_term.2}\\
		&\quad + 	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{\tilde{F}^{(i)}(z)} - F^{(i)}(z) \big| > s_3 \bigg).			\label{eqn:hat_term.3}
\end{align}
We establish upper bounds on the terms in \eqref{eqn:hat_term.1}, \eqref{eqn:hat_term.2}, and \eqref{eqn:hat_term.3} separately.

\paragraph
{\bf Upper bound on \eqref{eqn:hat_term.1}} 
We apply Lemma \ref{lem:sup_hat} with $\Nnet = |\cB_i|$ and
\[	s_1 =  \frac{ \hres{|\cB_i|}( \tfmax - \tfmin )}{\Nnet}
		= \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  \frac{\left( \log |\cB_i| \right)^{\frac{1}{\beta}}}{ |\cB_i|^{\frac{17}{24}}}
\]
where $\hres{|\cB_i|} =  \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  |\cB_i|^{\frac{7}{24}} \left( \log |\cB_i| \right)^{\frac{1}{\beta}}$; 
recall the definition of $\hres{k}$ from \eqref{eqn:resolution_hat}. Then for any $t \geq 0$,
\begin{align*}
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax]} \left| \tilde{F}^{(i)}(z) - \Exp{\tilde{F}^{(i)}(z)} \right| \geq t + s_1 \bigg)
		&\leq 	2 |\cB_i| \exp\left( \frac{- |\cB_i|^{5/12} t^2 }{2 \constdd^2 \left( \log |\cB_i| \right)^{\frac{2}{\beta}} }  \right). 
\end{align*}
by Lemma \ref{lem:sup_hat}.

\paragraph
{\bf Upper bound on \eqref{eqn:hat_term.2}} 
We choose $s_2 = \constcc \big( \log |\cB_i| \big)^{-\frac{1}{\beta}}$. Then it follows from Lemma \ref{lem:mean_difference_tilde} that
\[
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{ \hat{F}^{(i)} (z) - \tilde{F}^{(i)}(z) } \big| > s_2 \bigg) = 0.
\]

\paragraph
{\bf Upper bound on \eqref{eqn:hat_term.3}} 
By the law of total probability and the trivial upper bound on probability, the following inequality holds:
\begin{align*}
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{\tilde{F}^{(i)}(z)} - F^{(i)}(z) \big| > s_3 \bigg)
		&\leq \bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{\tilde{F}^{(i)}(z)} - F^{(i)}(z) \big| > s_3 ~\Big|~ \Ephi \bigg)
			+ \bbP \big( \Ephi^c \big).
\end{align*}
We choose 
\[	s_3 =  \frac{2B \kmax(\tfmax - \tfmin)}
	{ \pi (4\gamma)^{\frac{1}{\beta}} } \Big( |\cB_i|^{\frac{1}{4}} \big( \valphi \big) + |\cB_i|^{-\frac{1}{24}}\Big)(\log |\cB_i|)^{\frac{1}{\beta}}
\]
so that 
\[
	\bbP\bigg( \sup_{z \in [\tfmin, \tfmax] } \big| \Exp{\tilde{F}^{(i)}(z)} - F^{(i)}(z) \big| > s_3 ~\Big|~ \Ephi \bigg) = 0
\] 
by Lemma \ref{lem:bias_hat_conditioned}. 


Now it remains to find an upper bound on $ \bbP \big( \Ephi^c \big)$. We observe that
\begin{align}
	\Prob{\Ephi^c} 	&\leq	\Prob{\Ephi^c \Big| \EcTi \cap \EdA \cap \EdN} + \Prob{\EcTi^c \cup \EdA^c \cup \EdN^c}		\nonumber\\
		&= \Prob{\Ephi^c \Big| \EcTi \cap \EdA \cap \EdN} + \Prob{\EcTi^c \cup \EdA^c} + \Prob{\EdN^c \cap \EcTi}.	\label{eqn:prob_E6}
\end{align}
First of all, by Lemma \ref{lem:Ephi_small},
\begin{equation}\label{eqn:prob_E6.1}
	\Prob{\Ephi^c \Big| \EcTi \cap \EdA \cap \EdN} \leq \frac{128}{mnp}.
\end{equation}
Second, we note that
\begin{align}
	\Prob{\EcTi^c \cup \EdA^c}
		&\leq \Prob{\EJ^c} + \Prob{\EcTi^c \cup \EdA^c ~\big|~ \EJ}		\nonumber\\
		&\leq \Prob{\EJ^c} + \Prob{\EcTi^c ~\big|~ \EJ} + \Prob{\EdA^c ~\big|~ \EJ}	\nonumber\\
		&\leq \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg)
			+ n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)		\label{eqn:prob_E6.2}
\end{align}
because
\begin{align*}
	\Prob{\EJ^c}  			&\leq \exp\bigg( - \frac{n}{16} \bigg)		
		&&\text{by Lemma \ref{lem:event_J}},\\
	\Prob{\EcTi^c \big| \EJ}	&\leq \exp\bigg( - \frac{m}{16} \bigg)	
		&&\text{by Lemma \ref{lem:event_Ti}},\\	%when } m \geq 8 \text{ and } p \geq \frac{16}{n}\\
	\Prob{ \EdA^c | \EJ }	 	&\leq  n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)
		&&\text{by Lemma \ref{lem:event_dA}}.
\end{align*}
Lastly,
\begin{align}
	\Prob{\EdN^c \cap \EcTi}
		&\leq \Prob{\EdN^c \cap \EcTi \cap \EcT} + \Prob{\EcT^c}		\nonumber\\
		&= \Prob{\EdN^c \big| \EcTi \cap \EcT} \Prob{\EcTi \cap \EcT} + \Prob{\EcT^c}	\nonumber\\
		&\leq \Prob{\EdN^c \big| \EcTi \cap \EcT} + \Prob{\EcT^c}		\nonumber\\
		&\leq  \frac{128}{mnp} + \exp \left( - \frac{mnp}{3} \right)		\label{eqn:prob_E6.3}
\end{align}
because 
\begin{align*}
	&\Prob{\EcT^c}  				\leq \exp \left( - \frac{mnp}{3} \right)		
		&&\text{by Lemma \ref{lem:event_T}},\\
	&\Prob{\EdN^c ~\big|~ \EcTi, \EcT }	\leq \frac{128}{mnp}	
		&&\text{by Lemma \ref{lem:event_dN}}.
\end{align*}

Inserting \eqref{eqn:prob_E6.1}, \eqref{eqn:prob_E6.2}, \eqref{eqn:prob_E6.3} to \eqref{eqn:prob_E6}, we conclude
\[	
	\Prob{\Ephi^c} \leq  \frac{256}{mnp} 
		+ \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg)
		+ n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)
		+ \exp \left( - \frac{mnp}{3} \right).
\]
\end{proof}




%	\begin{proof}[Proof of Corollary \ref{coro:unknown_CDF_uniform}]	
%		Conditioned on event $\Erow$, it holds for all $i \in [m]$ that $\left| \cB_i \right| \geq \frac{np}{2}$. Similarly, $\left| \cB_i \right| \leq 2np$ for all $i \in [m]$, when conditioned on event $\Erowp$. Therefore, for any $i \in [m]$, and any $t \geq \Tos$,
%			\begin{align*}
%				&\Prob{ \left. \sup_{z \in [D_1, D_2]} \left| \tilde{F}^{(i)} (z) - F^{(i)}(z) \right| > t	\right| \Erow, \Erowp}
%					\leq (2np)^{\frac{1}{6}}\exp\left( \frac{- \left( \frac{np}{2} \right)^{5/12} }{8 C_4^2 \left( \log (2np) \right)^{\frac{2}{\beta}} }(t - \tos)^2 \right) + \tilde{\Psi}_{m,n,p}\left( \frac{np}{2} \right).
%			\end{align*}
%	\end{proof}


==> contents/proof_noiseless.tex <==
\section{Completing Proof of Theorem \ref{thm:MSE_noiseless}: Noiseless Scenario}	\label{sec:full_proof_noiseless}

We complete the proof of Theorem \ref{thm:MSE_noiseless} using Lemmas \ref{lem:quantile_noiseless} and \ref{lem:cdf_noiseless}. 
To that end, we first state exponential tail bound on error in estimation, $|\breve{A}(i, j) - A(i,j)|$ in Lemma \ref{thm:tail_noiseless} and 
then obtain an upper bound on Mean-Square-Error (MSE) by integrating the probabilistic tail bound. This completes the proof of 
Theorem \ref{thm:MSE_noiseless}. 
	 
\subsection{Tail Bound on $|\breve{A}(i, j) - A(i,j)|$}
	
\begin{theorem}[Probabilistic bound: noiseless]\label{thm:tail_noiseless}
			For each $(i,j) \in [m] \times [n]$ and $t \geq 0$,
			\begin{align}
				\Prob{\left|\breve{A}(i, j) - A(i,j)\right| > t}%	\nonumber\\	 
				&\leq 2 \exp\left( -mp \right)	+ 4\exp \Bigg( -(n-1)p \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \Bigg).
				\label{eqn:tail_noiseless}
			\end{align}
		\end{theorem}
\begin{proof}
Let $\breve{g}^{(i)} = \big(\breve{F}^{(i)}\big)^{-1}$ denote the quantile function (right pseudo-inverse) associated with $\breve{F}^{(i)}$. 
Note that $A(u,i) = g \big( \frow{i}, \fcol{j} \big)$ and $\breve{A}(i,j) = \breve{g}^{(i)}\big(\hat{q}(j) \big)$. Let $\theta^* := F^{(i)}\big( \breve{A}(i,j) \big) 
= F^{(i)}\big( \breve{g}^{(i)}\big(\hat{q}(j) \big) \big) $. We can observe that $\big|\theta^* - \hat{q}(j) \big| \leq 2\big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty}$. 
			
By definition of the uniform norm, we have that $\big| \theta^* - \hat{q}(j)\big| \leq \big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty}$ at the point of continuity. 
Else if $\breve{g}^{(i)}\big(\hat{q}(j) \big)$ is a jump discontinuity of $\breve{F}^{(i)}$, then it follows that for any $\delta >0$, 
$ \breve{F}^{(i)}\big( \breve{g}^{(i)}\big(\hat{q}(j) \big) - \delta \big) \leq \hat{q}(j) \leq \breve{F}^{(i)}\big(\breve{g}^{(i)}\big(\hat{q}(j) \big) \big) $. 
Since $F^{(i)}$ is assumed to be continuous, $\big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty} \geq \frac{1}{2}\sup_y \lim_{\delta \to 0+}
\breve{F}^{(i)}\big(y \big) -  \breve{F}^{(i)}\big(y - \delta \big)$. Therefore, $\big|\theta^* - \hat{q}(j)\big| \leq 2\big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty}.$

Since $\breve{A}(i,j) = \breve{g}^{(i)}\big(\hat{q}(j) \big)=g \big( \frow{i}, \theta^* \big)$, and $g$ is $(\lipmin, \lipmax)$-bi-Lipschitz,
\begin{align*}
	\big| \breve{A}(i,j) - A(i, j) \big|	&= \big|g \big( \frow{i}, \fcol{j} \big) - g \big( \frow{i}, \theta^* \big)\big| \\
		&\leq \lipmax \big| \fcol{j} - \theta^* \big|\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}(j) \big| + \big| \hat{q}(j) - \theta^* \big| \big)\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}(j) \big| + 2\big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty}\big).
\end{align*}
If $\big| \fcol{j} - \hat{q}(j) \big| \leq \frac{t}{3\lipmax}$ and $\big\| \breve{F}^{(i)} - F^{(i)} \big\|_{\infty} \leq \frac{t}{3\lipmax}$, then $\big|A(u,i) - \breve{A}(i,j)\big| \leq t$. Therefore, 
\begin{align*}
	\Prob{\big| \breve{A}(i, j) - A(i,j)\big| > t}
		&\leq \Prob{ \big| \hat{q}(j) - \theta_{col}^{(j)} \big| > \frac{t}{3\lipmax}\ } + \Prob{ \sup_{z \in \Reals} \big| \breve{F}^{(i)}(z) - F^{(i)}(z) \big| > \frac{t}{3\lipmax} }\\
		&\leq 2\exp \bigg(- \frac{2 \big| \cB_{i^*} \big| t^2}{9\lipmax^2} \bigg) + 2\exp\bigg(- \frac{2 \big| \cB_i \big| t^2}{9\lipmax^2} \bigg),
\end{align*}
where the last inequality follows from Lemma \ref{lem:quantile_noiseless} and Lemma \ref{lem:cdf_noiseless}. Recall that $i^*$ denote the row index 
chosen in the algorithm; see \eqref{eqn:quantile_est}.
			
Note that $\left| \cB_i \right|$ is the sum of $n$ independent Bernoulli random variables with parameter $p$ under our Bernoulli model. 
Therefore, it takes integral value in $\{0, 1, \ldots, n \}$ following Binomial$(n,p)$ distribution.
			
However, $\left| \cB_{i^*} \right|$ follows a slightly different distribution. By algorithm description (cf. \eqref{eqn:quantile_est}), 
$\left| \cB_{i^*} \right| = 0$ if and only if $\cB^j = \emptyset$, whose probability is $(1-p)^m$. For $i \in \cB^j$, it is already conditioned 
that $M(i,j) = 1$. Therefore, 
\begin{align*}
	&\Prob{\left| \cB_{i^*}\right| = k}
		 = \begin{cases}
			(1-p)^m,	& \text{if } k=0,\\
			\left[ 1 - (1-p)^m \right] {n-1 \choose k-1} p^{k-1}(1-p)^{n-k},	& \text{if } k \geq 1.
		\end{cases}	
\end{align*}
			
As a last step, we will marginalize out $\left| \cB_i \right|$ and $\left| \cB_{i^*} \right|$.
\begin{align}
	\Prob{\left| \breve{A}(i, j) - A(i,j)\right| > t}
		&= \sum_{k_1, k_2}  \Big[ \Prob{\left.\left| \breve{A}(i, j) - A(i,j)\right| > t \right| \left| \cB_i \right| = k_1, \left| \cB_{i^*} \right| = k_2}%	\nonumber\\
%			&\qquad\qquad \times
			\Prob{\left| \cB_i \right| = k_1, \left| \cB_{i^*} \right| = k_2} \Big]	\nonumber\\
		&\leq \sum_{k_1} 2\exp \left(- \frac{2 k_1 t^2}{9\lipmax^2} \right) \Prob{\left| \cB_i \right| = k_1}
			+ \sum_{k_2} 2\exp \left(- \frac{2 k_2 t^2}{9\lipmax^2} \right) \Prob{\left| \cB_{i^*} \right| = k_2}.	\label{eqn:noiseless_term.1}
\end{align}
We can further simplify the two terms in \eqref{eqn:noiseless_term.1} as follows: The first term is bounded from above as
\begin{align}
	\sum_{k_1} 2\exp \left(- \frac{2 k_1 t^2}{9\lipmax^2} \right) \Prob{\left| \cB_i \right| = k_1}
		&= \sum_{k_1} 2\exp \left(- \frac{2 k_1 t^2}{9\lipmax^2} \right) {n \choose k_1} p^{k_1} (1-p)^{n-k_1}	\nonumber\\
		&= 2 \sum_{k_1} {n \choose k_1} \left[p\exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big)\right]^{k_1} (1-p)^{n-k_1}	\nonumber\\
		&= 2\left[1 - p \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \right]^n	\qquad\because \text{binomial theorem}	\nonumber\\
		&= 2\left[1 - \frac{np}{n} \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \right]^n	\nonumber\\
		&\leq 2 \exp \left( -np \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \right).	\label{eqn:noiseless_term.2}
\end{align}
The inequality in the last line holds because $\left( 1 + \frac{a}{n} \right)^n \leq e^{a}$ for any $a \in \Reals$ and any $n \in \Nats$.
In a similar manner, the second term in \eqref{eqn:noiseless_term.1} is bounded as
\begin{align}
	&\sum_{k_2} 2\exp \left(- \frac{2 k_2 t^2}{9\lipmax^2} \right) \Prob{\left| \cB_{i^*} \right| = k_2}	\nonumber\\
		&\qquad= 2(1-p)^m + 2\left[ 1 - (1-p)^m \right]	
			\sum_{k_2 =1}^n  \exp \left(- \frac{2 k_2 t^2}{9\lipmax^2} \right)  {n-1 \choose k_2-1} p^{k_2-1}(1-p)^{n-k_2}	\nonumber\\
		&\qquad\leq 2(1-p)^m + 2\left[ 1 - (1-p)^m \right]
			\exp \left(- \frac{2 t^2}{9\lipmax^2} \right) \exp\Bigg( -(n-1)p \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \Bigg)	\nonumber\\
		&\qquad\leq 2 \exp\left( -mp \right) + 2\exp\Bigg( -(n-1)p \bigg( 1 - \exp \Big(- \frac{2 t^2}{9\lipmax^2} \Big) \bigg) \Bigg). 	\label{eqn:noiseless_term.3}
\end{align}
Inserting the upper bounds in \eqref{eqn:noiseless_term.2} and \eqref{eqn:noiseless_term.3} to \eqref{eqn:noiseless_term.1} completes the proof.
\end{proof}
		
		
		

\subsection{Proof of Theorem \ref{thm:MSE_noiseless}: Mean Squared Error Upper Bound for $\breve{\varphi}$}
Let $\breve{\varphi}$ denote the estimator which maps $Z$ to $\breve{A}$. Then we can rewrite the mean-squared-error of $\varphi$ as
%Recall the definition of the mean squared error (see Eq. \eqref{eqn:MSE}) of estimator $\breve{\varphi}$:
\begin{align}
	MSE\left( \breve{\varphi} \right)	
		&=\Exp{\frac{1}{mn} \sum_{i=1}^m \sum_{j=1}^n \left( \breve{A}(i,j) - A(i,j) \right)^2}	\nonumber\\
%		&=\frac{1}{mn} \sum_{i=1}^m \sum_{j=1}^n \Exp{\left( \breve{A}(i,j) - A(i,j) \right)^2}	&\because\text{linear}\nonumber\\
		&= \Exp{\left( \breve{A}(1,1) - A(1,1) \right)^2}						&\because\text{exchangeable}\nonumber\\
		&= \int_0^{\infty} \Prob{\left( \breve{A}(1,1) - A(1,1) \right)^2 > t } dt		&\because\text{positive}\nonumber\\
		&= \int_0^{\infty} \Prob{\left| \breve{A}(1,1) - A(1,1) \right| > \sqrt{t} } dt		&\because u = \sqrt{t}\nonumber\\
		&= \int_0^{\infty} 2u\Prob{\left| \breve{A}(1,1) - A(1,1) \right| > u } du.		\label{eqn:integration}
\end{align}
Now it remains to integrate the tail bounds obtained in Theorem \ref{thm:tail_noiseless} to conclude our first main theorem. 

Note that for any $ a > 0$,
\begin{align}
	\int_0^{\infty} u e^{-a u^2} ds &=\int_0^{\infty} \frac{1}{2a}e^{-z} dz = \left. -\frac{1}{2a}e^{-z} \right|_0^{\infty} = \frac{1}{2a},	\label{eqn:integral}\\
	\int_0^{\infty} u e^{-au} du &= \int_0^{\infty} \frac{z}{a^2} e^{-z} dz = \frac{\Gamma(2)}{a^2} = \frac{1}{a^2}.	\label{eqn:Gamma2}
\end{align}
We can derive the above formulae from integration by substitution. \eqref{eqn:integral} and \eqref{eqn:Gamma2} will be frequently used, because 
many of our error bound have such forms. 
	
Also, we observe that the estimation error is bounded as
\[	\left| \breve{A}(i,j) - A(i,j) \right| \leq \fmax - \fmin = \frange,		\]
by the model assumption (see Section \ref{sec:model_assumption}) and the manner our estimator $\breve{\varphi}$ is defined (see Section \ref{sec:alg_noiseless}). 
Note that $\frange$ is a constant independent of the problem size $m, n$
	 	
Now we are ready to prove Theorem \ref{thm:MSE_noiseless}.
	
\begin{proof}[Proof of Theorem \ref{thm:MSE_noiseless}]
We find an upper bound on MSE by integrating the probabilistic tail bound in Theorem \ref{thm:tail_noiseless}. 
For that purpose, we first observe that given $c > 0$, 
\[	1 - e^{-cu^2} \geq c e^{-c} u^2 \quad\text{for }0 \leq u \leq 1 ; \qquad\text{and}\qquad 1 - e^{-cu^2} \geq 1 - e^{-c} \quad\text{for }u \geq 1.	\]
		
Plugging in \eqref{eqn:tail_noiseless} to \eqref{eqn:integration}, we obtain(with notation $c = \frac{2}{9L^2}$ below)
\begin{align*}
	 \MSE\left( \breve{\varphi} \right) 
		&= \int_0^{\frange} 2u \Prob{\left|\breve{A}(i,j) - A(i, j)\right| > u} du\\
		&\leq \int_0^{\frange} 4u\exp \left(- mp\right) du
			+ \int_0^{\frange}  8u\exp \left( -(n-1)p \bigg( 1 - \exp \Big(- \frac{2 u^2}{9\lipmax^2} \Big) \bigg) \right) du\\
		&\leq 2\frange^2 \exp\left(-mp\right) + \int_0^1 8u \exp \left( -(n-1)p ~c e^{-c} u^2 \right) du
			+ \int_1^{\frange} 8u \exp\left( -(n-1)p\big( 1 - e^{-c} \big)\right) du\\
		&\leq \frac{18\lipmax^2 \exp\left(\frac{2}{9\lipmax^2}\right)}{(n-1)p }
			+ \frange^2 \left[ 2 \exp(-mp) + 4 \exp\Big( -(n-1)p \big( 1 - e^{-\frac{2}{9\lipmax^2}} \big)\Big) \right].
\end{align*}
\end{proof}

==> contents/proof_noisy_known.tex <==
\section{Completing Proof of Theorem \ref{thm:MSE_noisy_known}: Noisy Scenario with Known Noise Distribution}	\label{sec:full_proof_noisy_known}

In this section, we complete the proof of Theorem \ref{thm:MSE_noisy_known} by using Lemma \ref{lem:quantile_noisy} and Lemma \ref{lem:cdf_noisy_known}. 
As in Appendix \ref{sec:full_proof_noiseless}, we first state a probabilistic tail bound on error in estimation, $|\tilde{A}(i, j) - A(i,j)|$ in Lemma \ref{thm:tail_noisy_known} 
and then obtain an upper bound on Mean-Square-Error (MSE) by integrating the tail bound. The details differ due to extra care required to handle noisy setting.  
	
\subsection{Tail Bound on $|\tilde{A}(i,j) - A(i,j)|$}\label{sec:tail_noisy_known}
Recall the definition of problem size $m, n$, mask parameter $p$, model parameter $\lipmax$, and the constants $\constcc, \constdd$; 
see \eqref{eqn:const_3} and \eqref{eqn:const_4} in Section \ref{sec:notation_constants}. Also, we recall the definition of $\Qf: \Reals_+ \to \Reals_+$ 
from \eqref{eqn:Q_function} (can be found in the proof of Lemma \ref{lem:quantile_noisy} in Appendix \ref{sec:proof_noisy_quantile}): 
\[
\Qf(x) = 2\sqrt{\pi} \left( \frac{1}{\sqrt{\constaa x}} + \frac{1}{\sqrt{\constbb x}} + \frac{e^{\constaa/2}}{\sqrt{mp \constaa }} 
		+  \frac{e^{\constbb/2}}{\sqrt{mp \constbb }} \right).
\]

We define two conditioning events on $t$:
\begin{align}\label{eqn:technical_conditions}
	E_1 & \triangleq \Big\{ t \leq 8 \lipmax \Qf\left(\frac{mp}{2} \right) \Big\}
	\qquad \text{and} \qquad 
	E_2  \triangleq \Big\{ t \leq 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} \Big\}. 
\end{align}

Now we present a probabilistic tail bound on the estimation error of $\tilde{\varphi}$.
\begin{theorem}\label{thm:tail_noisy_known}
For each $(i,j) \in [m] \times [n]$, and for any $t \geq 0$, 
\begin{align*}
	&\Prob{\left| \tilde{A}(i, j) - A(i,j)\right| > t }\\%+ \lipmax (\constcc + \constdd) \left( \log \Big(\frac{np}{2}\Big)\right)^{-1/\beta} }\\
		&\qquad \leq	\Ind{ E_1 } + \Ind {E_2} 
			+ \exp\left( -\frac{n \big( t - 4 \lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12 \lipmax} \right)  \Ind{E_1^c} \\
		&\qquad \quad + 2 (2np)^{\frac{1}{4}} \left( \log (2np) \right)^{\frac{2}{\beta}}
			\exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2 \constdd^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} 
				\left( \frac{t}{2\lipmax} -  (\constcc + \constdd) \Big( \log \Big(\frac{np}{2}\Big) \Big)^{-1/\beta} \right)^2 \right)  \Ind{E_2^c} \\
		&\qquad\quad + \exp\left( -\frac{n t^2}{8\lipmax^2} \right) + \exp\left( - \frac{mp}{8} \right) + 2  \exp\left(-\frac{np}{8} \right).
\end{align*}
\end{theorem}

Note that the terms in the last line which are independent of $t$, decays to $0$ as $n \to \infty$ at the exponential rate of $np$ as long as the sampling probability is sufficiently large, i.e., $p = \omega \left(\frac{1}{n}\right)$, .
	
\begin{proof}
Let $\theta^* \equiv F^{(i)}\big( \tilde{A}(i,j) \big) = F^{(i)}\big( \tilde{g}^{(i)}\big(\hat{q}_{\marg}(j) \big) \big) $. Since $\tilde{F}^{(i)}$ is continuous, 
$\big|\theta^* - \hat{q}_{\marg}(j)\big| \leq \big\| \tilde{F}^{(i)} - F^{(i)} \big\|_{\infty}$. By the same line of argument as in the proof of Theorem 
\ref{thm:tail_noiseless}, since $\tilde{A}(i,j) = \tilde{g}^{(i)}\big(\hat{q}_{\marg}(j) \big)=g \big( \frow{i}, \theta^* \big)$, and $g$ is $(\lipmin, \lipmax)$-bi-Lipschitz, 
\begin{align*}
	\big|\tilde{A}(u,i) - A(i,j)\big|	
		&= \big|g \big( \frow{i}, \fcol{j} \big) - g \big( \frow{i}, \theta^* \big)\big| \\
		&\leq \lipmax \big| \fcol{j} - \theta^* \big|\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}_{\marg}(j) \big| + \big| \hat{q}_{\marg}(j) - \theta^* \big| \big)\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}_{\marg}(j) \big| + \big\| \tilde{F}^{(i)} - F^{(i)} \big\|_{\infty}\big).
\end{align*}
Again, if both $\big| \fcol{j} - \hat{q}_{\marg}(j) \big| \leq \frac{t}{2\lipmax}$ and $\big\| \tilde{F}^{(i)} - F^{(i)} \big\|_{\infty} \leq \frac{t}{2\lipmax}$ are satisfied, 
then $\big| \tilde{A}(u,i) - A(i,j)\big| \leq t$. We can achieve the following upper bound by applying the union bound on the contraposition. 
With letting $E_{(i)} := \Erow \cap \Erowp$, we have the following upper bound: for any $t > 0$,
\begin{align}
	&\Prob{\big| \tilde{A}(i, j) - A(i,j)\big| > t + \lipmax (\constcc + \constdd) \left( \log \Big(\frac{np}{2}\Big)\right)^{-1/\beta} }	\nonumber\\
		&\qquad\leq \Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} } 
			+ \Prob{\sup_{z \in \Reals} \big| \tilde{F}^{(i)}(z) - F^{(i)}(z) \big| > \frac{t}{2\lipmax} + (\constcc + \constdd) \left( \log \Big(\frac{np}{2}\Big)\right)^{-1/\beta}}	\nonumber\\
		&\qquad\leq \Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} }		\nonumber\\
			&\qquad\quad + \Prob{ \big. \sup_{z \in \Reals} \big| \tilde{F}^{(i)}(z) - F^{(i)}(z) \big| > \frac{t}{2\lipmax} + (\constcc + \constdd) 
				\left( \log \Big(\frac{np}{2}\Big)\right)^{-1/\beta} ~\bigg|~ E_{(i)}} + \Prob{E_{(i)}^c}.		\label{eqn:prob_aggr}
\end{align}

Since we know that probability cannot exceed $1$, it follows from Lemma \ref{lem:quantile_noisy} that for any $t > 0$,
\begin{align}
	&\Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} }		\nonumber\\
	&\qquad\leq	\Ind{t \leq 8\lipmax \Qf\Big(\frac{mp}{2}\Big) }		\nonumber\\
	&\qquad\quad+  
		\bigg[ \exp\bigg( -\frac{n t^2}{8\lipmax^2} \bigg) + \exp\bigg( -\frac{n \big( \frac{t}{4\lipmax} - \Qf\big(\frac{mp}{2}\big) \big)}{3} \bigg) + \exp\bigg( - \frac{mp}{8} \bigg)\bigg]
		\Ind{t \geq 8\lipmax \Qf\Big(\frac{mp}{2}\Big) }.		\label{eqn:tail_known_term.1}
\end{align}
%	
Also, it follows from Lemma \ref{lem:cdf_noisy_known} that for any $t \geq 0$,
\begin{align*}
	&\Prob{ \sup_{z \in \Reals} \left| \tilde{F}^{(i)}(z) - F^{(i)}(z) \right| > \frac{t}{2\lipmax} + (\constcc + \constdd) \Big( \log \Big(\frac{np}{2}\Big) \Big)^{-1/\beta} ~ \bigg|~ E_{(i)}}\\
		&\qquad \leq
			2 (2np)^{\frac{1}{4}} \left( \log (2np) \right)^{\frac{2}{\beta}}
			\exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2C_4^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} \left( \frac{t}{2\lipmax} \right)^2 \right).
\end{align*}
We used the fact that for all $i \in [m]$, $\left| \cB_i \right| \geq \frac{np}{2}$ conditioned on event $\Erow$ 
and $\left| \cB_i \right| \leq 2np$ when conditioned on event $\Erowp$.

By the trivial upper bound on the probability and changing the variable, we obtain
\begin{align}
	&\Prob{ \sup_{z \in \Reals} \left| \tilde{F}^{(i)}(z) - F^{(i)}(z) \right| > \frac{t}{2\lipmax} ~ \bigg|~ E_{(i)}}	\nonumber\\
		&\qquad\leq	\Ind{t \leq 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} }		\nonumber\\
		&\qquad\quad +
			2 (2np)^{\frac{1}{4}} \left( \log (2np) \right)^{\frac{2}{\beta}}
			\exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2 \constdd^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} 
				\left( \frac{t}{2\lipmax} -  (\constcc + \constdd) \Big( \log \Big(\frac{np}{2}\Big) \Big)^{-1/\beta} \right)^2 \right)	\nonumber\\
		&\qquad\qquad \times \Ind{t > 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} }.			\label{eqn:tail_known_term.2}
\end{align}

Lastly, we obtain an upper bound on $\Prob{E_{(i)}^c}$ by applying the binomial Chernoff bound:
\begin{align}
	\Prob{E_{(i)}^c} &= \Prob{ \left| \cB_i \right| < \frac{np}{2} \text{ or } \left| \cB_i \right| > 2np }	\nonumber\\
		&\leq \Prob{\left| \cB_i \right| < \frac{np}{2}} + \Prob{\left| \cB_i \right| > 2np }		\nonumber\\
		&\leq \exp\left(-\frac{np}{8} \right) + \exp\left(-\frac{np}{3} \right)		\nonumber\\
		&\leq 2  \exp\left(-\frac{np}{8} \right).					\label{eqn:tail_known_term.3}
\end{align}
		
Substituting the three upper bounds obtained in \eqref{eqn:tail_known_term.1}, \eqref{eqn:tail_known_term.2}, \eqref{eqn:tail_known_term.3} back to 
\eqref{eqn:prob_aggr}, we can conclude that
\begin{align*}
	\Prob{\left| \tilde{A}(i, j) - A(i,j)\right| > t}
		&\leq	 \Ind{t \leq 8\lipmax \Qf\left(\frac{mp}{2}\right) } +  \Ind{t \leq 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} }\\
		&\quad + \exp\left( -\frac{n \big( t - 4 \lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12 \lipmax} \right) \Ind{t > 8\lipmax \Qf\left(\frac{mp}{2}\right) }\\
		&\quad + 2 (2np)^{\frac{1}{4}} \left( \log (2np) \right)^{\frac{2}{\beta}}
			\exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2 \constdd^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} 
				\left( \frac{t}{2\lipmax} -  (\constcc + \constdd) \Big( \log \Big(\frac{np}{2}\Big) \Big)^{-1/\beta} \right)^2 \right)	\nonumber\\
		&\qquad \times \Ind{t > 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} }\\
		&\quad + \exp\left( -\frac{n t^2}{8\lipmax^2} \right) + \exp\left( - \frac{mp}{8} \right) + 2  \exp\left(-\frac{np}{8} \right).
\end{align*}
We simplified our upper bound using the fact that the indicator takes value between $0$ and $1$, i.e., 
$ \Big[ \exp\left( -\frac{n t^2}{8\lipmax^2} \right) + \exp\left( - \frac{mp}{8} \right)  \Big]  \Ind{t \geq 8\lipmax \Qf\left(\frac{mp}{2}\right) } 
\leq  \exp\left( -\frac{n t^2}{8\lipmax^2} \right) + \exp\left( - \frac{mp}{8} \right) $.
\end{proof}
	



\subsection{Proof of Theorem \ref{thm:MSE_noisy_known}: Mean Squared Error Upper Bound for $\tilde{\varphi}$}

Let $\tilde{\varphi}$ denote the estimator defined as in \eqref{eqn:estimate_noisy_known}, which maps $Z$ to $\tilde{A}$. 
By the same line of arguments as in \eqref{eqn:integration},
\begin{align*}
	\MSE\left( \tilde{\varphi} \right)			
		&= \int_0^{\infty} 2u\Prob{\left| \tilde{A}(i,j) - A(i,j) \right| > u } du		\label{eqn:integration2}
\end{align*}
Also, from the model assumption and the construction of the estimators, the estimation error is bounded above:
\[	\left| \tilde{A}(i,j) - A(i,j) \right| \leq \tfmax - \tfmin,		\]

	
\begin{proof}[Proof of Theorem \ref{thm:MSE_noisy_known}]
In order to achieve an upper bound on the MSE for the kernel density estimator with known noise, $\tilde{\varphi}$, we integrate the tail probability bound 
from Theorem \ref{thm:tail_noisy_known}.
		
First of all, we recall from Eqs. \eqref{eqn:integral} and \eqref{eqn:Gamma2} that
\begin{align*}
	\int_0^{\infty} u e^{-a u^2} du =\frac{1}{2a},	\quad\text{and}\quad \int_0^{\infty} u e^{-au} du = \frac{1}{a^2}.	
\end{align*}

Now, the mean squared error can be written in the following form:
\begin{align}
	\MSE\left( \tilde{\varphi} \right)
		&= \int_0^{\tfmax - \tfmin} 2u \Prob{\left| \tilde{A}(i, j) - A(i,j)\right| > u} du	\nonumber\\
		&\leq \int_0^{8\lipmax\Qf\left(\frac{mp}{2}\right)}  2u~ du + \int_0^{4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta}} 2u~ du		\nonumber\\
		&\quad	+ \int_{8\lipmax\Qf\left(\frac{mp}{2}\right)}^{\tfmax - \tfmin}  2u\exp\left( -\frac{n \big( u - 4\lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12\lipmax} \right)du	
			\label{eqn:MSE_tilde_term.1}\\
		&\quad 	+ \int_{4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta}}^{\tfmax - \tfmin} 
			4 (2np)^{\frac{1}{4}} \left( \log (2np) \right)^{\frac{2}{\beta}}  u 	\nonumber\\
			&\quad\qquad	\times\exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2C_4^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} 
				\left( \frac{u}{2\lipmax} -(\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} \right)^2 \right) du \label{eqn:MSE_tilde_term.2}\\
		&\quad	+ \int_0^{\tfmax - \tfmin} 2u\exp\left( -\frac{n u^2}{8\lipmax^2} \right) du 		\label{eqn:MSE_tilde_term.3}\\
		&\quad + \int_0^{\tfmax - \tfmin} 2u \left[ \exp\left( - \frac{mp}{8}\right)  + 2 \exp\left( - \frac{np}{8}\right) \right] du.	\nonumber
\end{align}
In the rest of the proof, we establish upper bounds on the terms in \eqref{eqn:MSE_tilde_term.1}, \eqref{eqn:MSE_tilde_term.2}, and 
\eqref{eqn:MSE_tilde_term.3} one by one.

First of all, we can achieve the following upper bound for \eqref{eqn:MSE_tilde_term.1}:
\begin{align}
	&\int_{8\lipmax\Qf\left(\frac{mp}{2}\right)}^{\tfmax - \tfmin}  2u\exp\left( -\frac{n \big( u - 4\lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12\lipmax} \right)du
					\nonumber\\
	 	&\qquad = \int_{0}^{\tfmax - \tfmin - 8\lipmax\Qf\left(\frac{mp}{2}\right)}  2\left(u' + 8\lipmax \Qf\left(\frac{mp}{2}\right) \right) 
			\exp\left( -\frac{n\left( u' + 4\lipmax \Qf\left(\frac{mp}{2}\right)\right)}{12\lipmax } \right)du'		&&\because\text{change of variables}
					\nonumber\\
		&\qquad \leq \int_{0}^{\tfmax - \tfmin - 8\lipmax\Qf\left(\frac{mp}{2}\right)}  2\left(u' + 8\lipmax \Qf\left(\frac{mp}{2}\right) \right) 
			\exp\left( -\frac{n u'}{12\lipmax } \right)du'										&&\because \Qf\left(\frac{mp}{2}\right) \geq 0 
					\nonumber\\
		&\qquad \leq  \int_{0}^{\infty}  2\left(u' + 8\lipmax \Qf\left(\frac{mp}{2}\right) \right) \exp\left( -\frac{n u'}{12\lipmax } \right)du'
					\nonumber\\
		&\qquad = \frac{288\lipmax ^2}{n^2} + 8\lipmax \Qf\left(\frac{mp}{2}\right) \sqrt{\frac{3\lipmax \pi}{n}}.		\label{eqn:simplified_tilde.1}
\end{align}
				
Next, we establish an upper bound of the term in \eqref{eqn:MSE_tilde_term.2}. To simplify the notation in our derivation, 
we let 
\[	c_1 \triangleq \frac{ 1 }{2 \constdd^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}}\left( \frac{np}{2} \right)^{\frac{1}{2}}, \quad\text{and}\quad 
	c_2 \triangleq (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta}.		\]
%	 and divide the region of integration into two parts pivoting on $u = 2L c_2$:
Then
\begin{align}
	&\int_{4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta}}^{\tfmax - \tfmin} 
			u  \exp\left( \frac{-\left( \frac{np}{2} \right)^{1/2} }{2C_4^2 \left( \log \left( 2np \right) \right)^{\frac{2}{\beta}}} 
				\left( \frac{u}{2\lipmax} -(\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} \right)^2 \right) du	\nonumber\\
		&\qquad	= \int_{4\lipmax c_2}^{\tfmax - \tfmin} u\exp\left( - c_1 \left( \frac{u}{2\lipmax} - c_2 \right)^2	 \right)du	\nonumber\\
		&\qquad	\leq	\int_{4\lipmax c_2}^{\tfmax - \tfmin}u\exp\left( - c_1 \left( \frac{u}{4\lipmax} \right)^2	 \right)du	
					\qquad\because \frac{u}{2\lipmax} - c_2 \geq \frac{u}{4\lipmax}, ~\forall u \geq 4\lipmax c_2		\nonumber\\	
		&\qquad	\leq \int_{0}^{\infty}u\exp\left( - \frac{c_1}{16\lipmax ^2} u^2 \right)du 		
					\qquad\qquad\qquad\because u \exp\left( - \frac{c_1}{16\lipmax^2} u^2	 \right) \geq 0, ~\forall u \geq 0	\nonumber\\
		&\qquad	= \frac{8 \lipmax^2}{c_1}.		\label{eqn:simplified_tilde.2}
\end{align}

Lastly, we can easily observe the following upper bound on \eqref{eqn:MSE_tilde_term.3}:
\begin{align}
	\int_0^{\tfmax - \tfmin} 2u\exp\left( -\frac{n u^2}{8\lipmax^2} \right) du 
		&\leq  \int_0^{\infty} 2u\exp\left( -\frac{n u^2}{8\lipmax^2} \right) du
		= \frac{8\lipmax^2}{n}.		\label{eqn:simplified_tilde.3}
\end{align}


Inserting \eqref{eqn:simplified_tilde.1} to \eqref{eqn:MSE_tilde_term.1}, \eqref{eqn:simplified_tilde.2} to \eqref{eqn:MSE_tilde_term.2}, and 
\eqref{eqn:simplified_tilde.3} to \eqref{eqn:MSE_tilde_term.3}, we acquire the following upper bound:
\begin{align*}
	\MSE\left( \tilde{\varphi} \right)
	&\leq  \left[ 8\lipmax \Qf\left(\frac{mp}{2}\right) \right]^2 + \left[ 4\lipmax (\constcc + \constdd) \left( \log \frac{np}{2} \right)^{-1/\beta} \right]^2
			+ \frac{288\lipmax^2}{n^2} +  8\lipmax\Qf\left(\frac{mp}{2}\right) \sqrt{\frac{3\lipmax\pi}{n}}\\
	 	&\quad+ 64\sqrt[4]{8}\lipmax^2 \constdd^2 \frac{\left( \log \left( 2np \right) \right)^{\frac{4}{\beta}}}{(np)^{\frac{1}{4}}}
	 	+ \frac{8\lipmax^2}{n}  
		+  \big( \tfmax - \tfmin \big)^2 \left[ \exp\left( - \frac{mp}{8}\right)  + 2 \exp\left( - \frac{np}{8}\right) \right] .
\end{align*}
Recall that $\Qf\big(\frac{mp}{2}\big) = \frac{\constee}{\sqrt{mp}}$. Rearranging the terms in the increasing order of convergence rates concludes the proof.

\end{proof}



==> contents/proof_noisy_unknown.tex <==
\section{Proof of Corollary \ref{coro:answer.2}}\label{sec:proof_ME}


\subsection{Helper Lemma}
In this section, we establish a probabilistic tail bound on $ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) | $.

\begin{lemma}
For $i \in [m]$, let $\hat{F}_i$ be defined as in \eqref{eqn:ECDF_unknown_noise} with $\hat{\phi}_{N}(t) = \hat{\phi}_{N, i}(t)$ as described 
in Section \ref{sec:noise_estimation}, cf. \eqref{eqn:chN_est}. For $j \in [n]$, let $\hat{q}_{\marg}(j)$ be defined as in \eqref{eqn:estimate_marg}.

If we choose the kernel bandwidth $h = (4\gamma)^{\frac{1}{\beta}}(\log |\cB_i|)^{-\frac{1}{\beta}}$ and the ridge parameter 
$\rho = \frac{1}{B} |\cB_i|^{-\frac{9}{20}}$. If $|\cB_i| \geq 1024$ and $mp$ and $n$ are sufficiently large so that 
$\valphiAA + \valphiBB \leq \frac{1}{B} |\cB_i|^{-\frac{9}{20}}$, then for any $t \geq 0$, then for any $t > 0$,
	\begin{align*}
		\Prob{ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) | > t }
			\leq -----.
	\end{align*}
\end{lemma}

\begin{proof}
Let $\theta^* \equiv F^{(i)}\big( \hat{A}(i,j) \big) = F^{(i)}\big( \hat{g}^{(i)}\big(\hat{q}_{\marg}(j) \big) \big) $. Since $\hat{F}^{(i)}$ is continuous, 
$\big|\theta^* - \hat{q}_{\marg}(j)\big| \leq \big\| \hat{F}^{(i)} - F^{(i)} \big\|_{\infty}$. By the same line of argument as in the proof of Theorem 
\ref{thm:tail_noisy_known}, since $\hat{A}(i,j) = \hat{g}^{(i)}\big(\hat{q}_{\marg}(j) \big)=g \big( \frow{i}, \theta^* \big)$, and $g$ is $(\lipmin, \lipmax)$-bi-Lipschitz, 
\begin{align*}
	\big|\hat{A}(u,i) - A(i,j)\big|	
		&= \big|g \big( \frow{i}, \fcol{j} \big) - g \big( \frow{i}, \theta^* \big)\big| \\
		&\leq \lipmax \big| \fcol{j} - \theta^* \big|\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}_{\marg}(j) \big| + \big| \hat{q}_{\marg}(j) - \theta^* \big| \big)\\
		&\leq \lipmax \big( \big| \fcol{j} - \hat{q}_{\marg}(j) \big| + \big\| \hat{F}^{(i)} - F^{(i)} \big\|_{\infty}\big).
\end{align*}
Again, if both $\big| \fcol{j} - \hat{q}_{\marg}(j) \big| \leq \frac{t}{2\lipmax}$ and $\big\| \hat{F}^{(i)} - F^{(i)} \big\|_{\infty} \leq \frac{t}{2\lipmax}$ are satisfied, 
then $\big| \hat{A}(u,i) - A(i,j)\big| \leq t$. We can achieve the following upper bound by applying the union bound on the contraposition. 
With letting $E_{(i)} := \Erow \cap \Erowp$, we have the following upper bound: for any $t > 0$,
\begin{align}
	&\Prob{\big| \hat{A}(i, j) - A(i,j)\big| > t + \lipmax \big( \slackAA + \slackBB + \slackCC \big) }	\nonumber\\
		&\qquad\leq \Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} } 
			+ \Prob{\sup_{z \in \Reals} \big| \hat{F}^{(i)}(z) - F^{(i)}(z) \big| > \frac{t}{2\lipmax} + \slackAA + \slackBB + \slackCC}	\nonumber\\
		&\qquad\leq \Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} }
			 + \Prob{ \big. \sup_{z \in \Reals} \big| \hat{F}^{(i)}(z) - F^{(i)}(z) \big| > \frac{t}{2\lipmax} + \slackAA + \slackBB + \slackCC
				 ~\bigg|~ E_{(i)}} + \Prob{E_{(i)}^c}.		\label{eqn:prob_aggr_hat}
\end{align}

Since we know that probability cannot exceed $1$, it follows from Lemma \ref{lem:quantile_noisy} that for any $t > 0$,
\begin{align}
	&\Prob{ \big| \hat{q}_{\marg}(j) - \theta_{col}^{(j)} \big| > \frac{t}{2\lipmax} }		\nonumber\\
	&\qquad\leq	\Ind{t \leq 8\lipmax \Qf\Big(\frac{mp}{2}\Big) }		\nonumber\\
	&\qquad\quad+  
		\bigg[ \exp\bigg( -\frac{n t^2}{8\lipmax^2} \bigg) + \exp\bigg( -\frac{n \big( \frac{t}{4\lipmax} - \Qf\big(\frac{mp}{2}\big) \big)}{3} \bigg) + \exp\bigg( - \frac{mp}{8} \bigg)\bigg]
		\Ind{t \geq 8\lipmax \Qf\Big(\frac{mp}{2}\Big) }.		\label{eqn:tail_unknown_term.1}
\end{align}
%	
Recall we assumed $m \geq 8 \text{ and } p \geq \frac{16}{n}$. By Lemma \ref{lem:cdf_noisy_unknown}, for any $t \geq 0$,
%Suppose that $m \geq 8 \text{ and } p \geq \frac{16}{n}$. For any $t \geq 0$,
\begin{align*}
	\bbP\bigg( \sup_{z \in \Reals} \big| \hat{F}^{(i)} (z) - F^{(i)}(z) \big| > \frac{t}{2\lipmax} + \slackAA + \slackBB + \slackCC ~ \bigg|~ E_{(i)} \bigg)
		&\leq 4np \exp\bigg( \frac{- \big( \frac{np}{2} \big)^{5/12} t^2 }{2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} } \bigg) \\
		&\quad+  \frac{256}{mnp} + n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)\\
		&\quad+ \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg) + \exp \left( - \frac{mnp}{3} \right).
\end{align*}
We used the fact that for all $i \in [m]$, $\left| \cB_i \right| \geq \frac{np}{2}$ conditioned on event $\Erow$ and $\left| \cB_i \right| \leq 2np$ 
when conditioned on event $\Erowp$. Observe that we obtain the following upper bound by changing the variable:% the trivial upper bound on the probability
\begin{align}
	&\Prob{ \sup_{z \in \Reals} \left| \hat{F}^{(i)}(z) - F^{(i)}(z) \right| > \frac{t}{2\lipmax} ~ \bigg|~ E_{(i)}}	\nonumber\\
		&\qquad\leq	\Ind{t \leq 4\lipmax \big( \slackAA + \slackBB + \slackCC \big) }	\nonumber\\
		&\qquad\quad+	4np \exp\bigg( \frac{- \big( \frac{np}{2} \big)^{5/12}  }{2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} } 
			\Big( t - 2\lipmax \big( \slackAA + \slackBB + \slackCC \big) \Big)^2 \bigg) \Ind{t > 4\lipmax \big( \slackAA + \slackBB + \slackCC \big) }	\nonumber\\
		&\qquad\quad+  \frac{256}{mnp} + n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)
			+ \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg) + \exp \left( - \frac{mnp}{3} \right).		\label{eqn:tail_unknown_term.2}
\end{align}

Lastly, we recall from \eqref{eqn:tail_known_term.3} that
\begin{equation}\label{eqn:tail_unknown_term.3}
	\Prob{E_{(i)}^c} \leq 2  \exp\left(-\frac{np}{8} \right).		
\end{equation}
		
Substituting the three upper bounds obtained in \eqref{eqn:tail_unknown_term.1}, \eqref{eqn:tail_unknown_term.2}, \eqref{eqn:tail_unknown_term.3} back to 
\eqref{eqn:prob_aggr_hat}, we can conclude that for any $t \geq 0$,
\begin{align*}
	\Prob{\left| \hat{A}(i, j) - A(i,j)\right| > t}
		&\leq	 \Ind{t \leq 8\lipmax \Qf\left(\frac{mp}{2}\right) } +  \Ind{t \leq 4\lipmax \big( \slackAA + \slackBB + \slackCC \big) }\\
		&\quad + \exp\left( -\frac{n \big( t - 4 \lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12 \lipmax} \right) \Ind{t > 8\lipmax \Qf\left(\frac{mp}{2}\right) }\\
		&\quad + 4np \exp\bigg( \frac{- \big( \frac{np}{2} \big)^{5/12}  }{2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} } 
			\Big( t - 2\lipmax \big( \slackAA + \slackBB + \slackCC \big) \Big)^2 \bigg) \Ind{t > 4\lipmax \big( \slackAA + \slackBB + \slackCC \big) } \\
		&\quad + \exp\left( -\frac{n t^2}{8\lipmax^2} \right) + \exp\left( - \frac{mp}{8} \right)\\
		&\quad +  \frac{256}{mnp} + n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)\\
		&\quad + \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg) + \exp \left( - \frac{mnp}{3} \right).
\end{align*}
We simplified our upper bound using the fact that the indicator takes value between $0$ and $1$.
\end{proof}





\subsection{Proof of Corollary \ref{coro:answer.2}}
\begin{proof}[Proof of Corollary \ref{coro:answer.2}]
Letting $\hat{A} = \psi(Z)$, we have $\hat{A} = \hat{F}_i^{-1} \big( \hat{q}_{\marg}(j) \big)$ for $(i, j) \in [m] \times [n]$. 
We recall the definition of $\RiskME(\psi)$ from \eqref{eqn:loss_psi} and see that
\begin{align*}
	\RiskME(\psi) &= \bbE_{Z} \bigg[ \sup_{i \in [m]} \frac{1}{n}  \sum_{j=1}^n | \hat{A}(i,j) - A(i,j) |^2 \bigg]\\
		&\leq  \bbE_{Z} \bigg[ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) |^2 \bigg].
\end{align*}
Since $| \hat{A}(i,j) - A(i,j) |^2 \geq 0$, it follows that 
\begin{align*}
	\bbE_{Z} \bigg[ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) |^2 \bigg]
		= \int_{0}^{\infty} \Prob{ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) |^2 > t} dt\\
		= \int_{0}^{\infty} 2 s \Prob{ \sup_{i \in [m]} \sup_{j \in [n]} | \hat{A}(i,j) - A(i,j) | > s} ds
\end{align*}
by the changing of variables $s = \sqrt{t}$.

\end{proof}


	
\subsection{Preparation}
Recall the definition of problem size $m, n$, mask parameter $p$, model parameter $\lipmax$, and the constants $\constcc, \constdd$; 
see \eqref{eqn:const_3} and \eqref{eqn:const_4} in Section \ref{sec:notation_constants}. Also, we recall the definition of $\Qf: \Reals_+ \to \Reals_+$ 
from \eqref{eqn:Q_function} (can be found in the proof of Lemma \ref{lem:quantile_noisy} in Appendix \ref{sec:proof_noisy_quantile}): 
\[
\Qf(x) = 2\sqrt{\pi} \left( \frac{1}{\sqrt{\constaa x}} + \frac{1}{\sqrt{\constbb x}} + \frac{e^{\constaa/2}}{\sqrt{mp \constaa }} 
		+  \frac{e^{\constbb/2}}{\sqrt{mp \constbb }} \right).
\]

We recall the definition of $E_1$, a conditioning event on $t$, from \eqref{eqn:technical_conditions}
\begin{align*}
	E_1 & \triangleq \Big\{ t \leq 8 \lipmax \Qf\left(\frac{mp}{2} \right) \Big\}
\end{align*}
and define a new event $E_3$ (a variant of $E_2$, adapted to the setting of unknown noise distribution) as 
\begin{equation}
	E_3  \triangleq \Big\{ t \leq 4\lipmax (\slackAA + \slackBB + \slackCC) \Big\}
\end{equation}
where (recall the definition from \eqref{eqn:slackA}, \eqref{eqn:slackB}, \eqref{eqn:slackC})
\begin{align*}
	\slackAA 	&= \frac{\kmax }{\pi \left( 4\gamma \right)^{\frac{1}{\beta}} }  \frac{\left( \log (2np) \right)^{\frac{1}{\beta}}}{\big(\frac{np}{2} \big)^{\frac{17}{24}}},\\
	\slackBB 	&= \constcc \bigg( \log \Big(\frac{np}{2}\Big)\bigg)^{-\frac{1}{\beta}},\\
	\slackCC 	&=  \frac{2B \kmax(\tfmax - \tfmin)}{ \pi (4\gamma)^{\frac{1}{\beta}} } \frac{(\log (2np))^{\frac{1}{\beta}}}{ \big(\frac{np}{2} \big)^{\frac{1}{24}}} 
			 \Big( 1 + ( 2np )^{\frac{7}{24}} \big( \valphi \big) \Big) .
\end{align*}
Recall from \eqref{eqn:valphi_A} and \eqref{eqn:valphi_B} that
\begin{align*}
	\valphiAA	&=	\frac{32 \big( 1 + 4\lipmax(\constee + \sqrt{2}) \big) }{(4\gamma)^{\frac{1}{\beta}}}
		\frac{(\log n )^{\frac{1}{\beta}}}{\sqrt{mnp}}	
		\bigg[\log\Big( \frac{mn^2 p \log(mnp)}{32} \Big) \bigg]^{\frac{1}{2}},	\\
	\valphiBB	&=	\frac{16 \big( \lipmax (\constee + \sqrt{2}) + \sigma \big)^2 }{(4\gamma)^{\frac{2}{\beta}}} 
		\frac{\log(4mnp) (\log n )^{\frac{2}{\beta}} }{n \log(mnp)}
		+ \frac{2 \sigma B }{(4\gamma)^{\frac{1}{\beta}}} \frac{ (\log n )^{\frac{1}{\beta}} }{n \log(mnp)}.	
\end{align*}	



%%% =====================================
%%%	MSE
%%% =====================================	

\subsection{Proof of Theorem \ref{thm:MSE_noisy_unknown}: Mean Squared Error Upper Bound for $\hat{\varphi}$}

Let $\hat{\varphi}$ denote the estimator defined as in \eqref{eqn:estimate_noisy_known}, which maps $Z$ to $\hat{A}$. 
By the same line of arguments as in \eqref{eqn:integration},
\begin{align*}
	\MSE\left( \hat{\varphi} \right)			
		&= \int_0^{\infty} 2u\Prob{\left| \hat{A}(i,j) - A(i,j) \right| > u } du		\label{eqn:integration2}
\end{align*}
Also, from the model assumption and the construction of the estimators, the estimation error is bounded above:
\[	\left| \hat{A}(i,j) - A(i,j) \right| \leq \tfmax - \tfmin,		\]

	
\begin{proof}[Proof of Theorem \ref{thm:MSE_noisy_unknown}]
In order to achieve an upper bound on the MSE for the kernel density estimator with known noise, $\hat{\varphi}$, we integrate the tail probability bound 
from Theorem \ref{thm:tail_noisy_unknown}.
		
First of all, we recall from Eqs. \eqref{eqn:integral} and \eqref{eqn:Gamma2} that
\begin{align*}
	\int_0^{\infty} u e^{-a u^2} du =\frac{1}{2a},	\quad\text{and}\quad \int_0^{\infty} u e^{-au} du = \frac{1}{a^2}.	
\end{align*}

Now, the mean squared error can be written in the following form:
\begin{align}
	\MSE\left( \hat{\varphi} \right)
		&= \int_0^{\tfmax - \tfmin} 2u \Prob{\left| \hat{A}(i, j) - A(i,j)\right| > u} du	\nonumber\\
%
		&\leq \int_0^{8\lipmax\Qf\left(\frac{mp}{2}\right)}  2u~ du + \int_0^{4\lipmax ( \slackAA + \slackBB + \slackCC )} 2u~ du		\nonumber\\
		&\quad	+ \int_{8\lipmax\Qf\left(\frac{mp}{2}\right)}^{\tfmax - \tfmin}  2u\exp\left( -\frac{n \big( u - 4\lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12\lipmax} \right)du		\label{eqn:MSE_hat_term.1}\\
		&\quad	+ \int_{4\lipmax( \slackAA + \slackBB + \slackCC)}^{\tfmax - \tfmin}
			8np \exp\bigg( \frac{- \big( \frac{np}{2} \big)^{5/12}  }{2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} } 
			\Big( u - 2\lipmax \big( \slackAA + \slackBB + \slackCC \big) \Big)^2 \bigg) u ~ du		\label{eqn:MSE_hat_term.2}\\
		&\quad	+ \int_0^{\tfmax - \tfmin} 2 u \exp\left( -\frac{n u^2}{8\lipmax^2} \right) du		\label{eqn:MSE_hat_term.3}\\
		&\quad	+ C_{m,n,p} \int_0^{\tfmax - \tfmin} 2 u du		\nonumber
\end{align}
where we recall the definition of $C_{m,n,p}$ from \eqref{eqn:Cmnp} as
\begin{align*}
	C_{m,n,p} &\triangleq	 \frac{256}{mnp} + n \exp\big( - n^{\frac{1}{2}} \big) + n \exp \bigg( -\frac{1}{3 \sqrt{2} } n^{\frac{3}{4}} \bigg)
		+ \exp\bigg( - \frac{m}{16} \bigg) + \exp\bigg( - \frac{n}{16} \bigg) + \exp \left( - \frac{mnp}{3} \right) + \exp\left( - \frac{mp}{8} \right).
\end{align*}
In the rest of the proof, we establish upper bounds on the terms in \eqref{eqn:MSE_hat_term.1}, \eqref{eqn:MSE_hat_term.2}, 
and \eqref{eqn:MSE_hat_term.3}.

In fact, we notice that  \eqref{eqn:MSE_hat_term.1} is the same with  \eqref{eqn:MSE_tilde_term.1} and  \eqref{eqn:MSE_hat_term.3} is the same with 
 \eqref{eqn:MSE_tilde_term.3}. Therefore, we recall the upper bounds obtained in \eqref{eqn:simplified_tilde.1} and \eqref{eqn:simplified_tilde.3}:
\begin{align}
	 \int_{8\lipmax\Qf\left(\frac{mp}{2}\right)}^{\tfmax - \tfmin}  2u\exp\left( -\frac{n \big( u - 4\lipmax \Qf\left(\frac{mp}{2}\right) \big)}{12\lipmax} \right)du
	 	&\leq \frac{288\lipmax ^2}{n^2} + 8\lipmax \Qf\left(\frac{mp}{2}\right) \sqrt{\frac{3\lipmax \pi}{n}},		\label{eqn:simplified_hat.1}\\
	 \int_0^{\tfmax - \tfmin} 2 u \exp\left( -\frac{n u^2}{8\lipmax^2} \right) du.								\label{eqn:simplified_hat.3}
	 	&\leq \frac{8\lipmax^2}{n}.
\end{align}
It remains to establish an upper bound for the term in \eqref{eqn:MSE_hat_term.2}. By the same argument as in the proof of Theorem 
\ref{thm:MSE_noisy_known} (more precisely, the argument to obtain \eqref{eqn:simplified_tilde.2}), we let
\[	c_1' \triangleq \frac{ 1 }{ 2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} }\big( \frac{np}{2} \big)^{5/12} , \quad\text{and}\quad 
	c_2' \triangleq  2\lipmax \big( \slackAA + \slackBB + \slackCC \big).		\]
Then we achieve
\begin{align}
	&\int_{4\lipmax( \slackAA + \slackBB + \slackCC)}^{\tfmax - \tfmin}
			8np \exp\bigg( \frac{- \big( \frac{np}{2} \big)^{5/12}  }{2 \constdd^2 \left( \log (2np) \right)^{\frac{2}{\beta}} } 
			\Big( u - 2\lipmax \big( \slackAA + \slackBB + \slackCC \big) \Big)^2 \bigg) u ~ du		\nonumber\\
		&\qquad=	\int_{2  c_2'}^{\tfmax - \tfmin} u\exp\left( - c_1' \left( u - c_2' \right)^2	 \right)du	\nonumber\\
		&\qquad\leq	\int_{2  c_2'}^{\tfmax - \tfmin} u\exp\left( - \frac{c_1'}{4} u^2	 \right)du		
			\qquad	\because u - c_2' \geq \frac{u}{2}, ~ \forall u \geq 2c_2'		\nonumber\\
		&\qquad\leq	\int_{0}^{\infty} u\exp\left( - \frac{c_1'}{4} u^2	 \right)du
			\qquad\qquad\quad\because u \exp\left( - \frac{c_1'}{4} u^2	 \right) \geq 0,~\forall u \geq 0	\nonumber\\
		&\qquad= \frac{2}{c_1'}.	\label{eqn:simplified_hat.2}
\end{align}

Inserting \eqref{eqn:simplified_hat.1} to \eqref{eqn:MSE_hat_term.1}, \eqref{eqn:simplified_hat.3} to \eqref{eqn:MSE_hat_term.3}, and 
\eqref{eqn:simplified_hat.2} to \eqref{eqn:MSE_hat_term.2}, we acquire the following upper bound:
\begin{align*}
	\MSE\left( \hat{\varphi} \right)
	&\leq \left[ 8\lipmax \Qf\left(\frac{mp}{2}\right) \right]^2 
		+ \left[ 4\lipmax \big( \slackAA + \slackBB + \slackCC \big) \right]^2\\
	&\quad + \frac{288\lipmax ^2}{n^2} + 8\lipmax \Qf\left(\frac{mp}{2}\right) \sqrt{\frac{3\lipmax \pi}{n}}
		+ 4\sqrt{2} \constdd^2  \frac{ \big( \log (2np) \big)^{\frac{2}{\beta}} }{ ( np )^{5/12}}
		+  \frac{8\lipmax^2}{n} 
		+ C_{m,n,p} \big( \tfmax - \tfmin \big)^2.
\end{align*}
Recall that $\Qf\big( \frac{mp}{2}\big) = \frac{\constee}{\sqrt{mp}}$. Rearranging the terms in the increasing order of convergence rates concludes the proof.
\end{proof}


